The Relative Specific Type Ia Supernovae Rate From Three Years of ASAS-SN

We analyze the 476 SN Ia host galaxies from the All-Sky Automated Survey for Supernova (ASAS-SN) Bright Supernova Catalogs to determine the observed relative Type Ia supernova (SN) rates as a function of luminosity and host galaxy properties. We find that the luminosity distribution of the SNe Ia in our sample is reasonably well described by a Schechter function with a faint-end slope $\alpha \approx 1.5$ and a knee $M_{\star} \approx -18.0$. Our specific SN Ia rates are consistent with previous results but extend to far lower host galaxy masses. We find an overall rate that scales as $(M_{\star}/10^{10} M_{\odot})^{\alpha}$ with $\alpha \approx -0.5$. This shows that the specific SN Ia rate continues rising towards lower masses even in galaxies as small as $\log(M_{\star} / M_{\odot}) \lesssim 7.0$, where it is enhanced by a factor of $\sim10-20$ relative to host galaxies with stellar masses $\sim10^{10}M_{\odot}$. We find no strong dependence of the specific SN Ia rate on the star formation activity of the host galaxies, but additional observations are required to improve the constraints on the star formation rates.

==> tab1.tex <==
\begin{table}
\begin{minipage}{\textwidth}
\caption{Physical host data.\hfill}\begin{tabular}{llcclllrr}
\hline
SN name & Host name & Included?$^{a}$ & SN type & Redshift &$V_{\rm peak}^{b}$ & $A_{\rm V}$ & $\log({\rm M}_{\star})$ [M$_{\odot}$] & $\log({\rm SFR})$ [M$_{\odot}$~yr$^{-1}$]$^{c}$  \\
\hline
ASASSN-13an & 2MASX J13453653-0719350 & True & Ia & 0.0216 & 15.8 & 0.11 & $10.52_{-0.29}^{+0.14}$ & $ 0.01_{-0.09}^{+0.07}$ \\
ASASSN-13ar & VV 478 & True & Ia & 0.01775 & 14.8 & 0.15 & $9.26_{-0.14}^{+0.07}$ & $-0.65_{-3.35}^{+0.18}$ \\
ASASSN-13av & NGC 7068 & True & Ia & 0.01729 & 15.7 & 0.27 & $10.79_{-0.18}^{+0.09}$ & $<-0.51$ \\
ASASSN-13aw & CGCG 252-043 & True & Ia & 0.016835 & 15.0 & 0.07 & $9.84_{-0.15}^{+0.45}$ & $-0.36_{-0.23}^{+0.25}$ \\
ASASSN-13bb & UGC 01395 & True & Ia & 0.017405 & 15.7 & 0.20 & $10.80_{-0.24}^{+0.08}$ & $-0.06_{-0.23}^{+0.03}$ \\
ASASSN-13cc & NGC 1954 & True & Ia & 0.01044 & 15.0 & 0.39 & $11.46_{-0.01}^{+0.01}$ & $<-4.00$ \\
ASASSN-13ch & CGCG 023-030 & True & Ia & 0.01646 & 15.8 & 0.33 & $9.12_{-0.10}^{+0.20}$ & $-0.42_{-0.28}^{+0.11}$ \\
ASASSN-13cj & CGCG 051-075 & True & Ia & 0.018 & 15.3 & 0.20 & $9.43_{-0.01}^{+0.01}$ & $<-4.00$ \\
ASASSN-13cp & ARK 477 & True & Ia & 0.023576 & 15.9 & 0.16 & $11.12_{-0.33}^{+0.01}$ & $-0.19_{-0.34}^{+0.01}$ \\
ASASSN-13cu & VIII Zw 035 & True & Ia & 0.0272 & 16.6 & 0.09 & $10.30_{-0.17}^{+0.15}$ & $-0.02_{-0.15}^{+0.02}$ \\
ASASSN-13dd & NGC 2765 & True & Ia & 0.01255 & 15.2 & 0.09 & $11.01_{-0.14}^{+0.14}$ & $<-1.83$ \\
ASASSN-13dl & Uncatalogued & True & Ia & 0.027 & 16.6 & 0.14 & $8.59_{-0.92}^{+0.33}$ & $<0.84$ \\
ASASSN-13dm & 2MASX J03021111+1555387 & True & Ia & 0.017 & 15.6 & 0.36 & $10.29_{-0.07}^{+0.07}$ & $-0.93_{-0.02}^{+0.03}$ \\
ASASSN-14ad & KUG 1237+183 & True & Ia & 0.0264 & 16.9 & 0.05 & $9.71_{-0.47}^{+0.18}$ & $-0.23_{-0.24}^{+0.09}$ \\
ASASSN-14ar & IC 0527 & True & Ia-91bg & 0.02298 & 16.0 & 0.06 & $10.88_{-0.44}^{+0.21}$ & $ 0.20_{-4.20}^{+0.11}$ \\
ASASSN-14as & MGC +06-29-001 & True & Ia & 0.03744 & 16.9 & 0.04 & $10.30_{-0.10}^{+0.09}$ & $-1.30_{-2.70}^{+0.98}$ \\
ASASSN-14ax & SDSS J171000.69+270619.5 & True & Ia & 0.033 & 16.4 & 0.13 & $9.00_{-0.10}^{+0.10}$ & $-0.58_{-0.19}^{+0.04}$ \\
ASASSN-14ay & 2MASX J15570268+3725001 & True & Ia & 0.030869 & 16.3 & 0.06 & $10.19_{-0.13}^{+0.24}$ & $-1.70_{-2.30}^{+0.51}$ \\
ASASSN-14ba & SDSS J102131.91+082419.8 & True & Ia-91T & 0.032668 & 16.8 & 0.08 & $9.19_{-0.08}^{+0.08}$ & $-1.07_{-1.70}^{+0.01}$ \\
ASASSN-14bb & 2MASX J12141125+3839400 & True & Ia & 0.023 & 16.1 & 0.04 & $9.72_{-0.09}^{+0.08}$ & $-1.48_{-0.01}^{+0.00}$ \\
ASASSN-14bd & IC 0831 & True & Ia-91bg & 0.021405 & 16.9 & 0.03 & $11.00_{-0.28}^{+0.04}$ & $-2.19_{-1.81}^{+0.06}$ \\
ASASSN-14bt & UGC 05566 & True & Ia & 0.0289 & 16.2 & 0.03 & $11.18_{-0.01}^{+0.01}$ & $<-4.00$ \\
ASASSN-14cb & 2MASXi J1308145+620200 & True & Ia & 0.033643 & 16.5 & 0.04 & $9.49_{-0.16}^{+0.04}$ & $<-2.18$ \\
ASASSN-14co & CGCG 023-005 & True & Ia & 0.03334 & 16.9 & 0.26 & $10.62_{-0.32}^{+0.07}$ & $ 0.21_{-0.08}^{+0.09}$ \\
ASASSN-14cu & 2MASX J12470274-2414435 & True & Ia & 0.024797 & 16.7 & 0.26 & $10.65_{-0.24}^{+0.07}$ & $-1.54_{-2.46}^{+0.04}$ \\
ASASSN-14db & ESO 075-G049 & True & Ia & 0.037519 & 16.8 & 0.08 & $10.57_{-0.03}^{+0.50}$ & $-3.69_{-0.31}^{+4.10}$ \\
ASASSN-14dc & 2MASX J02183825+3336556 & False & Ia+CSM & 0.044 & 14.9 & 0.20 & $10.20_{-0.07}^{+0.30}$ & $-0.28_{-0.04}^{+0.14}$ \\
ASASSN-14dz & Mrk 842 & True & Ia & 0.022202 & 15.8 & 0.10 & $10.45_{-0.06}^{+0.27}$ & $-3.23_{-0.77}^{+1.70}$ \\
ASASSN-14ef & MCG -05-52-046 & True & Ia & 0.028733 & 16.1 & 0.06 & $10.91_{-0.19}^{+0.04}$ & $-2.27_{-1.73}^{+0.77}$ \\
ASASSN-14em & KUG 1359+345 & True & Ia & 0.035124 & 16.7 & 0.04 & $10.35_{-0.18}^{+0.16}$ & $-0.13_{-0.24}^{+0.03}$ \\
ASASSN-14eo & CGCG 461-012 & True & Ia & 0.026819 & 15.8 & 0.15 & $10.17_{-0.07}^{+0.09}$ & $ 0.07_{-0.23}^{+0.18}$ \\
ASASSN-14ep & CGCG 338-006 & True & Ia & 0.022829 & 15.6 & 0.07 & $10.46_{-0.13}^{+0.23}$ & $-1.54_{-2.46}^{+0.03}$ \\
ASASSN-14es & IC 4462 & True & Ia & 0.030705 & 16.5 & 0.07 & $10.44_{-0.08}^{+0.24}$ & $ 0.06_{-0.02}^{+0.15}$ \\
ASASSN-14eu & MCG -01-38-015 & False & Ia-00cx & 0.022722 & 15.3 & 0.42 & $11.32_{-0.01}^{+0.01}$ & $<-4.00$ \\
ASASSN-14ew & 2MASX J20220000-5147474 & True & Ia & 0.019597 & 14.9 & 0.16 & $9.46_{-0.07}^{+0.50}$ & $<-0.31$ \\
ASASSN-14fa & ESO 416-G039 & True & Ia & 0.022589 & 15.8 & 0.06 & $10.90_{-0.17}^{+0.14}$ & $-1.99_{-2.01}^{+0.67}$ \\
ASASSN-14fo & GALEXASC J203406.21-015759.2 & True & Ia & 0.02 & 15.6 & 0.34 & $9.08_{-0.12}^{+0.31}$ & $<-1.86$ \\
ASASSN-14fw & MCG -01-60-044 & True & Ia & 0.027169 & 16.5 & 0.08 & $10.37_{-0.18}^{+0.23}$ & $ 0.15_{-0.18}^{+0.05}$ \\
ASASSN-14gh & SDSS J171509.30+414841.6 & True & Ia & 0.02 & 15.6 & 0.07 & $7.86_{-0.30}^{+0.17}$ & $-1.17_{-2.83}^{+0.06}$ \\
ASASSN-14hp & 2MASX J21303015-7038489 & True & Ia & 0.03892 & 16.5 & 0.10 & $9.62_{-0.07}^{+0.55}$ & $-3.09_{-0.91}^{+3.22}$ \\
ASASSN-14hr & 2MASX J01504127-1431032 & True & Ia & 0.03362 & 16.6 & 0.04 & $10.53_{-0.30}^{+0.08}$ & $ 0.13_{-0.09}^{+0.09}$ \\
ASASSN-14hu & ESO 058-G012 & True & Ia & 0.015 & 15.6 & 0.20 & $10.34_{-1.68}^{+0.10}$ & $<1.88$ \\
ASASSN-14ig & ESO 113-G032 & True & Ia & 0.029 & 16.3 & 0.06 & $11.15_{-0.34}^{+0.24}$ & $-0.24_{-3.76}^{+0.02}$ \\
ASASSN-14ih & MCG -04-53-013 & True & Ia & 0.033466 & 16.6 & 0.06 & $11.07_{-0.22}^{+0.08}$ & $-1.03_{-2.97}^{+0.02}$ \\
ASASSN-14ii & 2dFGRS S588Z294 & True & Ia & 0.0308 & 16.6 & 0.06 & $10.68_{-0.24}^{+0.12}$ & $-1.51_{-2.49}^{+0.01}$ \\
ASASSN-14in & 2MASX J18242915+5226380 & True & Ia & 0.033 & 16.0 & 0.10 & $9.72_{-0.31}^{+0.15}$ & $-0.78_{-0.12}^{+0.08}$ \\
ASASSN-14iu & NGC 2771 & True & Ia & 0.016855 & 15.5 & 0.05 & $10.81_{-0.01}^{+0.01}$ & $-0.16_{0.00}^{+0.00}$ \\
ASASSN-14jc & 2MASX J07353554-6246099 & True & Ia & 0.011325 & 15.6 & 0.43 & $9.80_{-0.51}^{+0.07}$ & $-0.45_{-3.55}^{+0.05}$ \\
ASASSN-14jg & 2MASX J23331223-6034201 & True & Ia & 0.014827 & 14.9 & 0.04 & $9.37_{-0.09}^{+0.55}$ & $-3.34_{-0.66}^{+3.25}$ \\
ASASSN-14jz & GALEXASC J184443.33-524819.2 & True & Ia & 0.012 & 14.9 & 0.15 & $8.09_{-1.42}^{+0.38}$ & $-0.76_{-3.24}^{+0.20}$ \\
ASASSN-14kd & 2MASX J22532475+0447583 & True & Ia & 0.026 & 15.9 & 0.19 & $10.39_{-0.09}^{+0.15}$ & $-0.64_{-0.04}^{+0.01}$ \\
ASASSN-14kq & 2MASX J23451480-2947009 & True & Ia & 0.0336 & 16.3 & 0.05 & $9.79_{-0.08}^{+0.23}$ & $-0.14_{-0.19}^{+0.10}$ \\
ASASSN-14kr & GALEXASC J125413.02-073849.5 & True & Ia & 0.014 & 15.5 & 0.10 & $8.48_{-0.19}^{+0.27}$ & $-1.04_{-2.96}^{+0.44}$ \\
ASASSN-14lo & UGC 06837 & True & Ia & 0.01993 & 15.8 & 0.09 & $10.14_{-0.08}^{+0.01}$ & $-0.82_{0.00}^{+0.02}$ \\
ASASSN-14lp & NGC 4666 & True & Ia & 0.0051 & 11.9 & 0.07 & $10.69_{-0.01}^{+0.01}$ & $-0.62_{0.00}^{+0.00}$ \\
ASASSN-14lq & 2MASX J22571481-2058014 & True & Ia-91T & 0.026191 & 16.2 & 0.09 & $10.97_{-0.01}^{+0.01}$ & $<-4.00$ \\
ASASSN-14lt & IC 0299 & True & Ia & 0.032046 & 16.5 & 0.15 & $10.97_{-0.22}^{+0.15}$ & $-1.13_{-2.87}^{+0.02}$ \\
ASASSN-14lu & 2MASX J14103977-0241003 & True & Ia & 0.026995 & 16.4 & 0.18 & $10.91_{-0.15}^{+0.08}$ & $-1.19_{-0.72}^{+0.01}$ \\
ASASSN-14lv & LCRS B232926.0-413242 & True & Ia & 0.049194 & 16.4 & 0.06 & $10.28_{-0.51}^{+0.15}$ & $ 0.23_{-4.23}^{+0.06}$ \\
ASASSN-14lw & GALEXASC J010647.95-465904.1 & True & Ia & 0.016 & 15.5 & 0.04 & $7.35_{-0.64}^{+0.71}$ & $<-2.02$ \\
ASASSN-14me & ESO 113-G047 & True & Ia & 0.018 & 14.9 & 0.06 & $8.46_{-1.13}^{+0.62}$ & $<1.96$ \\
ASASSN-14mf & GALEXASC J000454.54-322615.3 & True & Ia & 0.0311 & 15.9 & 0.04 & $8.71_{-1.14}^{+0.65}$ & $-2.90_{-1.10}^{+2.30}$ \\
ASASSN-14mg & GALEXASC J025358.03-213854.7 & True & Ia & 0.031 & 16.6 & 0.07 & $8.95_{-0.03}^{+0.06}$ & $-2.95_{-1.05}^{+1.70}$ \\
ASASSN-14mu & KUG 0923+457 & True & Ia & 0.027249 & 16.5 & 0.05 & $8.78_{-0.17}^{+0.01}$ & $<-1.43$ \\
ASASSN-14mw & AM 0139-655 NED02 & True & Ia & 0.027406 & 15.7 & 0.06 & $11.22_{-1.69}^{+0.09}$ & $<2.59$ \\
ASASSN-14my & NGC 3774 & True & Ia & 0.020514 & 15.3 & 0.10 & $10.55_{-0.44}^{+0.27}$ & $ 0.05_{-4.05}^{+0.47}$ \\
ASASSN-15ad & PGC 902451 & True & Ia & 0.024 & 16.3 & 0.58 & $9.08_{-1.07}^{+0.30}$ & $<0.06$ \\
ASASSN-15ae & 2MASX J15510599+3425520 & True & Ia & 0.03124 & 16.4 & 0.09 & $9.31_{-0.03}^{+0.08}$ & $<-0.32$ \\
ASASSN-15aj & NGC 3449 & True & Ia & 0.01092 & 14.7 & 0.21 & $10.89_{-0.27}^{+0.24}$ & $-0.40_{-3.60}^{+0.21}$ \\
ASASSN-15ak & UGC 00110 & True & Ia-91T & 0.01503 & 14.7 & 0.12 & $9.26_{-0.23}^{+0.46}$ & $-0.48_{-3.52}^{+0.20}$ \\
ASASSN-15al & GALEXASC J045749.46-213526.3 & True & Ia & 0.032 & 16.8 & 0.09 & $8.95_{-0.11}^{+0.10}$ & $-0.76_{-3.24}^{+0.26}$ \\
ASASSN-15ar & CGCG 439-010 & True & Ia & 0.02882 & 16.6 & 0.30 & $10.64_{-0.22}^{+0.36}$ & $-2.89_{-1.11}^{+3.72}$ \\
ASASSN-15as & SDSS J093916.69+062551.1 & True & Ia & 0.028 & 16.1 & 0.12 & $7.89_{-0.16}^{+0.15}$ & $-1.92_{-2.08}^{+0.16}$ \\
ASASSN-15az & 2MASX J11083863-1014456 & True & Ia & 0.02832 & 16.3 & 0.17 & $10.17_{-0.06}^{+0.24}$ & $<-2.52$ \\
ASASSN-15ba & SDSS J140455.12+085514.0 & True & Ia & 0.02313 & 15.8 & 0.07 & $8.63_{-0.25}^{+0.45}$ & $-1.21_{-2.79}^{+0.17}$ \\
ASASSN-15bc & 2MASX J04061478-0853112 & True & Ia & 0.03672 & 16.9 & 0.12 & $10.11_{-0.05}^{+0.01}$ & $<-1.33$ \\
ASASSN-15be & GALEXASC J025245.83-341850.6 & True & Ia & 0.0219 & 15.6 & 0.05 & $8.34_{-1.52}^{+0.40}$ & $-0.71_{-3.29}^{+0.09}$ \\
ASASSN-15bf & 2MASX J04384102-4137212 & True & Ia & 0.04853 & 16.9 & 0.07 & $9.70_{-0.56}^{+1.22}$ & $-0.49_{-3.51}^{+2.83}$ \\
ASASSN-15bk & CGCG 078-056 & False & Ia & 0.03428 & 17.1 & 0.12 & $10.32_{-0.09}^{+0.24}$ & $-0.32_{-0.01}^{+0.23}$ \\
ASASSN-15bm & GALEXASC J150551.56-053737.2 & True & Ia & 0.0206 & 15.5 & 0.22 & $10.40_{-0.29}^{+0.01}$ & $-0.30_{-0.10}^{+0.05}$ \\
ASASSN-15bn & GALEXASC J155536.57+664316.5 & True & Ia & 0.028 & 16.1 & 0.09 & $9.21_{-0.25}^{+0.16}$ & $-0.79_{-3.21}^{+0.26}$ \\
ASASSN-15bo & SDSS J144455.21+243443.9 & True & Ia & 0.0363 & 16.4 & 0.12 & $8.87_{-0.17}^{+0.30}$ & $-1.06_{-0.20}^{+0.21}$ \\
ASASSN-15cb & VCC 1810 & True & Ia & 0.04004 & 16.8 & 0.09 & $10.18_{-0.05}^{+0.25}$ & $ 0.08_{-0.01}^{+0.19}$ \\
ASASSN-15cd & CGCG 064-017 & True & Ia & 0.03435 & 16.4 & 0.08 & $9.84_{-0.12}^{+0.08}$ & $-0.32_{-3.68}^{+0.27}$ \\
ASASSN-15cq & CGCG 218-007 & True & Ia & 0.02728 & 15.9 & 0.04 & $10.65_{-0.01}^{+0.18}$ & $-1.24_{-0.04}^{+0.00}$ \\
ASASSN-15cz & SBS 1132+579 & True & Ia & 0.02877 & 16.0 & 0.04 & $11.08_{-0.36}^{+0.01}$ & $ 0.12_{-4.12}^{+0.20}$ \\
ASASSN-15da & 2MASX J05235186-2442081 & True & Ia & 0.048 & 16.8 & 0.10 & $10.44_{-0.29}^{+0.07}$ & $-0.88_{-3.12}^{+0.34}$ \\
ASASSN-15db & NGC 5996 & True & Ia & 0.011 & 14.5 & 0.09 & $9.78_{-0.12}^{+0.08}$ & $ 0.07_{-4.07}^{+0.28}$ \\
ASASSN-15dc & SDSS J150130.77-003222.8 & True & Ia & 0.04161 & 16.7 & 0.18 & $9.54_{-0.19}^{+0.43}$ & $-0.39_{-0.42}^{+0.13}$ \\
ASASSN-15dd & CGCG 107-031 & True & Ia & 0.02437 & 16.1 & 0.15 & $10.69_{-0.10}^{+0.10}$ & $<-2.14$ \\
ASASSN-15de & SDSS J112849.43+295454.2 & True & Ia-91T & 0.05172 & 16.7 & 0.06 & $10.36_{-0.10}^{+0.27}$ & $<0.82$ \\
ASASSN-15df & SDSS J103529.47+343420.2 & True & Ia & 0.03631 & 16.7 & 0.05 & $8.88_{-0.20}^{+0.32}$ & $-0.76_{-3.24}^{+0.25}$ \\
ASASSN-15dz & CGCG 080-055 & True & Ia & 0.03222 & 16.3 & 0.17 & $10.40_{-0.17}^{+0.26}$ & $ 0.38_{-0.11}^{+0.11}$ \\
ASASSN-15eb & ESO 561-G012 & True & Ia & 0.01648 & 15.7 & 0.53 & $11.25_{-0.11}^{+0.01}$ & $<-2.93$ \\
ASASSN-15fa & NGC 6319 & True & Ia & 0.02741 & 16.3 & 0.07 & $11.27_{-0.16}^{+0.07}$ & $ 0.05_{-0.02}^{+0.03}$ \\
ASASSN-15fj & 2MASX J17100856+7443426 & True & Ia & 0.045 & 16.9 & 0.10 & $10.56_{-0.07}^{+0.18}$ & $<-2.12$ \\
ASASSN-15fk & 2MASX J05401415-3848285 & True & Ia & 0.03597 & 16.4 & 0.08 & $10.85_{-0.11}^{+0.18}$ & $<-1.36$ \\
ASASSN-15fr & 2MASX J09202045-0738229 & True & Ia & 0.03344 & 16.5 & 0.10 & $9.84_{-0.13}^{+0.06}$ & $<0.43$ \\
ASASSN-15fs & CGCG 229-010 & True & Ia-91T & 0.02902 & 16.3 & 0.25 & $10.69_{-0.31}^{+0.01}$ & $-0.27_{-0.20}^{+0.02}$ \\
ASASSN-15fy & Uncatalogued & True & Ia & 0.025 & 16.2 & 0.42 & $6.49_{-0.64}^{+0.30}$ & $-1.65_{-2.35}^{+0.32}$ \\
ASASSN-15ga & NGC 4866 & True & Ia & 0.00663 & 15.1 & 0.08 & $10.89_{-0.01}^{+0.07}$ & $-0.89_{-0.54}^{+0.00}$ \\
ASASSN-15go & 2MASX J06113048-1629085 & True & Ia & 0.01892 & 15.8 & 0.44 & $10.39_{-0.46}^{+0.09}$ & $-0.11_{-3.89}^{+0.18}$ \\
ASASSN-15gr & ESO 366-G015 & True & Ia & 0.024 & 16.0 & 0.27 & $8.77_{-0.98}^{+0.77}$ & $-0.59_{-3.41}^{+3.01}$ \\
ASASSN-15gw & NGC 5536 & True & Ia & 0.01951 & 16.2 & 0.03 & $10.62_{-0.20}^{+0.17}$ & $-0.21_{-0.37}^{+0.01}$ \\
ASASSN-15gz & 2MASX J14423254-1327294 & True & Ia & 0.03403 & 16.7 & 0.26 & $10.51_{-0.05}^{+0.23}$ & $<-1.43$ \\
ASASSN-15hc & LCRS B102206.7-024353 & True & Ia & 0.03098 & 16.6 & 0.12 & $9.87_{-0.09}^{+0.17}$ & $-0.32_{-0.02}^{+0.16}$ \\
ASASSN-15he & ESO 069-G005 & True & Ia & 0.01588 & 16.2 & 0.23 & $8.60_{-0.58}^{+1.20}$ & $-2.38_{-1.62}^{+3.82}$ \\
ASASSN-15hf & ESO 375-G041 & True & Ia & 0.00618 & 14.3 & 0.27 & $9.77_{-0.26}^{+0.08}$ & $-2.33_{-1.67}^{+0.00}$ \\
ASASSN-15hg & CGCG 063-098 & True & Ia & 0.02977 & 16.6 & 0.13 & $10.90_{-0.16}^{+0.07}$ & $-0.79_{-0.02}^{+0.04}$ \\
ASASSN-15hh & NGC 2115A & True & Ia & 0.02339 & 15.7 & 0.17 & $10.98_{-1.68}^{+0.10}$ & $<2.36$ \\
ASASSN-15ho & 2MASXi J0909234-044327 & True & Ia & 0.046 & 16.8 & 0.06 & $9.94_{-0.16}^{+0.39}$ & $ 0.26_{-0.17}^{+0.11}$ \\
ASASSN-15hx & GALEXASC J134316.80-313318.2 & True & Ia & 0.0081 & 13.3 & 0.13 & $<8.47$ & $-1.68_{-2.32}^{+0.03}$ \\
ASASSN-15hy & Uncatalogued & False & Ia-07if & 0.025 & 15.2 & 0.42 & $8.62_{-0.06}^{+0.06}$ & $-3.47_{-0.53}^{+1.30}$ \\
ASASSN-15hz & APMUKS B222606.49-654315.6 & True & Ia & 0.033 & 16.1 & 0.07 & $9.07_{-1.13}^{+0.63}$ & $<2.57$ \\
ASASSN-15ic & 2MASX J06145320-4247357 & True & Ia & 0.025 & 15.9 & 0.15 & $10.21_{-0.18}^{+0.08}$ & $-2.88_{-1.12}^{+0.08}$ \\
ASASSN-15ih & GALEXASC J095959.71-025322.1 & True & Ia & 0.01983 & 16.0 & 0.13 & $9.38_{-0.25}^{+0.32}$ & $-0.39_{-0.15}^{+0.13}$ \\
ASASSN-15il & 2MASX J15570808-1240252 & True & Ia & 0.02332 & 16.2 & 0.48 & $10.27_{-0.20}^{+0.21}$ & $-1.13_{-1.31}^{+0.03}$ \\
ASASSN-15ja & ESO 113-G018 & True & Ia & 0.02632 & 16.0 & 0.06 & $10.76_{-0.06}^{+0.27}$ & $-1.91_{-2.09}^{+0.69}$ \\
ASASSN-15jb & 2MASX J11200680+3407396 & True & Ia & 0.03566 & 17.0 & 0.07 & $10.74_{-0.09}^{+0.05}$ & $<-2.28$ \\
ASASSN-15jf & GALEXASC J222510.84-502347.7 & True & Ia & 0.036 & 16.2 & 0.04 & $8.19_{-0.82}^{+0.49}$ & $-1.29_{-2.71}^{+0.04}$ \\
ASASSN-15jg & SDSS J104655.44-021927.0 & True & Ia & 0.036 & 16.9 & 0.12 & $9.14_{-0.10}^{+0.25}$ & $-0.86_{-0.26}^{+0.16}$ \\
ASASSN-15ji & ESO 536-G008 & True & Ia & 0.05559 & 17.0 & 0.07 & $11.18_{-0.15}^{+0.07}$ & $ 0.32_{-0.03}^{+0.04}$ \\
ASASSN-15jl & SDSS J152241.16+505836.0 & True & Ia & 0.03475 & 16.1 & 0.04 & $9.14_{-0.19}^{+0.38}$ & $-0.88_{-0.88}^{+0.28}$ \\
ASASSN-15jm & 2MASX J17210913+2534558 & True & Ia-91T & 0.053 & 16.6 & 0.18 & $10.32_{-0.07}^{+0.06}$ & $-0.03_{-0.98}^{+0.61}$ \\
ASASSN-15jo & ALLWISE J140643.89-342721.4 & True & Ia & 0.011 & 15.2 & 0.20 & $<8.35$ & $<1.25$ \\
ASASSN-15js & 2MFGC 08437 & True & Ia & 0.02106 & 16.7 & 0.07 & $9.31_{-0.01}^{+0.26}$ & $-1.14_{-0.02}^{+0.26}$ \\
ASASSN-15jt & 2MASX J13080914+2749354 & True & Ia & 0.023 & 16.2 & 0.03 & $10.15_{-0.11}^{+0.01}$ & $<-3.52$ \\
ASASSN-15ke & 2MASX J15254441+5921091 & True & Ia & 0.04536 & 16.9 & 0.03 & $10.34_{-0.11}^{+0.08}$ & $ 0.05_{-0.27}^{+0.01}$ \\
ASASSN-15kg & 2MASX J08401168-0435369 & True & Ia & 0.01426 & 15.1 & 0.06 & $10.22_{-0.16}^{+0.23}$ & $-0.09_{-0.18}^{+0.09}$ \\
ASASSN-15kk & UGC 04883 & True & Ia & 0.00989 & 14.1 & 0.09 & $10.53_{-0.25}^{+0.13}$ & $-1.06_{-0.47}^{+0.03}$ \\
ASASSN-15kn & 2MASX J12415081-0710092 & True & Ia & 0.02473 & 16.1 & 0.08 & $10.90_{-0.15}^{+0.02}$ & $-1.49_{-0.78}^{+0.05}$ \\
ASASSN-15kp & AM 1255-315 & True & Ia & 0.0174 & 15.3 & 0.23 & $10.64_{-0.17}^{+0.15}$ & $-2.25_{-1.75}^{+0.68}$ \\
ASASSN-15kq & GALEXASC J064843.83-541213.4 & True & Ia & 0.02676 & 16.3 & 0.28 & $10.30_{-0.46}^{+0.06}$ & $-0.57_{-3.43}^{+0.03}$ \\
ASASSN-15kx & MCG +06-49-001 & True & Ia & 0.01802 & 15.9 & 0.45 & $10.74_{-0.06}^{+0.01}$ & $<-4.00$ \\
ASASSN-15la & NGC 5517 & True & Ia & 0.0279 & 16.4 & 0.05 & $10.96_{-0.28}^{+0.16}$ & $ 0.03_{-0.37}^{+0.02}$ \\
ASASSN-15lg & CGCG 044-042 & True & Ia & 0.02032 & 15.8 & 0.09 & $9.89_{-0.09}^{+0.32}$ & $-0.85_{0.00}^{+0.23}$ \\
ASASSN-15li & 2MASX J14250783+6253235 & True & Ia & 0.0261 & 16.2 & 0.04 & $9.67_{-0.09}^{+0.08}$ & $-0.97_{-0.02}^{+0.01}$ \\
ASASSN-15lo & GALEXASC J225332.83+194232.9 & True & Ia & 0.041 & 16.6 & 0.18 & $9.68_{-0.12}^{+0.27}$ & $-0.25_{-0.89}^{+0.32}$ \\
ASASSN-15lp & MRK 0576 & True & Ia & 0.01769 & 15.1 & 0.18 & $9.89_{-0.17}^{+0.24}$ & $-0.13_{-0.11}^{+0.05}$ \\
ASASSN-15lu & 2MASX J13211289+4015564 & True & Ia & 0.03504 & 16.5 & 0.04 & $10.03_{-0.11}^{+0.09}$ & $-0.26_{-0.26}^{+0.00}$ \\
ASASSN-15mc & UGC 02295 & True & Ia & 0.01392 & 15.0 & 0.17 & $10.85_{-0.25}^{+0.10}$ & $-0.83_{-3.17}^{+0.42}$ \\
ASASSN-15mf & UGC 09108 NED02 & True & Ia & 0.026 & 16.2 & 0.10 & $10.74_{-0.26}^{+0.08}$ & $<-1.03$ \\
ASASSN-15mg & 2MASX J15322270+4150586 & True & Ia & 0.04286 & 17.0 & 0.09 & $10.10_{-0.19}^{+0.09}$ & $-0.54_{-0.40}^{+0.02}$ \\
ASASSN-15mi & MRK 0283a & True & Ia & 0.03445 & 16.3 & 0.06 & $9.49_{-0.18}^{+0.06}$ & $ 0.04_{-0.95}^{+0.10}$ \\
ASASSN-15ml & 2MASX J20030163-2154516 & True & Ia & 0.01862 & 16.6 & 0.49 & $10.18_{-0.24}^{+0.14}$ & $-0.49_{-0.23}^{+0.03}$ \\
ASASSN-15mp & 2MASX J00584521-1404122 & True & Ia & 0.037 & 16.3 & 0.06 & $10.14_{-0.07}^{+0.20}$ & $-3.48_{-0.52}^{+1.74}$ \\
ASASSN-15mq & 2MASX J05014660-1343503 & False & Ia & 0.02494 & 17.2 & 0.32 & $10.44_{-0.18}^{+0.18}$ & $-2.45_{-1.55}^{+0.77}$ \\
ASASSN-15ms & SDSS J145027.61+063713.3 & False & Ia & 0.04411 & 17.2 & 0.10 & $9.41_{-0.18}^{+0.38}$ & $-0.08_{-0.16}^{+0.13}$ \\
ASASSN-15mx & SDSS J142443.90+260255.4 & True & Ia & 0.041 & 16.9 & 0.04 & $9.26_{-0.22}^{+0.26}$ & $-0.74_{-3.26}^{+0.26}$ \\
ASASSN-15nh & 2MASX J00443129-0301012 & True & Ia & 0.0541 & 16.8 & 0.07 & $11.44_{-0.27}^{+0.01}$ & $-0.66_{-3.34}^{+0.01}$ \\
ASASSN-15nn & UGC 01332 & True & Ia & 0.02262 & 16.0 & 0.56 & $11.45_{-0.16}^{+0.01}$ & $<0.04$ \\
ASASSN-15np & 2MASX J15060265+0733415 & True & Ia & 0.03769 & 16.5 & 0.08 & $10.14_{-0.05}^{+0.18}$ & $-1.75_{-0.76}^{+0.00}$ \\
ASASSN-15nq & 2MFGC 13779 & True & Ia & 0.03042 & 16.2 & 0.13 & $10.87_{-0.03}^{+0.01}$ & $<-4.00$ \\
ASASSN-15nr & CGCG 082-031 & True & Ia-91T & 0.02321 & 16.0 & 0.36 & $10.46_{-0.31}^{+0.14}$ & $-0.31_{-0.20}^{+0.04}$ \\
ASASSN-15ns & MRK 0887 & True & Ia & 0.03067 & 16.2 & 0.04 & $11.36_{-0.03}^{+0.01}$ & $<-3.98$ \\
ASASSN-15od & MCG -01-07-004 & True & Ia & 0.01799 & 16.6 & 0.08 & $9.71_{-0.17}^{+0.14}$ & $-0.03_{-3.97}^{+0.09}$ \\
ASASSN-15og & GALEXASC J032107.24-311845.8 & False & Ia+CSM & 0.06831 & 16.1 & 0.04 & $9.80_{-0.09}^{+0.27}$ & $-0.74_{-0.01}^{+0.26}$ \\
ASASSN-15oh & MCG +06-49-027 & True & Ia & 0.01684 & 16.1 & 0.41 & $10.53_{-0.13}^{+0.22}$ & $-3.14_{-0.86}^{+2.69}$ \\
ASASSN-15ol & NGC 0745 & True & Ia & 0.01978 & 15.3 & 0.08 & $11.35_{-1.79}^{+0.01}$ & $<1.95$ \\
ASASSN-15om & LCRS B021111.4-453206 & True & Ia & 0.04172 & 16.4 & 0.06 & $10.56_{-0.43}^{+0.01}$ & $ 0.06_{-0.28}^{+0.03}$ \\
ASASSN-15on & SDSS J163636.15+553311.0 & True & Ia & 0.033 & 16.6 & 0.04 & $8.91_{-0.20}^{+0.10}$ & $-1.63_{-2.37}^{+0.01}$ \\
ASASSN-15os & GALEXASC J205408.07-551628.8 & True & Ia & 0.039 & 16.8 & 0.12 & $8.72_{-1.29}^{+0.57}$ & $-0.73_{-3.27}^{+0.11}$ \\
ASASSN-15ou & None & True & Ia & 0.049 & 16.8 & 0.03 & $<9.19$ & $-0.33_{-3.67}^{+2.39}$ \\
ASASSN-15ox & LSBG F418-058 & False & Ia & 0.0465 & 17.1 & 0.04 & $9.85_{-0.96}^{+0.43}$ & $ 0.20_{-4.20}^{+0.02}$ \\
ASASSN-15pe & CGCG 226-005 & True & Ia & 0.03793 & 16.3 & 0.11 & $11.72_{-0.08}^{+0.11}$ & $-1.37_{-2.63}^{+0.03}$ \\
ASASSN-15pf & ESO 241-G016 & True & Ia & 0.03935 & 16.9 & 0.03 & $10.82_{-0.07}^{+0.23}$ & $-1.97_{-2.03}^{+0.69}$ \\
ASASSN-15ph & 2MASX J22090684+0144384 & False & Ia & 0.041 & 17.4 & 0.14 & $10.80_{-0.25}^{+0.08}$ & $-0.42_{-0.34}^{+0.02}$ \\
ASASSN-15pl & ESO 545-G025 & True & Ia & 0.01617 & 15.0 & 0.06 & $8.84_{-0.02}^{+0.04}$ & $<-1.09$ \\
ASASSN-15pm & 2MASX J01383676-0440581 & True & Ia & 0.04878 & 16.8 & 0.09 & $10.67_{-0.10}^{+0.08}$ & $ 0.03_{-0.02}^{+0.00}$ \\
ASASSN-15pn & SDSS J040326.23-052930.6 & True & Ia & 0.03839 & 16.7 & 0.26 & $9.66_{-0.35}^{+0.25}$ & $-0.45_{-0.11}^{+0.06}$ \\
ASASSN-15pp & ESO 159-G023 & True & Ia & 0.02396 & 16.0 & 0.17 & $10.91_{-0.29}^{+0.25}$ & $ 0.08_{-4.08}^{+0.15}$ \\
ASASSN-15pr & 2MASX J23063962-1234238 & True & Ia & 0.03309 & 16.1 & 0.09 & $9.87_{-0.04}^{+0.04}$ & $-0.37_{-0.07}^{+0.05}$ \\
ASASSN-15ps & 2MASS J06144589-6613031 & True & Ia & 0.04 & 16.6 & 0.17 & $9.37_{-0.19}^{+0.33}$ & $-1.83_{-2.17}^{+0.29}$ \\
ASASSN-15py & SDSS J080519.59+225751.1 & False & Ia & 0.04474 & 17.2 & 0.14 & $10.14_{-0.42}^{+0.01}$ & $-0.82_{-0.21}^{+0.03}$ \\
ASASSN-15pz & ESO 357-G005 & True & Ia & 0.0149 & 14.2 & 0.05 & $7.28_{-0.34}^{+0.86}$ & $-0.29_{-0.94}^{+0.29}$ \\
ASASSN-15qc & UGC 00402 & True & Ia & 0.01765 & 15.4 & 0.07 & $10.24_{-0.11}^{+0.10}$ & $-1.36_{-2.64}^{+0.00}$ \\
ASASSN-15qy & 2MASX J00011837-3321048 & True & Ia & 0.03 & 16.8 & 0.04 & $8.99_{-0.27}^{+0.16}$ & $-0.27_{-3.73}^{+0.05}$ \\
ASASSN-15re & CGCG 448-007 & True & Ia & 0.03031 & 16.2 & 0.21 & $10.87_{-0.25}^{+0.08}$ & $-0.35_{-0.32}^{+0.02}$ \\
ASASSN-15rm & 2MFGC 05056 & True & Ia & 0.02077 & 16.9 & 0.47 & $10.43_{-0.14}^{+0.01}$ & $<-1.42$ \\
ASASSN-15rq & GALEXASC J000802.78-363348.1 & True & Ia & 0.024 & 15.4 & 0.04 & $8.43_{-0.67}^{+0.70}$ & $<-1.09$ \\
ASASSN-15rv & 2MASX J04225455-5230097 & True & Ia & 0.04 & 16.9 & 0.04 & $10.16_{-0.46}^{+0.14}$ & $-0.35_{-3.65}^{+0.05}$ \\
ASASSN-15rw & GALEXASC J021558.44+121415.2 & True & Ia & 0.0189 & 15.5 & 0.38 & $8.40_{-0.24}^{+0.24}$ & $-1.34_{-2.66}^{+0.09}$ \\
ASASSN-15sb & 2MFGC 04848 & True & Ia & 0.02271 & 16.3 & 0.90 & $10.94_{-0.25}^{+0.15}$ & $-1.25_{-2.75}^{+0.07}$ \\
ASASSN-15sf & GALEXASC J001127.51-062549.8 & True & Ia & 0.027 & 15.9 & 0.08 & $9.05_{-0.26}^{+0.25}$ & $-0.95_{-3.05}^{+0.16}$ \\
ASASSN-15sh & 2MASX J19320827-6226340 & True & Ia-91T & 0.031 & 16.1 & 0.16 & $10.59_{-0.45}^{+0.14}$ & $ 0.08_{-4.08}^{+0.06}$ \\
ASASSN-15so & NGC 3583 & True & Ia & 0.00713 & 13.8 & 0.04 & $10.85_{-0.18}^{+0.05}$ & $-1.54_{-2.46}^{+0.60}$ \\
ASASSN-15ss & MCG -02-16-004 & False & Ia & 0.03556 & 17.1 & 0.64 & $11.35_{-0.10}^{+0.01}$ & $<-0.50$ \\
ASASSN-15sx & ESO 472-G018 & True & Ia & 0.03481 & 16.3 & 0.06 & $10.87_{-0.08}^{+0.08}$ & $-0.42_{-0.02}^{+0.01}$ \\
ASASSN-15tb & LCRS B123822.1-062502 & True & Ia & 0.02461 & 16.2 & 0.07 & $10.06_{-0.05}^{+0.11}$ & $-0.38_{-0.37}^{+0.26}$ \\
ASASSN-15tf & 2MASX J21291986-2305268 & True & Ia & 0.03529 & 16.7 & 0.13 & $9.95_{-0.02}^{+0.13}$ & $-0.06_{-0.05}^{+0.16}$ \\
ASASSN-15tg & GALEXASC J002041.66+251341.1 & True & Ia-91T & 0.03561 & 16.4 & 0.08 & $10.19_{-0.08}^{+0.01}$ & $-0.31_{0.00}^{+0.08}$ \\
ASASSN-15ti & 2MASX J03051061+3754003 & True & Ia & 0.016 & 15.8 & 0.41 & $8.72_{-0.04}^{+0.04}$ & $-3.18_{-0.82}^{+1.31}$ \\
ASASSN-15tj & SDSS J075527.63+520911.1 & True & Ia & 0.02227 & 15.6 & 0.13 & $8.85_{-0.47}^{+0.45}$ & $-0.69_{-3.31}^{+0.36}$ \\
ASASSN-15tn & CGCG 496-051 & True & Ia & 0.023 & 16.0 & 0.17 & $9.77_{-0.16}^{+0.16}$ & $-0.26_{-0.18}^{+0.09}$ \\
ASASSN-15ts & 2MASX J03344211-2050502 & False & Ia & 0.05998 & 17.2 & 0.08 & $11.35_{-0.24}^{+0.15}$ & $-1.64_{-2.36}^{+2.07}$ \\
ASASSN-15tt & 2MASXi J0638012-373927 & True & Ia & 0.034 & 16.8 & 0.34 & $9.34_{-1.21}^{+0.58}$ & $<0.98$ \\
ASASSN-15tz & UGC 02164 & True & Ia & 0.02286 & 16.9 & 0.45 & $10.75_{-0.19}^{+0.14}$ & $<-0.44$ \\
ASASSN-15ub & CGCG 314-006 & True & Ia & 0.03205 & 16.4 & 0.04 & $10.86_{-0.32}^{+0.01}$ & $-0.10_{-0.20}^{+0.02}$ \\
ASASSN-15uh & KUG 0925+693 & True & Ia-91T & 0.0135 & 15.3 & 0.41 & $8.67_{-0.03}^{+0.08}$ & $-2.26_{-1.74}^{+0.95}$ \\
ASASSN-15uk & SDSS J144816.71+171235.6 & True & Ia & 0.037 & 16.6 & 0.07 & $7.82_{-0.21}^{+0.19}$ & $-1.41_{-0.27}^{+0.11}$ \\
ASASSN-15ul & KUG 1457+066 & True & Ia & 0.02979 & 16.8 & 0.09 & $10.10_{-0.06}^{+0.03}$ & $<-1.82$ \\
ASASSN-15up & GALEXASC J042539.92-494621.0 & True & Ia & 0.038 & 16.4 & 0.03 & $9.57_{-0.70}^{+0.62}$ & $-0.78_{-3.22}^{+0.31}$ \\
ASASSN-15uq & ALLWISE J070957.84-650756.9 & True & Ia & 0.02 & 16.0 & 0.31 & $8.30_{-0.82}^{+0.56}$ & $-2.24_{-1.76}^{+0.22}$ \\
ASASSN-15us & NGC 7213 & False & Ia-06bt & 0.00584 & 14.0 & 0.04 & $10.42_{-0.85}^{+0.92}$ & $<3.24$ \\
ASASSN-15uu & VV 790a & True & Ia & 0.0268 & 16.5 & 0.19 & $9.85_{-0.03}^{+0.04}$ & $<-0.08$ \\
ASASSN-15uv & 2MASX J08270817+2748382 & True & Ia & 0.02033 & 16.1 & 0.09 & $9.67_{-0.16}^{+0.31}$ & $-1.43_{-2.57}^{+0.86}$ \\
ASASSN-15uw & 2MASX J02353437-0603496 & True & Ia & 0.03081 & 16.8 & 0.07 & $10.85_{-0.16}^{+0.08}$ & $-1.44_{-0.03}^{+0.03}$ \\
ASASSN-16aa & UGC 04251 & True & Ia & 0.01738 & 16.4 & 0.12 & $10.56_{-0.10}^{+0.22}$ & $-3.06_{-0.94}^{+2.75}$ \\
ASASSN-16ad & KUG 0136+335 & True & Ia & 0.01614 & 15.1 & 0.13 & $8.72_{-0.01}^{+0.03}$ & $<-2.86$ \\
ASASSN-16ah & Uncatalogued & True & Ia & 0.0285 & 16.7 & 0.72 & $9.51_{-0.30}^{+0.16}$ & $-0.84_{-3.16}^{+0.41}$ \\
ASASSN-16aj & NGC 1562 & True & Ia & 0.03075 & 16.8 & 0.09 & $11.13_{-0.07}^{+0.03}$ & $-1.26_{-0.77}^{+0.03}$ \\
ASASSN-16ar & 2MASX J04283087-1739233 & True & Ia & 0.03108 & 16.5 & 0.10 & $10.87_{-0.25}^{+0.16}$ & $-2.12_{-1.88}^{+2.07}$ \\
ASASSN-16av & NGC 3926 NED02 & True & Ia & 0.02567 & 16.0 & 0.07 & $11.02_{-0.12}^{+0.21}$ & $-1.77_{-2.23}^{+0.73}$ \\
ASASSN-16aw & ESO 306-G 016 & True & Ia & 0.03728 & 16.3 & 0.09 & $10.08_{-0.38}^{+1.40}$ & $-0.70_{-3.30}^{+3.60}$ \\
ASASSN-16ax & 2MASX J01312331+6019128 & True & Ia & 0.0187 & 16.0 & 1.51 & $10.62_{-0.32}^{+0.08}$ & $-0.08_{-3.92}^{+0.26}$ \\
ASASSN-16ay & UGC 03738 & True & Ia & 0.02834 & 16.3 & 0.19 & $10.81_{-0.32}^{+0.09}$ & $ 0.11_{-4.11}^{+0.26}$ \\
ASASSN-16az & 2MASX J11303364-4233359 & True & Ia & 0.03407 & 16.4 & 0.23 & $10.68_{-1.74}^{+0.04}$ & $-1.71_{-2.29}^{+3.71}$ \\
ASASSN-16bb & SDSS J140557.36+435257.2 & True & Ia-91T & 0.03375 & 16.2 & 0.02 & $9.18_{-0.25}^{+0.16}$ & $-0.56_{-3.44}^{+0.10}$ \\
ASASSN-16bc & 2MASX J12052488-2123572 & True & Ia & 0.03194 & 16.4 & 0.15 & $10.68_{-0.15}^{+0.16}$ & $-0.24_{-0.04}^{+0.04}$ \\
ASASSN-16bg & 2MASX J12592491+2744198 & True & Ia & 0.02022 & 16.8 & 0.02 & $10.25_{-0.22}^{+0.09}$ & $-2.74_{-1.26}^{+0.75}$ \\
ASASSN-16bl & 2MASX J11422674-3654256 & True & Ia & 0.02955 & 16.8 & 0.32 & $10.97_{-1.78}^{+0.01}$ & $<2.24$ \\
ASASSN-16bn & 2MASX J03103162+0416184 & True & Ia & 0.02317 & 15.7 & 0.47 & $10.73_{-0.09}^{+0.06}$ & $<-3.21$ \\
ASASSN-16bp & CGCG 336-041 & True & Ia & 0.03419 & 16.0 & 0.06 & $10.93_{-0.16}^{+0.15}$ & $-0.09_{-0.05}^{+0.20}$ \\
ASASSN-16bq & IC 0986 & True & Ia & 0.0204 & 15.4 & 0.10 & $10.93_{-0.15}^{+0.14}$ & $-2.06_{-1.94}^{+0.71}$ \\
ASASSN-16br & 2MASX J15453055-1309057 & True & Ia & 0.02852 & 16.5 & 0.44 & $10.22_{-0.07}^{+0.23}$ & $-0.35_{-0.05}^{+0.10}$ \\
ASASSN-16bv & LCRS B014209.4-420839 & True & Ia-91T & 0.0273 & 15.9 & 0.04 & $8.62_{-1.53}^{+0.50}$ & $-0.68_{-3.32}^{+0.10}$ \\
ASASSN-16bx & CGCG 280-023 & True & Ia & 0.02662 & 16.3 & 0.34 & $10.91_{-0.31}^{+0.07}$ & $ 0.05_{-0.20}^{+0.05}$ \\
ASASSN-16ch & MSPM 00984 & False & Ia & 0.02644 & 17.1 & 0.07 & $10.11_{-0.09}^{+0.16}$ & $-0.82_{-0.03}^{+0.02}$ \\
ASASSN-16ci & NGC 1272 & True & Ia & 0.01273 & 16.4 & 0.44 & $10.48_{-0.01}^{+0.10}$ & $-0.83_{-0.37}^{+0.00}$ \\
ASASSN-16cm & 2MASX J15192684-0055256 & True & Ia & 0.02972 & 16.2 & 0.17 & $10.08_{-0.09}^{+0.25}$ & $-0.65_{-0.01}^{+0.22}$ \\
ASASSN-16cn & ESO 579-G018 & True & Ia & 0.02713 & 16.7 & 0.34 & $11.19_{-0.08}^{+0.07}$ & $-0.03_{-0.03}^{+0.02}$ \\
ASASSN-16cs & KUG 0647+311 & True & Ia & 0.0113 & 15.8 & 0.36 & $8.83_{-0.01}^{+0.06}$ & $-1.43_{-0.03}^{+0.27}$ \\
ASASSN-16ct & SDSS J151354.30+044525.7 & True & Ia & 0.04193 & 16.8 & 0.14 & $9.33_{-0.14}^{+0.49}$ & $-1.67_{-2.33}^{+0.92}$ \\
ASASSN-16cu & IC 4723 & True & Ia & 0.01113 & 15.8 & 0.26 & $9.04_{-0.50}^{+1.28}$ & $-2.86_{-1.14}^{+4.83}$ \\
ASASSN-16cy & CGCG 295-010 & True & Ia & 0.03481 & 16.6 & 0.05 & $11.22_{-0.01}^{+0.01}$ & $-0.09_{-0.01}^{+0.00}$ \\
ASASSN-16dn & GALEXASC J104848.62-201544.1 & True & Ia & 0.012 & 14.7 & 0.10 & $7.95_{-0.41}^{+0.16}$ & $-1.07_{-2.93}^{+0.06}$ \\
ASASSN-16dp & SDSS J145942.12+040518.1 & True & Ia & 0.03264 & 16.4 & 0.13 & $8.99_{-0.23}^{+0.33}$ & $-1.01_{-2.99}^{+0.23}$ \\
ASASSN-16dw & 2MASX J13300119-2758297 & True & Ia & 0.03466 & 16.3 & 0.14 & $10.44_{-0.13}^{+0.27}$ & $<0.14$ \\
ASASSN-16dx & APMUKS B032028.93-441621.0 & True & Ia & 0.02997 & 16.1 & 0.04 & $8.05_{-0.17}^{+0.60}$ & $-2.74_{-1.26}^{+2.62}$ \\
ASASSN-16ec & 2MASX J13031054-2159149 & True & Ia & 0.02377 & 16.8 & 0.28 & $10.27_{-0.16}^{+0.15}$ & $-0.40_{-0.03}^{+0.12}$ \\
ASASSN-16ej & UGC 11409 & True & Ia & 0.02802 & 16.6 & 0.48 & $10.94_{-0.20}^{+0.10}$ & $<-0.62$ \\
ASASSN-16em & GALEXASC J133213.24+844042.7 & True & Ia & 0.0234 & 15.8 & 0.37 & $8.83_{-0.11}^{+0.01}$ & $-1.52_{-2.48}^{+0.03}$ \\
ASASSN-16eo & ALLWISE J054312.80+413115.5 & True & Ia & 0.037 & 16.3 & 0.12 & $7.97_{-0.22}^{+1.53}$ & $ 0.42_{-4.42}^{+1.95}$ \\
ASASSN-16eq & UGC 11898 & True & Ia & 0.01431 & 15.7 & 0.87 & $10.82_{-0.28}^{+0.04}$ & $-0.49_{-3.51}^{+0.02}$ \\
ASASSN-16es & SDSS J115054.45+021828.1 & True & Ia & 0.029 & 16.5 & 0.07 & $8.69_{-0.24}^{+0.16}$ & $-1.32_{-2.68}^{+0.14}$ \\
ASASSN-16et & 2MASX J10200192+5627397 & True & Ia & 0.02492 & 16.7 & 0.08 & $9.20_{-0.08}^{+0.07}$ & $-1.06_{-0.94}^{+0.27}$ \\
ASASSN-16ex & SDSS J171023.63+262350.3 & False & Ia-09dc & 0.0418 & 16.6 & 0.09 & $9.07_{-0.25}^{+0.55}$ & $-0.67_{-3.33}^{+0.24}$ \\
ASASSN-16fa & UGC 06434 & True & Ia & 0.03433 & 16.5 & 0.07 & $11.11_{-0.01}^{+0.01}$ & $-0.20_{-0.01}^{+0.00}$ \\
ASASSN-16fc & SDSS J153151.40+372445.8 & True & Ia & 0.0298 & 16.2 & 0.05 & $9.08_{-0.33}^{+0.46}$ & $-0.65_{-3.35}^{+0.13}$ \\
ASASSN-16fd & 2MASX J22212881-2215454 & True & Ia & 0.02391 & 16.2 & 0.09 & $10.48_{-0.07}^{+0.20}$ & $-3.15_{-0.85}^{+1.74}$ \\
ASASSN-16fe & APMUKS B225823.09-373218.0 & True & Ia & 0.0386 & 17.0 & 0.04 & $9.35_{-0.84}^{+0.60}$ & $-0.39_{-3.61}^{+0.13}$ \\
ASASSN-16fg & 2MASX J00051603-1629348 & True & Ia & 0.02489 & 16.2 & 0.07 & $9.82_{-0.15}^{+0.32}$ & $-0.21_{-0.05}^{+0.14}$ \\
ASASSN-16fh & 2MASXi J0002057-265846 & True & Ia & 0.0335 & 16.1 & 0.04 & $9.07_{-0.01}^{+0.04}$ & $<-1.84$ \\
ASASSN-16fj & IC 1289 & True & Ia & 0.01831 & 15.8 & 0.17 & $10.06_{-0.17}^{+0.23}$ & $-0.25_{-0.16}^{+0.08}$ \\
ASASSN-16fl & 2MASX J10065350-1543022 & True & Ia & 0.02944 & 16.0 & 0.16 & $10.83_{-0.10}^{+0.11}$ & $<-2.03$ \\
ASASSN-16fn & Uncatalogued & True & Ia & 0.0212 & 15.3 & 0.16 & $8.65_{-1.05}^{+0.23}$ & $<-0.32$ \\
ASASSN-16fo & 2MASX J13323577-0516218 & True & Ia-91T & 0.02961 & 16.1 & 0.09 & $10.29_{-0.09}^{+0.26}$ & $-2.50_{-1.50}^{+0.73}$ \\
ASASSN-16fs & UGC 09523 & True & Ia & 0.02909 & 16.6 & 0.09 & $11.46_{-0.08}^{+0.03}$ & $-0.93_{-0.76}^{+0.02}$ \\
ASASSN-16fv & IC 4705 & True & Ia & 0.01197 & 14.8 & 0.27 & $10.68_{-0.35}^{+0.14}$ & $-0.91_{-3.09}^{+0.02}$ \\
ASASSN-16fx & GALEXASC J020044.56-461644.0 & True & Ia & 0.037 & 16.6 & 0.07 & $8.64_{-1.56}^{+0.41}$ & $-0.41_{-3.59}^{+0.16}$ \\
ASASSN-16gf & CGCG 104-069 & True & Ia & 0.03061 & 16.7 & 0.10 & $10.94_{-0.17}^{+0.11}$ & $<-1.98$ \\
ASASSN-16gm & GALEXASC J200348.67-601528.7 & True & Ia & 0.036 & 16.3 & 0.11 & $9.17_{-0.73}^{+0.68}$ & $<-0.21$ \\
ASASSN-16gp & WKK 2066 & True & Ia & 0.016 & 16.8 & 1.18 & $8.31_{-0.80}^{+0.95}$ & $-2.04_{-1.96}^{+4.18}$ \\
ASASSN-16gq & ESO 446-G023 & True & Ia & 0.02314 & 15.7 & 0.20 & $10.66_{-0.26}^{+0.24}$ & $-0.63_{-3.37}^{+0.21}$ \\
ASASSN-16gv & CGCG 503-021 & True & Ia & 0.03733 & 16.9 & 0.12 & $10.42_{-0.09}^{+0.24}$ & $ 0.13_{-0.03}^{+0.16}$ \\
ASASSN-16gz & APMUKS B043218.28-211910.3 & True & Ia & 0.032 & 16.5 & 0.10 & $9.23_{-1.20}^{+0.52}$ & $-2.18_{-1.82}^{+2.18}$ \\
ASASSN-16ha & FAIRALL 0673 & True & Ia & 0.02253 & 16.2 & 0.03 & $10.58_{-0.38}^{+0.15}$ & $-0.91_{-3.09}^{+0.01}$ \\
ASASSN-16hc & 2MASX J13590394+3308172 & True & Ia-91T & 0.05097 & 16.5 & 0.04 & $11.17_{-0.10}^{+0.08}$ & $<-1.78$ \\
ASASSN-16hd & GALEXASC J015051.89+223348.8 & True & Ia & 0.029 & 16.5 & 0.25 & $8.79_{-0.20}^{+0.15}$ & $-0.86_{-3.14}^{+0.16}$ \\
ASASSN-16hh & MCG +03-06-031 & True & Ia & 0.032 & 16.5 & 0.35 & $9.57_{-0.04}^{+0.14}$ & $<-0.19$ \\
ASASSN-16hp & ESO 509-IG064 & True & Ia & 0.00866 & 14.2 & 0.35 & $8.57_{-0.05}^{+0.01}$ & $-3.75_{-0.25}^{+1.75}$ \\
ASASSN-16hr & 2MASX J22253147+3859010 & True & Ia & 0.024 & 16.9 & 0.34 & $9.17_{-0.06}^{+0.02}$ & $-1.85_{-2.15}^{+0.00}$ \\
ASASSN-16hw & GALEXASC J215327.92-342420.8 & True & Ia & 0.012 & 14.6 & 0.07 & $8.06_{-0.16}^{+0.21}$ & $-1.31_{-2.69}^{+0.06}$ \\
ASASSN-16hz & 2MASX J23154564-0120135 & True & Ia & 0.02531 & 16.0 & 0.10 & $10.44_{-0.26}^{+0.15}$ & $-0.68_{-0.34}^{+0.02}$ \\
ASASSN-16ic & GALEXASC J011415.49-162456.4 & True & Ia & 0.047 & 16.7 & 0.06 & $8.84_{-0.41}^{+0.34}$ & $-0.74_{-0.64}^{+0.11}$ \\
ASASSN-16ie & 2MASXi J1604144+164124 & False & Ia & 0.04452 & 17.1 & 0.10 & $10.00_{-0.20}^{+0.46}$ & $<-0.31$ \\
ASASSN-16if & AM 0557-522 NED03 & True & Ia & 0.03202 & 16.2 & 0.17 & $11.44_{-1.69}^{+0.10}$ & $<2.81$ \\
ASASSN-16io & 2MASX J18400114+5413042 & True & Ia & 0.032 & 16.7 & 0.10 & $9.84_{-0.31}^{+0.01}$ & $-0.86_{-0.11}^{+0.05}$ \\
ASASSN-16ip & ESO 479-G007 & True & Ia & 0.012 & 15.1 & 0.05 & $9.84_{-0.03}^{+0.24}$ & $<-2.21$ \\
ASASSN-16iq & ESO 471-G041 & True & Ia & 0.0286 & 15.9 & 0.05 & $9.57_{-0.50}^{+1.28}$ & $-2.33_{-1.67}^{+4.77}$ \\
ASASSN-16jc & NGC 6942 & True & Ia & 0.01091 & 14.0 & 0.13 & $10.98_{-0.24}^{+0.19}$ & $-2.94_{-1.06}^{+1.67}$ \\
ASASSN-16je & 2MASX J17055033+6950555 & True & Ia & 0.0394 & 16.5 & 0.09 & $9.98_{-0.08}^{+0.31}$ & $-0.21_{-0.04}^{+0.18}$ \\
ASASSN-16jf & UGCA 430 & True & Ia & 0.01144 & 14.9 & 0.06 & $7.32_{-0.07}^{+0.08}$ & $ 0.10_{-0.49}^{+0.10}$ \\
ASASSN-16jh & 2dFGRS S501Z101 & True & Ia & 0.0389 & 16.6 & 0.04 & $8.97_{-1.51}^{+0.40}$ & $-0.13_{-3.87}^{+0.07}$ \\
ASASSN-16jj & GALEXASC J234711.93+100501.3 & True & Ia & 0.025 & 16.6 & 0.17 & $9.20_{-0.17}^{+0.43}$ & $-0.90_{-0.24}^{+0.25}$ \\
ASASSN-16jq & CGMW 2-2125 & True & Ia & 0.024 & 16.1 & 0.59 & $9.10_{-0.16}^{+0.36}$ & $<-0.34$ \\
ASASSN-16jw & IC 1780 & True & Ia & 0.03476 & 16.9 & 0.15 & $10.80_{-0.17}^{+0.15}$ & $ 0.03_{-0.23}^{+0.02}$ \\
ASASSN-16ke & AGC 331536 & True & Ia-91T & 0.028 & 16.2 & 0.20 & $8.60_{-0.11}^{+0.28}$ & $-1.75_{-0.98}^{+0.43}$ \\
ASASSN-16kk & LSBG F156-039 & True & Ia-91T & 0.04371 & 16.7 & 0.04 & $11.27_{-0.21}^{+0.11}$ & $-1.72_{-2.28}^{+0.02}$ \\
ASASSN-16km & ESO 197-G010 & True & Ia & 0.02059 & 15.9 & 0.06 & $11.64_{-0.15}^{+0.01}$ & $<-1.60$ \\
ASASSN-16kv & 2MASX J05073951-1932539 & True & Ia & 0.03043 & 16.6 & 0.11 & $10.47_{-0.18}^{+0.15}$ & $-1.53_{-2.47}^{+0.03}$ \\
ASASSN-16kw & 2MASX J05080487-4141151 & True & Ia & 0.04453 & 16.6 & 0.06 & $10.02_{-0.12}^{+0.50}$ & $<0.25$ \\
ASASSN-16kz & ESO 555-G029 & True & Ia & 0.00965 & 14.4 & 0.19 & $9.79_{-0.41}^{+0.21}$ & $-0.88_{-0.23}^{+0.09}$ \\
ASASSN-16la & 2MASXi J0229172+180515 & True & Ia & 0.0164 & 15.2 & 0.57 & $9.11_{-0.17}^{+0.38}$ & $<-0.38$ \\
ASASSN-16lc & GALEXASC J192901.47-515813.5 & True & Ia & 0.0161 & 15.6 & 0.14 & $7.94_{-1.12}^{+0.40}$ & $-1.86_{-2.14}^{+0.04}$ \\
ASASSN-16lg & ARK 530 & True & Ia & 0.02117 & 15.9 & 0.21 & $11.03_{-0.30}^{+0.09}$ & $ 0.07_{-4.07}^{+0.22}$ \\
ASASSN-16lm & 2MASX J09033461+4142367 & False & Ia & 0.04048 & 17.3 & 0.05 & $9.98_{-0.03}^{+0.06}$ & $<-0.68$ \\
ASASSN-16lx & IC 0607 & True & Ia & 0.0186 & 15.4 & 0.12 & $10.06_{-0.12}^{+0.05}$ & $-0.29_{-3.71}^{+0.00}$ \\
ASASSN-16lz & ALLWISE J060551.48-504652.2 & True & Ia & 0.04 & 16.5 & 0.12 & $8.29_{-0.74}^{+0.71}$ & $<-1.10$ \\
ASASSN-16mc & ESO 233-IG014 & True & Ia & 0.01891 & 16.0 & 0.12 & $10.45_{-0.45}^{+0.07}$ & $-0.15_{-3.85}^{+0.04}$ \\
ASASSN-16mj & SDSS J092119.07+170159.5 & True & Ia-91T & 0.028 & 16.4 & 0.08 & $8.49_{-0.17}^{+0.26}$ & $-1.34_{-0.43}^{+0.10}$ \\
ASASSN-16mt & 2MASX J01004149-0026406 & False & Ia & 0.0436 & 17.1 & 0.10 & $10.44_{-0.12}^{+0.15}$ & $-2.23_{-1.77}^{+0.76}$ \\
ASASSN-16mv & ESO 563-G035 & True & Ia & 0.01856 & 16.4 & 0.47 & $11.02_{-0.14}^{+0.01}$ & $-0.76_{0.00}^{+0.05}$ \\
ASASSN-16na & 2MASX J04091030+2126244 & True & Ia-91T & 0.02119 & 16.6 & 1.30 & $10.90_{-0.22}^{+0.17}$ & $<0.20$ \\
ASASSN-16nm & 2MASX J21255058-3724071 & True & Ia & 0.03069 & 16.3 & 0.22 & $10.09_{-0.04}^{+0.50}$ & $<-0.01$ \\
ASASSN-16nn & APMUKS B214820.71-555825.5 & True & Ia & 0.032 & 16.6 & 0.06 & $8.81_{-1.43}^{+0.60}$ & $-0.73_{-3.27}^{+0.10}$ \\
ASASSN-16no & IC 0493 & True & Ia & 0.02071 & 16.4 & 0.11 & $10.59_{-0.15}^{+0.15}$ & $-0.08_{-0.05}^{+0.12}$ \\
ASASSN-16np & SDSS J123643.42+260647.1 & True & Ia & 0.02084 & 15.8 & 0.04 & $8.73_{-0.01}^{+0.06}$ & $-1.27_{-0.27}^{+0.00}$ \\
ASASSN-16nt & CGCG 068-029 & True & Ia & 0.03422 & 16.9 & 0.10 & $10.65_{-0.12}^{+0.18}$ & $-2.02_{-1.98}^{+0.74}$ \\
ASASSN-16nv & 2MASX J05482726-2319189 & True & Ia & 0.04607 & 17.0 & 0.08 & $9.87_{-0.16}^{+0.18}$ & $ 0.45_{-4.45}^{+0.14}$ \\
ASASSN-16of & ESO 087-IG 041 & True & Ia & 0.03021 & 16.6 & 0.21 & $10.16_{-0.70}^{+0.64}$ & $-2.93_{-1.07}^{+2.69}$ \\
ASASSN-16oj & SDSS J053208.29-020407.9 & True & Ia & 0.029 & 16.9 & 1.59 & $9.92_{-0.08}^{+0.06}$ & $<-0.89$ \\
ASASSN-16ok & GALEXASC J005328.92-362154.1 & True & Ia & 0.037 & 16.9 & 0.04 & $8.09_{-1.47}^{+0.43}$ & $-1.10_{-2.90}^{+0.08}$ \\
ASASSN-16ol & GALEXASC J011003.70-702046.4 & True & Ia & 0.03 & 15.6 & 0.07 & $8.66_{-1.47}^{+0.61}$ & $<-0.52$ \\
ASASSN-16om & AM 2329-410 & True & Ia & 0.04531 & 17.0 & 0.05 & $11.21_{-0.30}^{+0.01}$ & $-1.18_{-2.82}^{+0.07}$ \\
ASASSN-16oo & 2MASX J01411858-0012382 & True & Ia & 0.05546 & 16.6 & 0.08 & $10.13_{-0.08}^{+0.15}$ & $ 0.13_{0.00}^{+0.16}$ \\
ASASSN-16oq & AM 1228-353 NED02 & True & Ia & 0.01992 & 15.2 & 0.17 & $10.39_{-0.52}^{+0.01}$ & $-0.31_{-3.69}^{+0.06}$ \\
ASASSN-16ov & NPM1G +01.0158 & True & Ia & 0.02834 & 16.6 & 0.16 & $10.25_{-0.32}^{+0.28}$ & $-1.24_{-2.76}^{+1.04}$ \\
ASASSN-16oz & GALEXASC J090013.19-133803.5 & True & Ia-91T & 0.031 & 16.2 & 0.15 & $8.06_{-0.10}^{+0.06}$ & $<-1.50$ \\
ASASSN-16pa & ALLWISE J003315.83-842917.8 & True & Ia & 0.034 & 16.4 & 0.45 & $9.03_{-0.74}^{+0.63}$ & $-2.19_{-1.81}^{+1.20}$ \\
ASASSN-16pb & CGCG 058-057 & True & Ia & 0.02978 & 16.3 & 0.08 & $9.79_{-0.25}^{+0.51}$ & $-0.30_{-3.70}^{+0.24}$ \\
ASASSN-16pd & PGC 241921 & True & Ia & 0.0215 & 15.8 & 0.47 & $8.57_{-0.67}^{+0.71}$ & $<-0.82$ \\
ASASSN-16pj & GALEXASC J232303.16-361420.6 & True & Ia & 0.0371 & 16.6 & 0.05 & $9.02_{-0.78}^{+0.66}$ & $-0.79_{-3.21}^{+0.26}$ \\
ASASSN-16pk & SDSS J122739.65+403648.9 & True & Ia & 0.02328 & 16.4 & 0.04 & $8.89_{-0.17}^{+0.43}$ & $-0.84_{-0.25}^{+0.10}$ \\
ASASSN-16pl & IC 0988 & True & Ia & 0.02693 & 16.4 & 0.09 & $11.07_{-0.28}^{+0.07}$ & $-0.52_{-0.50}^{+0.02}$ \\
2014bz & 2MASX J13560316-4334319 & False & Ia & 0.025 & 16.9 & 0.24 & $9.48_{-0.76}^{+1.02}$ & $-1.65_{-2.35}^{+3.80}$ \\
2014ba & NGC 7410 & False & Ia-91bg & 0.0058 & 14.7 & 0.03 & $11.01_{-0.80}^{+0.10}$ & $-0.77_{-3.23}^{+0.16}$ \\
2014bb & NGC 5214 & False & Ia & 0.026942 & 15.9 & 0.02 & $10.85_{-0.16}^{+0.24}$ & $ 0.54_{-0.16}^{+0.11}$ \\
PSN J15024996+4847062 & 2MASX J15024995+4847010 & False & Ia & 0.026138 & 16.1 & 0.05 & $9.78_{-0.27}^{+0.27}$ & $-1.04_{-2.96}^{+0.52}$ \\
2014bg & UGC 09396 & False & Ia & 0.03604 & 16.1 & 0.09 & $11.40_{-0.16}^{+0.08}$ & $ 0.28_{-0.02}^{+0.03}$ \\
iPTF14bdn & UGC 08503 & True & Ia-91T & 0.01558 & 14.7 & 0.03 & $8.63_{-0.19}^{+0.15}$ & $-1.51_{-2.49}^{+0.96}$ \\
2014ch & SDSS J155830.96+125157.5 & False & Ia & 0.044 & 16.5 & 0.11 & $8.29_{-0.07}^{+0.18}$ & $<-1.24$ \\
2014bs & NGC 5270 & False & Ia & 0.02352 & 16.9 & 0.08 & $10.83_{-0.16}^{+0.15}$ & $ 0.32_{-0.04}^{+0.11}$ \\
LSQ14cnm & 2MASX J16052452+0113000 & True & Ia & 0.0326 & 16.5 & 0.35 & $9.63_{-0.07}^{+0.17}$ & $-0.20_{-0.17}^{+0.12}$ \\
2014bv & NGC 4386 & True & Ia & 0.005594 & 14.1 & 0.11 & $10.76_{-0.14}^{+0.01}$ & $<-0.66$ \\
CSS140628:164427+285658 & SDSS J164427.41+285656.8 & False & Ia & 0.053 & 17.0 & 0.10 & $8.37_{-0.09}^{+0.16}$ & $-1.86_{-2.14}^{+0.86}$ \\
2014ck & UGC 12182 & False & Ia-pec & 0.00497 & 16.2 & 1.26 & $9.05_{-0.41}^{+0.36}$ & $-0.87_{-3.13}^{+0.16}$ \\
2014by & UGC 09267 & True & Ia & 0.024794 & 16.4 & 0.08 & $10.49_{-0.14}^{+0.24}$ & $-0.15_{-0.40}^{+0.21}$ \\
2014bx & NGC 6808 & True & Ia & 0.017 & 15.8 & 0.22 & $11.30_{-0.42}^{+0.13}$ & $ 0.17_{-4.17}^{+0.03}$ \\
PSN J01340299-0104458 & UGC 01120 & True & Ia & 0.015561 & 16.3 & 0.10 & $10.64_{-0.25}^{+0.08}$ & $-0.57_{-0.03}^{+0.04}$ \\
2014da & NGC 0128 & False & Ia-91bg & 0.0141 & 15.4 & 0.08 & $11.48_{-0.12}^{+0.11}$ & $-2.62_{-1.38}^{+1.03}$ \\
PSN J02451711+4213503 & GALEXASC J024517.55+421344.1 & False & Ia-91T & 0.03 & 16.8 & 0.25 & $9.23_{-0.29}^{+0.52}$ & $-0.51_{-3.49}^{+0.17}$ \\
2014cc & NGC 2255 & True & Ia & 0.02 & 15.9 & 0.29 & $10.28_{-0.11}^{+0.51}$ & $<0.55$ \\
2014cd & NGC 1578 & False & Ia & 0.020608 & 15.8 & 0.04 & $11.17_{-0.42}^{+0.13}$ & $ 0.05_{-4.05}^{+0.03}$ \\
2014cj & ESO 087-G031 & False & Ia & 0.02 & 17.0 & 0.16 & $10.90_{-0.44}^{+0.01}$ & $-0.88_{-3.12}^{+0.05}$ \\
MASTER OT J162412.26+091303.0 & CGCG 080-023 & False & Ia & 0.04 & 16.6 & 0.16 & $10.47_{-0.18}^{+0.08}$ & $ 0.18_{-0.27}^{+0.02}$ \\
2014cb & VV 322b & False & Ia & 0.03 & 16.4 & 0.21 & $10.87_{-0.01}^{+0.01}$ & $-0.09_{-0.01}^{+0.00}$ \\
2014dd & UGC 02504 & False & Ia & 0.0235 & 16.4 & 0.61 & $11.32_{-0.14}^{+0.01}$ & $<-0.10$ \\
2014dg & UGC 02855 & False & Ia & 0.004 & 13.9 & 2.00 & $10.59_{-0.28}^{+0.26}$ & $ 0.67_{-4.67}^{+0.08}$ \\
2014dk & DDG2014 J002812.09+070940.1 & False & Ia & 0.038 & 16.9 & 0.08 & $8.05_{-0.09}^{+0.47}$ & $-2.05_{-1.95}^{+0.58}$ \\
2014dm & NGC 1516A & False & Ia & 0.033 & 16.5 & 0.13 & $11.32_{-0.01}^{+0.01}$ & $<-4.00$ \\
PSN J09084248+4448132 & UGC 04798 & False & Ia & 0.0268 & 15.8 & 0.05 & $10.67_{-0.24}^{+0.08}$ & $ 0.07_{-0.15}^{+0.12}$ \\
2014dt & M61 & False & Ia-pec & 0.0052 & 13.2 & 0.06 & $11.63_{-0.48}^{+0.07}$ & $ 0.41_{-0.76}^{+0.03}$ \\
2014du & UGC 01899 & False & Ia & 0.0324 & 16.9 & 0.30 & $11.49_{-0.08}^{+0.01}$ & $-0.29_{0.00}^{+0.03}$ \\
MASTER OT J011330.63+493634.9 & UGC 00766 & False & Ia & 0.018283 & 15.8 & 0.42 & $9.48_{-0.15}^{+0.34}$ & $-0.55_{-0.17}^{+0.21}$ \\
PSN J04561965-1548027 & IC 2104 & True & Ia-91bg & 0.018393 & 16.1 & 0.21 & $10.78_{-0.04}^{+0.33}$ & $<-0.65$ \\
2014eg & ESO 154-G010 & True & Ia-91T & 0.0186 & 15.4 & 0.08 & $11.47_{-0.53}^{+0.07}$ & $-0.21_{-3.79}^{+0.03}$ \\
2014dv & NGC 2501 & False & Ia & 0.007 & 16.0 & 0.28 & $10.55_{-0.31}^{+0.01}$ & $-0.76_{-0.32}^{+0.04}$ \\
PSN J10292799+2200468 & UGC 05691 & False & Ia & 0.018393 & 16.1 & 0.07 & $10.44_{-0.08}^{+0.01}$ & $-0.53_{0.00}^{+0.03}$ \\
PSN J04173792+3617317 & UGC 03000 & False & Ia & 0.0188 & 16.0 & 1.27 & $11.12_{-0.15}^{+0.01}$ & $-0.20_{0.00}^{+0.06}$ \\
2014ea & UGC 05912 & True & Ia & 0.021 & 15.7 & 0.10 & $10.40_{-0.26}^{+0.39}$ & $ 0.37_{-0.82}^{+0.15}$ \\
MASTER OT J062509.46+283255.1 & UGC 03462 & False & Ia & 0.029 & 17.0 & 0.73 & $10.94_{-0.45}^{+0.07}$ & $-0.84_{-3.16}^{+1.30}$ \\
2014dy & 2MASX J02485792-0045389 & False & Ia & 0.075 & 16.3 & 0.14 & $11.05_{-0.01}^{+0.01}$ & $-0.27_{0.00}^{+0.00}$ \\
2014dz & 2MASX J03281358+3800587 & True & Ia & 0.0176 & 16.6 & 0.77 & $10.26_{-0.14}^{+0.29}$ & $-3.42_{-0.58}^{+2.72}$ \\
2014dx & MCG -03-22-002 & False & Ia & 0.018926 & 15.6 & 0.18 & $10.81_{-0.10}^{+0.24}$ & $<-1.13$ \\
2015B & NGC 4782 & True & Ia & 0.01544 & 15.9 & 0.15 & $11.55_{-0.08}^{+0.05}$ & $-0.23_{-0.56}^{+0.02}$ \\
LSQ15z & 2MASX J13082255-0844002 & False & Ia & 0.07 & 17.0 & 0.10 & $10.36_{-0.08}^{+0.30}$ & $-0.12_{-0.02}^{+0.11}$ \\
2015A & NGC 2955 & True & Ia & 0.02339 & 16.5 & 0.03 & $10.87_{-0.09}^{+0.25}$ & $ 0.23_{-0.01}^{+0.25}$ \\
2015E & KUG 0311+000 & False & Ia & 0.04145 & 16.1 & 0.23 & $10.27_{-0.17}^{+0.08}$ & $-0.31_{-0.01}^{+0.03}$ \\
2015H & NGC 3464 & False & Ia-02cx & 0.01246 & 16.3 & 0.15 & $10.80_{-0.24}^{+0.07}$ & $-0.16_{-0.29}^{+0.20}$ \\
PSN J13471211-2422171 & ESO 509-G108 & True & Ia & 0.01991 & 16.0 & 0.20 & $11.20_{-0.31}^{+0.01}$ & $-1.19_{-2.81}^{+0.03}$ \\
iPTF15ku & KUG 1232+315 & True & Ia-91T & 0.02818 & 16.0 & 0.04 & $9.41_{-0.26}^{+0.41}$ & $-0.52_{-0.12}^{+0.12}$ \\
CSS150214:140955+173155 & NGC 5490 & True & Ia-91bg & 0.0162 & 15.7 & 0.07 & $11.46_{-0.15}^{+0.05}$ & $-1.72_{-2.28}^{+0.75}$ \\
PSN J19235601-5955321 & NGC 6782 & False & Ia & 0.01308 & 15.1 & 0.16 & $10.76_{-0.07}^{+0.42}$ & $-1.43_{-2.57}^{+1.64}$ \\
2015F & NGC 2442 & True & Ia & 0.00489 & 13.3 & 0.56 & $10.19_{-0.19}^{+0.01}$ & $ 3.69_{-0.56}^{+0.01}$ \\
PS15mb & SDSS J085940.13+151113.5 & True & Ia & 0.02872 & 16.7 & 0.10 & $8.94_{-0.03}^{+0.18}$ & $-2.56_{-1.44}^{+0.98}$ \\
PSN J08593491+4555343 & UGC 04709 & True & Ia & 0.0281 & 16.5 & 0.07 & $10.58_{-0.29}^{+0.24}$ & $ 0.01_{-4.01}^{+0.25}$ \\
SMTJ10310056-3658262 & ESO 375-G052 & False & Ia-91T & 0.03044 & 16.5 & 0.20 & $9.95_{-0.49}^{+1.29}$ & $-0.94_{-3.06}^{+3.60}$ \\
2015bp & NGC 5839 & True & Ia-91bg & 0.00407 & 13.8 & 0.14 & $9.94_{-0.17}^{+0.01}$ & $<-2.01$ \\
PSN J13332289+5843315 & 2MASX J13332590+5843195 & False & Ia & 0.03023 & 16.9 & 0.02 & $9.67_{-0.18}^{+0.07}$ & $-0.46_{-0.16}^{+0.04}$ \\
LSQ15adm & AM 2010-581 & False & Ia+CSM & 0.073 & 16.2 & 0.12 & $10.69_{-0.54}^{+0.01}$ & $-0.00_{-4.00}^{+0.08}$ \\
MASTER OT J074610.09-712224.9 & 2MFGC 06148 & True & Ia & 0.019 & 15.8 & 0.46 & $9.48_{-1.17}^{+0.61}$ & $<1.38$ \\
2015I & NGC 2357 & False & Ia & 0.00759 & 14.0 & 0.18 & $9.50_{-0.79}^{+0.99}$ & $<2.37$ \\
PS15ahs & MCG +07-37-011 & True & Ia & 0.031 & 16.2 & 0.10 & $9.93_{-0.10}^{+0.15}$ & $-0.88_{-3.12}^{+0.99}$ \\
2015M & COMAi J130032.301+275841.02 & True & Ia-91T & 0.023 & 15.6 & 0.03 & $7.86_{-0.06}^{+0.09}$ & $<-2.83$ \\
PSN J16283836+3932552 & NGC 6166 & True & Ia-91bg & 0.03035 & 16.4 & 0.03 & $11.68_{-0.09}^{+0.01}$ & $<-0.77$ \\
PSN J16025128+4713292 & UGC 10156 NED01 & True & Ia & 0.02025 & 15.6 & 0.05 & $<11.01$ & $<-4.00$ \\
Gaia15agm & ESO 241-G005 & False & Ia & 0.029 & 16.1 & 0.03 & $8.39_{-1.44}^{+0.44}$ & $-1.56_{-2.44}^{+1.36}$ \\
MASTER OT J114925.48-050713.8 & NGC 3915 & True & Ia & 0.00557 & 13.4 & 0.08 & $9.32_{-0.17}^{+0.24}$ & $<-0.51$ \\
2015ai & UGC 08734 & True & Ia & 0.0307 & 16.0 & 0.05 & $11.12_{-0.18}^{+0.16}$ & $-0.97_{-0.04}^{+0.02}$ \\
2015N & UGC 11797 & True & Ia & 0.01859 & 16.1 & 1.47 & $11.33_{-1.69}^{+0.09}$ & $<2.70$ \\
Supernova in Mrk 477 & Mrk 477 & False & Ia & 0.03773 & 16.9 & 0.03 & $10.39_{-0.17}^{+0.19}$ & $ 0.73_{-0.27}^{+0.11}$ \\
2015ab & NGC 938 & True & Ia & 0.01374 & 14.7 & 0.31 & $11.03_{-0.04}^{+0.08}$ & $<-2.92$ \\
PSN J20435314+1230304 & NGC 6956 & True & Ia & 0.01551 & 15.8 & 0.27 & $10.39_{-0.86}^{+0.91}$ & $<3.83$ \\
2015aw & ESO 197-G024 & True & Ia-91T & 0.01962 & 15.6 & 0.05 & $10.41_{-0.52}^{+0.01}$ & $-0.55_{-3.45}^{+0.04}$ \\
2015ac & UGC 12474 & True & Ia-91bg & 0.01707 & 15.6 & 0.20 & $10.83_{-0.01}^{+0.24}$ & $-1.17_{-0.03}^{+0.46}$ \\
2015ad & UGC 02282 & False & Ia & 0.02415 & 16.9 & 0.28 & $10.20_{-1.17}^{+0.34}$ & $ 0.46_{-4.46}^{+0.85}$ \\
MASTER OT J233743.22-473039.3 & ESO 240-G010 & True & Ia & 0.01101 & 14.3 & 0.04 & $11.05_{-0.28}^{+0.14}$ & $-1.14_{-2.86}^{+0.01}$ \\
2015ak & ESO 108-IG021 & True & Ia & 0.01037 & 14.5 & 0.08 & $10.31_{-0.50}^{+0.07}$ & $-0.09_{-3.91}^{+0.07}$ \\
PSN J22412689+3917220 & UGC 12156 & True & Ia & 0.01729 & 16.4 & 0.35 & $9.39_{-0.27}^{+0.23}$ & $-2.84_{-1.16}^{+3.47}$ \\
PSN J00275992+3045595 & UGC 00276 & False & Ia & 0.02112 & 16.4 & 0.21 & $10.75_{-0.01}^{+0.01}$ & $<-4.00$ \\
PSN J23523718+1433092 & UGC 12822 & False & Ia & 0.02658 & 16.9 & 0.11 & $11.22_{-0.10}^{+0.06}$ & $<-1.73$ \\
PSN J02524671+4656470 & UGC 02351 & False & Ia & 0.02809 & 16.3 & 0.54 & $11.42_{-0.29}^{+0.13}$ & $<0.11$ \\
LSQ15bci & MCG -05-04-023 & False & Ia & 0.03563 & 17.0 & 0.07 & $11.23_{-0.41}^{+0.06}$ & $-0.45_{-3.55}^{+0.02}$ \\
2015ao & ESO 354-G003 & True & Ia-91bg & 0.01913 & 16.5 & 0.04 & $11.02_{-0.32}^{+0.01}$ & $-1.37_{-2.63}^{+0.05}$ \\
PS15cku & 2MASX J01242239+0335168 & True & Ia & 0.023 & 16.0 & 0.07 & $9.58_{-0.24}^{+0.31}$ & $-0.54_{-0.41}^{+0.17}$ \\
MASTER OT J103747.94-270507.2 & IC 2597 & False & Ia & 0.00756 & 16.5 & 0.19 & $10.83_{-0.24}^{+0.18}$ & $-3.09_{-0.91}^{+1.67}$ \\
PSN J02004778+1641365 & 2MASX J02004757+1641401 & False & Ia & 0.027 & 16.2 & 0.13 & $10.13_{-0.06}^{+0.07}$ & $-2.16_{-1.84}^{+0.00}$ \\
PSN J21312375+4336312 & 2MASX J21312321+4336182 & False & Ia & 0.01841 & 16.4 & 1.03 & $10.68_{-1.79}^{+0.01}$ & $<1.46$ \\
PSN J09100885+5003396 & UGC 04812 & False & Ia-09dc & 0.03445 & 16.5 & 0.05 & $10.27_{-1.15}^{+0.28}$ & $<1.54$ \\
CSS151109:101502+074830 & SDSS J101502.54+074826.6 & False & Ia & 0.02829 & 16.3 & 0.10 & $8.79_{-0.10}^{+0.25}$ & $-1.21_{-0.28}^{+0.16}$ \\
2015ar & NGC 383 & True & Ia & 0.01701 & 15.3 & 0.19 & $11.64_{-0.27}^{+0.10}$ & $<-0.04$ \\
PSN J07051005+2102327 & 2MASX J07051014+2102233 & False & Ia & 0.08 & 16.5 & 0.24 & $10.26_{-0.16}^{+0.06}$ & $-1.64_{-2.36}^{+2.77}$ \\
PS15cwx & 2MFGC 04279 & False & Ia-91T & 0.046 & 17.0 & 0.47 & $10.97_{-0.28}^{+0.10}$ & $-2.12_{-1.88}^{+2.08}$ \\
MASTER OT J215050.94-702028.9 & NGC 7123 & True & Ia & 0.01234 & 14.5 & 0.08 & $11.24_{-0.01}^{+0.01}$ & $<-4.00$ \\
2015az & IC 0290 & True & Ia & 0.02012 & 15.6 & 0.46 & $10.55_{-0.14}^{+0.29}$ & $-2.12_{-1.88}^{+1.95}$ \\
2015bd & NGC 3662 & False & Ia-91T & 0.01861 & 15.9 & 0.15 & $11.09_{-0.01}^{+0.01}$ & $<-4.00$ \\
CSS151209:232318+164003 & GALEXMSC J232317.78+164003.8 & False & Ia & 0.049 & 16.6 & 0.07 & $9.11_{-0.09}^{+0.11}$ & $-1.79_{-2.21}^{+0.02}$ \\
PSN J01534240+2956107 & UGC 01359 & True & Ia & 0.02554 & 16.4 & 0.15 & $10.73_{-0.17}^{+0.30}$ & $<0.42$ \\
CSS151230:044008+123051 & UGC 03123 & False & Ia & 0.02646 & 16.8 & 1.22 & $10.91_{-0.28}^{+0.09}$ & $-0.40_{-3.60}^{+0.53}$ \\
2016D & 2MASX J04012613-5445295 & True & Ia & 0.0451 & 16.5 & 0.04 & $11.41_{-0.34}^{+0.01}$ & $-0.98_{-3.02}^{+0.07}$ \\
2016W & NGC 946 & True & Ia & 0.01925 & 15.8 & 0.19 & $11.04_{-0.11}^{+0.21}$ & $-2.77_{-1.23}^{+1.66}$ \\
ATLAS16aaf & 2MASX J02030578-0350240 & False & Ia-07if & 0.04248 & 17.0 & 0.07 & $10.41_{-0.19}^{+0.01}$ & $-1.31_{-2.69}^{+0.00}$ \\
ATLAS16aab & 2MASX J03214217+4205549 & False & Ia-91bg & 0.018 & 16.5 & 0.51 & $9.79_{-0.08}^{+0.24}$ & $<-1.04$ \\
MASTER OT J105908.57+103834.8 & SDSS J105908.63+103829.7 & True & Ia & 0.035 & 17.0 & 0.07 & $8.25_{-0.19}^{+0.34}$ & $-1.43_{-0.21}^{+0.16}$ \\
2016adi & NGC 5292 & False & Ia & 0.0149 & 15.3 & 0.16 & $11.25_{-0.51}^{+0.15}$ & $ 0.13_{-4.13}^{+0.13}$ \\
2016ajf & NGC 1278 & True & Ia & 0.02031 & 16.9 & 0.45 & $11.56_{-0.14}^{+0.08}$ & $-1.52_{-2.48}^{+0.02}$ \\
Gaia16aeu & 2dFGRS S394Z183 & False & Ia-91bg & 0.02136 & 16.9 & 0.07 & $8.86_{-0.25}^{+0.05}$ & $-1.49_{-0.10}^{+0.06}$ \\
Gaia16agf & Uncatalogued & True & Ia & 0.03 & 16.2 & 0.18 & $9.44_{-0.87}^{+0.34}$ & $<0.23$ \\
2016aqt & SDSS J134550.90+264747.4 & True & Ia-91T & 0.05046 & 16.5 & 0.05 & $9.27_{-0.21}^{+0.28}$ & $-0.37_{-3.63}^{+0.21}$ \\
2016bfu & IC 2150 & True & Ia-91bg & 0.0104 & 15.5 & 0.13 & $9.83_{-0.27}^{+0.56}$ & $<-0.05$ \\
MASTER OT J152333.04+092125.6 & CGCG 077-110 & True & Ia & 0.03292 & 16.9 & 0.09 & $11.32_{-0.07}^{+0.02}$ & $<-2.69$ \\
iPTF16abc & NGC 5221 & True & Ia-91T & 0.02328 & 15.9 & 0.08 & $11.30_{-0.01}^{+0.01}$ & $-0.48_{0.00}^{+0.01}$ \\
2016brx & NGC 7391 & False & Ia & 0.01017 & 16.1 & 0.26 & $11.17_{-0.06}^{+0.01}$ & $<-2.07$ \\
2016bry & UGC 11635 & False & Ia & 0.01602 & 15.6 & 0.43 & $11.17_{-0.37}^{+0.01}$ & $ 0.21_{-0.20}^{+0.06}$ \\
Gaia16alq & Uncatalogued & True & Ia & 0.023 & 16.1 & 0.18 & $7.91_{-0.82}^{+0.23}$ & $<-1.13$ \\
CSS160427:134449+210448 & SDSS J134448.50+210447.1 & False & Ia & 0.053 & 17.1 & 0.07 & $8.58_{-0.11}^{+0.26}$ & $-1.25_{-0.48}^{+0.19}$ \\
iPTF16auf & Mrk 0685 & True & Ia & 0.01489 & 15.3 & 0.04 & $9.01_{-0.01}^{+0.01}$ & $<-4.00$ \\
MASTER OT J202606.27-200732.6 & GALEXASC J202606.38-200732.4 & True & Ia & 0.0226 & 16.7 & 0.15 & $8.75_{-0.02}^{+0.01}$ & $<-4.00$ \\
KAIT-16X & NGC 4125 & True & Ia & 0.00452 & 13.0 & 0.05 & $11.13_{-0.09}^{+0.08}$ & $-1.26_{-2.74}^{+0.01}$ \\
ATLAS16bdg & NGC 4708 & True & Ia & 0.0139 & 16.0 & 0.13 & $10.62_{-0.49}^{+0.13}$ & $-0.15_{-0.55}^{+0.10}$ \\
PTSS-16ijc & CGCG 280-024 & False & Ia & 0.04457 & 16.5 & 0.28 & $11.31_{-0.24}^{+0.17}$ & $-1.67_{-2.33}^{+2.07}$ \\
MASTER OT J211223.35+144645.1 & GALEXASC J211223.05+144644.9 & True & Ia & 0.0293 & 16.5 & 0.26 & $9.22_{-0.15}^{+0.21}$ & $-0.80_{-0.41}^{+0.10}$ \\
CSS160708:151956+052419 & SDSS J151955.92+052418.9 & False & Ia & 0.045 & 16.2 & 0.13 & $<8.21$ & $<-4.00$ \\
2016dag & ESO 018-G002 & False & Ia & 0.01928 & 17.0 & 0.22 & $10.43_{-0.79}^{+0.98}$ & $<3.29$ \\
2016ekg & ESO 466-G032 & True & Ia & 0.0171 & 15.0 & 0.06 & $8.79_{-0.05}^{+0.03}$ & $<-1.07$ \\
Gaia16axi & 2MASX J05595753-1805253 & True & Ia & 0.02805 & 16.0 & 0.26 & $11.03_{-0.07}^{+0.01}$ & $-0.28_{-0.01}^{+0.02}$ \\
2016eoa & NGC 83 & True & Ia & 0.02077 & 15.6 & 0.19 & $11.59_{-0.13}^{+0.01}$ & $<-1.62$ \\
ATLAS16cjv & IC 0272 & True & Ia & 0.02893 & 16.3 & 0.12 & $10.91_{-0.31}^{+0.21}$ & $ 0.24_{-0.21}^{+0.12}$ \\
Gaia16bba & GALEXASC J010135.75+170604.9 & True & Ia & 0.034 & 16.6 & 0.13 & $8.64_{-0.26}^{+0.35}$ & $-1.20_{-2.80}^{+0.18}$ \\
Gaia16bbi & GALEXASC J235916.23+220302.4 & False & Ia & 0.04 & 16.8 & 0.14 & $8.91_{-0.26}^{+0.15}$ & $-0.53_{-3.47}^{+0.11}$ \\
ATLAS16cpu & CGCG 249-11 & True & Ia & 0.0182 & 15.6 & 0.08 & $10.24_{-0.12}^{+0.17}$ & $-1.05_{-0.55}^{+0.00}$ \\
MASTER OT J021729.29-595123.9 & NGC 888 & False & Ia & 0.02919 & 16.1 & 0.11 & $11.29_{-0.13}^{+0.18}$ & $<-0.94$ \\
2016fnr & UGC 10502 & True & Ia & 0.01437 & 15.2 & 0.13 & $9.85_{-0.13}^{+0.62}$ & $<0.37$ \\
Gaia16bew & GALEXASC J140251.91-303700.7 & False & Ia & 0.037 & 16.8 & 0.16 & $9.44_{-1.13}^{+0.26}$ & $-0.24_{-1.35}^{+0.12}$ \\
CSS160904:230721+025428 & Uncatalogued & False & Ia+CSM & 0.063 & 16.9 & 0.20 & $8.35_{-0.12}^{+0.15}$ & $-1.65_{-2.35}^{+0.40}$ \\
2016gfk & IC 1657 & True & Ia & 0.01195 & 17.0 & 0.07 & $10.77_{-0.46}^{+0.14}$ & $ 0.00_{-4.00}^{+0.09}$ \\
2016gfr & 2MASX J18193566+2347137 & True & Ia & 0.014 & 15.1 & 0.37 & $9.83_{-0.09}^{+0.03}$ & $<-2.79$ \\
Gaia16bhj & MCG -01-12-008 & True & Ia & 0.03074 & 16.2 & 0.12 & $10.91_{-0.24}^{+0.21}$ & $ 0.24_{-0.23}^{+0.04}$ \\
2016ghq & UGC 11199 & True & Ia & 0.02121 & 16.5 & 0.10 & $10.92_{-0.38}^{+0.01}$ & $-0.39_{-0.31}^{+0.02}$ \\
OGLE16dha & GALEXASC J063224.91-713403.9 & True & Ia & 0.006 & 15.2 & 0.26 & $7.94_{-1.61}^{+0.41}$ & $-1.12_{-2.88}^{+0.18}$ \\
SNhunt325 & CGCG 500-022 & True & Ia & 0.03131 & 16.5 & 0.23 & $10.22_{-0.17}^{+0.08}$ & $ 0.10_{-0.16}^{+0.02}$ \\
Gaia16bkz & NGC 2865 & True & Ia & 0.00874 & 15.9 & 0.23 & $10.88_{-0.22}^{+0.17}$ & $-1.12_{-2.88}^{+0.41}$ \\
2016gxp & NGC 51 & True & Ia & 0.0186 & 14.7 & 0.34 & $11.03_{-0.14}^{+0.15}$ & $-0.97_{-1.74}^{+0.02}$ \\
ATLAS16dmf & UGC 05356 & False & Ia & 0.02554 & 16.8 & 0.04 & $10.76_{-0.13}^{+0.09}$ & $-3.35_{-0.65}^{+2.35}$ \\
ATLAS16dou & 2MASX J06045961-3324449 & False & Ia & 0.03162 & 16.9 & 0.12 & $11.18_{-1.78}^{+0.01}$ & $<2.44$ \\
MASTER OT J033333.26-623314.7 & 2MASX J03333430-6233033 & True & Ia & 0.024 & 16.0 & 0.14 & $10.49_{-0.18}^{+0.13}$ & $-1.61_{-2.39}^{+0.01}$ \\
MASTER OT J110533.80+194118.7 & SDSS J110534.12+194118.9 & False & Ia & 0.027 & 16.7 & 0.07 & $9.68_{-0.16}^{+0.45}$ & $-0.06_{-0.23}^{+0.11}$ \\
ATLAS16dtf & UGC 03524 & True & Ia & 0.01309 & 15.6 & 1.20 & $10.84_{-0.05}^{+0.01}$ & $<-1.60$ \\
Gaia16byh & ESO 374-G025 & True & Ia & 0.02367 & 16.9 & 0.28 & $10.57_{-0.37}^{+0.15}$ & $ 0.17_{-4.17}^{+0.05}$ \\
Gaia16caa & UGC 09165 & True & Ia & 0.01754 & 16.0 & 0.05 & $10.73_{-0.01}^{+0.08}$ & $-0.59_{-0.38}^{+0.00}$ \\
Gaia16cay & NGC 5032 & False & Ia & 0.02138 & 16.7 & 0.05 & $11.23_{-0.35}^{+0.17}$ & $<0.06$ \\
MASTER OT J133905.0-201718.3 & 2MASX J13390624-2017235 & True & Ia & 0.03174 & 16.8 & 0.25 & $10.51_{-0.25}^{+0.14}$ & $-0.17_{-0.21}^{+0.04}$ \\
Gaia16cbd & UGC 07367 & True & Ia & 0.0137 & 15.5 & 0.04 & $10.99_{-0.07}^{+0.07}$ & $-1.99_{-2.01}^{+0.00}$ \\
ATLAS16dzg & CGCG 068-006 & True & Ia & 0.02708 & 16.5 & 0.09 & $10.29_{-0.08}^{+0.24}$ & $-0.10_{-0.01}^{+0.16}$ \\
ATLAS16dzp & SDSS J084324.74+373246.0 & True & Ia & 0.041 & 16.9 & 0.10 & $8.55_{-0.16}^{+0.39}$ & $-1.27_{-0.13}^{+0.16}$ \\
\hline
\end{tabular}
\medskip
\raggedright
\noindent This table is available in its entirety in a machine readable form. A portion is shown here for guidance regarding its form and content.\\
$^{a}$ This column denotes whether or not this SN/host galaxy pair was used in the analysis.\\
$^{b}$ Peak magnitudes measured from ASAS-SN $V$-band data when possible. For instances when this was not possible, peak magnitudes from D. W. Bishop's Bright Supernova website were adopted and may be from different filters.\\
$^{c}$ The lower limits on the SFR generally not well constrained; we truncate the limits at $10^{-4}\msun$ yr$^{-1}$.\\
\label{tab:host_table}
\end{minipage}
\end{table}


==> tab2.tex <==
\begin{table}
\begin{minipage}{\textwidth}
\caption{Photometric host data.\hfill}\begin{tabular}{llllllllllllllllllc}
\hline
SN name & Host name & $m_{\rm NUV}$ & $m_{\rm SDSS~u}$ & $m_{\rm SDSS~g}$ & $m_{\rm SDSS~r}$ & $m_{\rm SDSS~i}$ & $m_{\rm SDSS~z}$ & $m_{\rm PS1~g}$ & $m_{\rm PS1~r}$ & $m_{\rm PS1~i}$ & $m_{\rm PS1~z}$ & $m_{\rm PS1~y}$ & $m_{\rm 2MASS~J}$ & $m_{\rm 2MASS~H}$ & $m_{\rm 2MASS~K_s}$ & $m_{\rm W1}$ & $m_{\rm W2}$ & Opt. survey \\
\hline
ASASSN-13an & 2MASX J13453653-0719350 & $16.8\pm0.1$ & -- & -- & -- & -- & -- & $14.7\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $13.6\pm0.1$ & $13.3\pm0.1$ & $13.2\pm0.1$ & $13.3\pm0.1$ & $14.2\pm0.1$ & $14.8\pm0.1$ & PS1\\
ASASSN-13ar & VV 478 & $17.7\pm0.1$ & $16.9\pm0.1$ & $15.2\pm0.1$ & $14.6\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $15.8\pm0.1$ & -- & $14.7\pm0.1$ & $14.7\pm0.1$ & $14.8\pm0.1$ & $15.3\pm0.1$ & $15.0\pm0.1$ & $15.4\pm0.2$ & $16.5\pm0.1$ & $17.1\pm0.1$ & PS1\\
ASASSN-13av & NGC 7068 & -- & $16.3\pm0.1$ & $14.6\pm0.1$ & $13.7\pm0.1$ & $13.3\pm0.1$ & $12.9\pm0.1$ & $14.5\pm0.1$ & $13.8\pm0.1$ & $13.4\pm0.1$ & $13.2\pm0.1$ & $14.8\pm0.1$ & $12.6\pm0.1$ & $12.2\pm0.1$ & $12.4\pm0.1$ & $13.8\pm0.1$ & $14.3\pm0.1$ & SDSS\\
ASASSN-13aw & CGCG 252-043 & $16.8\pm0.1$ & -- & -- & -- & -- & -- & $14.8\pm0.1$ & $14.2\pm0.1$ & $13.9\pm0.1$ & $13.8\pm0.1$ & $13.9\pm0.1$ & $13.3\pm0.1$ & $13.2\pm0.1$ & $13.5\pm0.1$ & $15.9\pm0.1$ & $16.5\pm0.1$ & PS1\\
ASASSN-13bb & UGC 01395 & $16.8\pm0.1$ & $15.6\pm0.1$ & $14.1\pm0.1$ & $13.3\pm0.1$ & $12.9\pm0.1$ & $12.6\pm0.1$ & -- & $15.6\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $13.6\pm0.1$ & $12.4\pm0.1$ & $12.0\pm0.1$ & $12.1\pm0.1$ & $14.2\pm0.1$ & $14.4\pm0.1$ & SDSS\\
ASASSN-13cc & NGC 1954 & -- & -- & -- & -- & -- & -- & $12.3\pm0.1$ & $13.5\pm0.1$ & $13.6\pm0.1$ & $12.9\pm0.1$ & $12.6\pm0.1$ & $10.2\pm0.1$ & $ 9.4\pm0.1$ & $ 9.2\pm0.1$ & $13.0\pm0.1$ & $13.7\pm0.1$ & --\\
ASASSN-13ch & CGCG 023-030 & $17.8\pm0.1$ & $16.9\pm0.1$ & $16.0\pm0.1$ & $15.7\pm0.1$ & $15.5\pm0.1$ & $15.3\pm0.1$ & $16.1\pm0.1$ & $15.7\pm0.1$ & $15.6\pm0.1$ & $15.4\pm0.1$ & $15.2\pm0.1$ & $15.1\pm0.1$ & $14.8\pm0.1$ & $15.4\pm0.2$ & $16.2\pm0.1$ & $16.6\pm0.1$ & SDSS\\
ASASSN-13cj & CGCG 051-075 & $20.3\pm0.1$ & $17.2\pm0.1$ & $15.5\pm0.1$ & $14.7\pm0.1$ & $14.3\pm0.1$ & $14.0\pm0.1$ & $15.7\pm0.1$ & $14.9\pm0.1$ & $14.6\pm0.1$ & $14.4\pm0.1$ & $14.3\pm0.1$ & $15.3\pm0.1$ & $15.1\pm0.1$ & $15.4\pm0.1$ & $15.3\pm0.1$ & $16.0\pm0.1$ & PS1\\
ASASSN-13cp & ARK 477 & $17.8\pm0.1$ & $16.1\pm0.1$ & $14.3\pm0.1$ & $13.5\pm0.1$ & $13.1\pm0.1$ & $12.7\pm0.1$ & $14.4\pm0.1$ & $13.8\pm0.1$ & $13.4\pm0.1$ & $13.1\pm0.1$ & $12.9\pm0.1$ & $12.6\pm0.1$ & $12.4\pm0.1$ & $12.6\pm0.1$ & $13.8\pm0.1$ & $14.5\pm0.1$ & SDSS\\
ASASSN-13cu & VIII Zw 035 & $17.4\pm0.1$ & $16.6\pm0.1$ & $15.4\pm0.1$ & $14.8\pm0.1$ & $14.6\pm0.1$ & $14.3\pm0.1$ & $15.3\pm0.1$ & $14.8\pm0.1$ & $14.6\pm0.1$ & $14.4\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $13.9\pm0.1$ & $14.0\pm0.1$ & $15.0\pm0.1$ & $15.5\pm0.1$ & SDSS\\
ASASSN-13dd & NGC 2765 & $17.9\pm0.1$ & $14.5\pm0.1$ & $12.7\pm0.1$ & $11.9\pm0.1$ & $11.5\pm0.1$ & $11.2\pm0.1$ & -- & $12.3\pm0.1$ & -- & -- & -- & $11.1\pm0.1$ & $10.9\pm0.1$ & $11.1\pm0.1$ & $13.0\pm0.1$ & $13.7\pm0.1$ & SDSS\\
ASASSN-13dl & Uncatalogued & -- & -- & -- & -- & -- & -- & $17.2\pm0.1$ & $16.7\pm0.1$ & $16.6\pm0.1$ & $16.4\pm0.1$ & $16.2\pm0.1$ & -- & -- & -- & $19.0\pm0.1$ & $19.7\pm0.2$ & PS1\\
ASASSN-13dm & 2MASX J03021111+1555387 & $19.2\pm0.1$ & -- & -- & -- & -- & -- & $15.6\pm0.1$ & $14.9\pm0.1$ & $14.5\pm0.1$ & $14.3\pm0.1$ & $14.0\pm0.1$ & $13.6\pm0.1$ & $13.4\pm0.1$ & $13.6\pm0.1$ & $14.2\pm0.1$ & $14.6\pm0.1$ & PS1\\
ASASSN-14ad & KUG 1237+183 & $17.8\pm0.1$ & $17.5\pm0.1$ & $16.5\pm0.1$ & $16.1\pm0.1$ & $16.0\pm0.1$ & $15.9\pm0.1$ & $16.6\pm0.1$ & $16.3\pm0.1$ & $16.1\pm0.1$ & $16.1\pm0.1$ & $16.1\pm0.1$ & $14.5\pm0.1$ & $14.7\pm0.1$ & $14.3\pm0.1$ & $17.6\pm0.1$ & $18.1\pm0.1$ & SDSS\\
ASASSN-14ar & IC 0527 & $16.3\pm0.1$ & $18.6\pm0.1$ & $16.9\pm0.1$ & $17.1\pm0.1$ & $15.4\pm0.1$ & $15.4\pm0.1$ & $15.7\pm0.1$ & $14.8\pm0.1$ & $14.2\pm0.1$ & $13.1\pm0.1$ & -- & $12.3\pm0.1$ & $12.1\pm0.1$ & $12.1\pm0.1$ & $14.4\pm0.1$ & $15.2\pm0.1$ & --\\
ASASSN-14as & MGC +06-29-001 & -- & $17.1\pm0.1$ & $15.7\pm0.1$ & $15.0\pm0.1$ & $14.6\pm0.1$ & $14.3\pm0.1$ & $16.0\pm0.1$ & $15.5\pm0.1$ & $15.2\pm0.1$ & $15.0\pm0.1$ & $14.7\pm0.1$ & $14.5\pm0.1$ & $14.4\pm0.1$ & $14.5\pm0.1$ & $15.4\pm0.1$ & $16.0\pm0.1$ & SDSS\\
ASASSN-14ax & SDSS J171000.69+270619.5 & $19.4\pm0.1$ & $18.7\pm0.1$ & $17.9\pm0.1$ & $17.6\pm0.1$ & $17.4\pm0.1$ & $17.2\pm0.1$ & $17.9\pm0.1$ & $17.6\pm0.1$ & $17.4\pm0.1$ & $17.4\pm0.1$ & $17.3\pm0.1$ & $17.2\pm0.1$ & $16.9\pm0.1$ & $17.3\pm0.2$ & $17.3\pm0.1$ & $17.7\pm0.1$ & SDSS\\
ASASSN-14ay & 2MASX J15570268+3725001 & $20.6\pm0.3$ & $18.0\pm0.1$ & $16.3\pm0.1$ & $15.5\pm0.1$ & $15.2\pm0.1$ & $14.9\pm0.1$ & $16.5\pm0.1$ & $15.7\pm0.1$ & $15.4\pm0.1$ & $15.2\pm0.1$ & $15.0\pm0.1$ & $14.6\pm0.1$ & $14.7\pm0.1$ & $14.8\pm0.1$ & $16.1\pm0.1$ & $16.8\pm0.1$ & SDSS\\
ASASSN-14ba & SDSS J102131.91+082419.8 & $19.6\pm0.1$ & $18.7\pm0.1$ & $17.3\pm0.1$ & $16.7\pm0.1$ & $16.4\pm0.1$ & $16.1\pm0.1$ & $17.2\pm0.1$ & $16.7\pm0.1$ & $16.5\pm0.1$ & $16.2\pm0.1$ & $16.1\pm0.1$ & $17.0\pm0.1$ & $16.6\pm0.1$ & $16.9\pm0.2$ & $16.5\pm0.1$ & $16.9\pm0.1$ & SDSS\\
ASASSN-14bb & 2MASX J12141125+3839400 & $19.9\pm0.1$ & $17.9\pm0.1$ & $16.5\pm0.1$ & $15.9\pm0.1$ & $15.5\pm0.1$ & $15.3\pm0.1$ & $16.6\pm0.1$ & $16.0\pm0.1$ & $15.6\pm0.1$ & $15.5\pm0.1$ & $15.3\pm0.1$ & $15.1\pm0.1$ & $14.7\pm0.1$ & $15.1\pm0.1$ & $15.9\pm0.1$ & $16.5\pm0.1$ & SDSS\\
ASASSN-14bd & IC 0831 & $19.6\pm0.1$ & $16.4\pm0.1$ & $14.6\pm0.1$ & $13.7\pm0.1$ & $13.3\pm0.1$ & $12.9\pm0.1$ & $14.6\pm0.1$ & $14.2\pm0.1$ & $13.5\pm0.1$ & $13.3\pm0.1$ & $13.1\pm0.1$ & $12.7\pm0.1$ & $12.4\pm0.1$ & $12.6\pm0.1$ & $13.9\pm0.1$ & $14.6\pm0.1$ & SDSS\\
ASASSN-14bt & UGC 05566 & $19.1\pm0.1$ & $17.3\pm0.1$ & $14.7\pm0.1$ & $13.7\pm0.1$ & $13.2\pm0.1$ & $12.7\pm0.1$ & $15.0\pm0.1$ & $14.1\pm0.1$ & $13.7\pm0.1$ & $13.5\pm0.1$ & $13.2\pm0.1$ & $12.8\pm0.1$ & $12.5\pm0.1$ & $12.6\pm0.1$ & $14.0\pm0.1$ & $14.6\pm0.1$ & SDSS\\
ASASSN-14cb & 2MASXi J1308145+620200 & -- & $19.3\pm0.1$ & $17.7\pm0.1$ & $16.9\pm0.1$ & $16.4\pm0.1$ & $16.0\pm0.1$ & $17.9\pm0.1$ & $17.1\pm0.1$ & $16.7\pm0.1$ & $16.5\pm0.1$ & $16.2\pm0.1$ & $16.6\pm0.1$ & $16.3\pm0.1$ & $16.3\pm0.1$ & $16.5\pm0.1$ & $17.0\pm0.1$ & SDSS\\
ASASSN-14co & CGCG 023-005 & $17.7\pm0.1$ & $17.0\pm0.1$ & $15.7\pm0.1$ & $15.1\pm0.1$ & $14.7\pm0.1$ & $14.5\pm0.1$ & $15.5\pm0.1$ & $15.0\pm0.1$ & $14.8\pm0.1$ & $14.7\pm0.1$ & $14.5\pm0.1$ & $14.1\pm0.1$ & $14.0\pm0.1$ & $14.2\pm0.1$ & $15.3\pm0.1$ & $15.8\pm0.1$ & SDSS\\
ASASSN-14cu & 2MASX J12470274-2414435 & $20.5\pm0.2$ & -- & -- & -- & -- & -- & $15.5\pm0.1$ & $14.7\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $13.9\pm0.1$ & $13.6\pm0.1$ & $13.4\pm0.1$ & $13.4\pm0.1$ & $14.4\pm0.1$ & $15.1\pm0.1$ & PS1\\
ASASSN-14db & ESO 075-G049 & $17.1\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.4\pm0.1$ & $13.3\pm0.1$ & $13.5\pm0.1$ & $14.5\pm0.1$ & $15.0\pm0.1$ & --\\
ASASSN-14dc & 2MASX J02183825+3336556 & $19.2\pm0.1$ & -- & -- & -- & -- & -- & $16.8\pm0.1$ & $16.2\pm0.1$ & $15.9\pm0.1$ & $15.8\pm0.1$ & $15.6\pm0.1$ & $15.2\pm0.1$ & $15.1\pm0.1$ & $15.3\pm0.1$ & $16.1\pm0.1$ & $16.6\pm0.1$ & PS1\\
ASASSN-14dz & Mrk 842 & $19.9\pm0.1$ & $16.6\pm0.1$ & $15.0\pm0.1$ & $14.2\pm0.1$ & $13.8\pm0.1$ & $14.8\pm0.1$ & $15.0\pm0.1$ & $14.3\pm0.1$ & $13.9\pm0.1$ & $13.8\pm0.1$ & $13.6\pm0.1$ & $13.3\pm0.1$ & $13.1\pm0.1$ & $13.2\pm0.1$ & $14.3\pm0.1$ & $15.0\pm0.1$ & PS1\\
ASASSN-14ef & MCG -05-52-046 & $20.7\pm0.3$ & -- & -- & -- & -- & -- & $15.3\pm0.1$ & $14.7\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $13.8\pm0.1$ & $13.4\pm0.1$ & $13.2\pm0.1$ & $13.4\pm0.1$ & $14.5\pm0.1$ & $15.2\pm0.1$ & PS1\\
ASASSN-14em & KUG 1359+345 & $18.0\pm0.1$ & $17.0\pm0.1$ & $15.8\pm0.1$ & $15.2\pm0.1$ & $14.8\pm0.1$ & $14.6\pm0.1$ & $15.7\pm0.1$ & $15.2\pm0.1$ & $15.0\pm0.1$ & $14.8\pm0.1$ & $14.6\pm0.1$ & $14.4\pm0.1$ & $14.3\pm0.1$ & $14.5\pm0.1$ & $15.8\pm0.1$ & $16.3\pm0.1$ & SDSS\\
ASASSN-14eo & CGCG 461-012 & $16.9\pm0.1$ & $16.0\pm0.1$ & $14.8\pm0.1$ & $14.3\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $15.1\pm0.1$ & $14.4\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $14.2\pm0.1$ & $13.9\pm0.1$ & $13.7\pm0.1$ & $13.8\pm0.1$ & $15.4\pm0.1$ & $16.0\pm0.1$ & SDSS\\
ASASSN-14ep & CGCG 338-006 & $19.7\pm0.1$ & -- & -- & -- & -- & -- & $15.1\pm0.1$ & $14.5\pm0.1$ & $14.2\pm0.1$ & $13.9\pm0.1$ & $13.8\pm0.1$ & $13.3\pm0.1$ & $12.9\pm0.1$ & $13.2\pm0.1$ & $14.8\pm0.1$ & $15.4\pm0.1$ & PS1\\
ASASSN-14es & IC 4462 & $17.2\pm0.1$ & $16.3\pm0.1$ & $15.1\pm0.1$ & $14.5\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $15.1\pm0.1$ & $14.7\pm0.1$ & $14.6\pm0.1$ & $14.2\pm0.1$ & $14.7\pm0.1$ & $13.7\pm0.1$ & $13.6\pm0.1$ & $13.9\pm0.1$ & $15.2\pm0.1$ & $15.7\pm0.1$ & SDSS\\
ASASSN-14eu & MCG -01-38-015 & -- & -- & -- & -- & -- & -- & $14.6\pm0.1$ & $13.5\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $12.5\pm0.1$ & $11.9\pm0.1$ & $11.7\pm0.1$ & $11.8\pm0.1$ & $13.3\pm0.1$ & $14.0\pm0.1$ & PS1\\
ASASSN-14ew & 2MASX J20220000-5147474 & $17.8\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $14.7\pm0.1$ & $14.6\pm0.1$ & $14.8\pm0.2$ & $15.8\pm0.1$ & $16.4\pm0.1$ & --\\
ASASSN-14fa & ESO 416-G039 & $19.5\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.6\pm0.1$ & $12.4\pm0.1$ & $12.6\pm0.1$ & $13.8\pm0.1$ & $14.5\pm0.1$ & --\\
ASASSN-14fo & GALEXASC J203406.21-015759.2 & $21.3\pm0.3$ & -- & -- & -- & -- & -- & $17.4\pm0.1$ & $16.6\pm0.1$ & $16.4\pm0.1$ & $16.1\pm0.1$ & $15.9\pm0.1$ & -- & -- & -- & $17.6\pm0.1$ & $18.2\pm0.1$ & PS1\\
ASASSN-14fw & MCG -01-60-044 & $17.0\pm0.1$ & $16.1\pm0.1$ & $15.0\pm0.1$ & $14.5\pm0.1$ & $14.2\pm0.1$ & $13.9\pm0.1$ & $14.9\pm0.1$ & $14.6\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $13.9\pm0.1$ & $13.7\pm0.1$ & $13.6\pm0.1$ & $13.6\pm0.1$ & $15.0\pm0.1$ & $15.5\pm0.1$ & SDSS\\
ASASSN-14gh & SDSS J171509.30+414841.6 & $19.6\pm0.1$ & $21.0\pm0.1$ & $19.3\pm0.1$ & $18.7\pm0.1$ & $18.4\pm0.1$ & $18.0\pm0.1$ & $18.8\pm0.1$ & $18.2\pm0.1$ & $18.7\pm0.1$ & $18.2\pm0.1$ & $18.5\pm0.1$ & -- & -- & -- & -- & -- & PS1\\
ASASSN-14hp & 2MASX J21303015-7038489 & $18.0\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $15.5\pm0.1$ & $15.4\pm0.2$ & $15.6\pm0.2$ & $16.5\pm0.1$ & $17.0\pm0.1$ & --\\
ASASSN-14hr & 2MASX J01504127-1431032 & $17.3\pm0.1$ & -- & -- & -- & -- & -- & $15.7\pm0.1$ & $15.1\pm0.1$ & $14.8\pm0.1$ & $14.6\pm0.1$ & $14.5\pm0.1$ & $14.3\pm0.1$ & $14.2\pm0.1$ & $14.2\pm0.1$ & $15.8\pm0.1$ & $16.4\pm0.1$ & PS1\\
ASASSN-14hu & ESO 058-G012 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.4\pm0.1$ & $13.0\pm0.1$ & $13.3\pm0.1$ & $14.7\pm0.1$ & $15.2\pm0.1$ & --\\
ASASSN-14ig & ESO 113-G032 & $17.5\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.2\pm0.1$ & $12.0\pm0.1$ & $12.1\pm0.1$ & $13.8\pm0.1$ & $14.4\pm0.1$ & --\\
ASASSN-14ih & MCG -04-53-013 & $19.2\pm0.1$ & -- & -- & -- & -- & -- & $14.7\pm0.1$ & $13.9\pm0.1$ & $13.5\pm0.1$ & $13.4\pm0.1$ & $13.4\pm0.1$ & $12.8\pm0.1$ & $12.5\pm0.1$ & $12.6\pm0.1$ & $14.1\pm0.1$ & $14.9\pm0.1$ & PS1\\
ASASSN-14ii & 2dFGRS S588Z294 & $20.5\pm0.2$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $14.0\pm0.1$ & $13.7\pm0.1$ & $13.9\pm0.1$ & $15.0\pm0.1$ & $15.7\pm0.1$ & --\\
ASASSN-14in & 2MASX J18242915+5226380 & $19.7\pm0.1$ & -- & -- & -- & -- & -- & $17.6\pm0.1$ & $17.1\pm0.1$ & $16.8\pm0.1$ & $16.6\pm0.1$ & $16.6\pm0.1$ & $16.0\pm0.2$ & $15.6\pm0.2$ & $15.6\pm0.2$ & $16.9\pm0.1$ & $17.4\pm0.1$ & PS1\\
ASASSN-14iu & NGC 2771 & $16.4\pm0.1$ & $16.2\pm0.1$ & $14.2\pm0.1$ & $13.3\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $14.4\pm0.1$ & $13.6\pm0.1$ & $12.9\pm0.1$ & $12.6\pm0.1$ & $12.6\pm0.1$ & $11.7\pm0.1$ & $11.5\pm0.1$ & $11.7\pm0.1$ & $13.6\pm0.1$ & $14.3\pm0.1$ & PS1\\
ASASSN-14jc & 2MASX J07353554-6246099 & $17.4\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.7\pm0.1$ & $13.3\pm0.1$ & $13.7\pm0.1$ & $15.2\pm0.1$ & $15.8\pm0.1$ & --\\
ASASSN-14jg & 2MASX J23331223-6034201 & $16.4\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.9\pm0.1$ & $13.8\pm0.1$ & $14.1\pm0.1$ & $15.9\pm0.1$ & $16.5\pm0.1$ & --\\
ASASSN-14jz & GALEXASC J184443.33-524819.2 & $17.7\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $17.4\pm0.1$ & $18.0\pm0.1$ & --\\
ASASSN-14kd & 2MASX J22532475+0447583 & $19.0\pm0.1$ & $17.3\pm0.1$ & $15.9\pm0.1$ & $15.1\pm0.1$ & $14.7\pm0.1$ & $14.4\pm0.1$ & $15.7\pm0.1$ & $15.1\pm0.1$ & $14.7\pm0.1$ & $14.5\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $14.0\pm0.1$ & $15.1\pm0.1$ & $15.7\pm0.1$ & SDSS\\
ASASSN-14kq & 2MASX J23451480-2947009 & $18.0\pm0.1$ & -- & -- & -- & -- & -- & $16.1\pm0.1$ & $15.8\pm0.1$ & $15.5\pm0.1$ & $15.5\pm0.1$ & $15.5\pm0.1$ & $15.2\pm0.1$ & $14.7\pm0.1$ & $15.3\pm0.2$ & $16.4\pm0.1$ & $16.8\pm0.1$ & PS1\\
ASASSN-14kr & GALEXASC J125413.02-073849.5 & $17.6\pm0.1$ & -- & -- & -- & -- & -- & $16.3\pm0.1$ & $16.0\pm0.1$ & $16.1\pm0.1$ & $15.9\pm0.1$ & $15.8\pm0.1$ & -- & -- & -- & $18.1\pm0.1$ & $18.5\pm0.1$ & PS1\\
ASASSN-14lo & UGC 06837 & $18.7\pm0.1$ & $17.6\pm0.1$ & $16.2\pm0.1$ & $15.5\pm0.1$ & $15.1\pm0.1$ & $14.8\pm0.1$ & -- & -- & $15.5\pm0.1$ & $15.2\pm0.1$ & $15.1\pm0.1$ & $14.5\pm0.1$ & $14.1\pm0.1$ & $14.1\pm0.1$ & $15.3\pm0.1$ & $15.7\pm0.1$ & SDSS\\
ASASSN-14lp & NGC 4666 & $14.1\pm0.1$ & $13.9\pm0.1$ & $12.1\pm0.1$ & $11.1\pm0.1$ & $10.6\pm0.1$ & $10.1\pm0.1$ & $13.0\pm0.1$ & $10.3\pm0.1$ & -- & $ 8.7\pm0.1$ & $ 9.9\pm0.1$ & $ 9.1\pm0.1$ & $ 8.8\pm0.1$ & $ 8.9\pm0.1$ & $11.2\pm0.1$ & $11.6\pm0.1$ & SDSS\\
ASASSN-14lq & 2MASX J22571481-2058014 & $23.1\pm0.7$ & -- & -- & -- & -- & -- & $14.6\pm0.1$ & $13.8\pm0.1$ & $13.4\pm0.1$ & $13.3\pm0.1$ & $13.0\pm0.1$ & $12.6\pm0.1$ & $12.4\pm0.1$ & $12.8\pm0.1$ & $13.9\pm0.1$ & $14.6\pm0.1$ & PS1\\
ASASSN-14lt & IC 0299 & $19.7\pm0.1$ & -- & -- & -- & -- & -- & $14.9\pm0.1$ & $14.3\pm0.1$ & $13.8\pm0.1$ & $13.6\pm0.1$ & $13.4\pm0.1$ & $13.0\pm0.1$ & $12.9\pm0.1$ & $13.0\pm0.1$ & $14.4\pm0.1$ & $15.1\pm0.1$ & PS1\\
ASASSN-14lu & 2MASX J14103977-0241003 & $19.6\pm0.1$ & $16.6\pm0.1$ & $14.8\pm0.1$ & $14.0\pm0.1$ & $13.6\pm0.1$ & $13.3\pm0.1$ & $14.8\pm0.1$ & $14.1\pm0.1$ & $13.8\pm0.1$ & $13.5\pm0.1$ & $13.3\pm0.1$ & $13.0\pm0.1$ & $12.7\pm0.1$ & $12.8\pm0.1$ & $13.9\pm0.1$ & $14.7\pm0.1$ & SDSS\\
ASASSN-14lv & LCRS B232926.0-413242 & $17.9\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $15.5\pm0.1$ & $15.2\pm0.2$ & $15.3\pm0.2$ & $16.7\pm0.1$ & $17.2\pm0.1$ & --\\
ASASSN-14lw & GALEXASC J010647.95-465904.1 & $21.2\pm0.2$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $20.0\pm0.1$ & -- & --\\
ASASSN-14me & ESO 113-G047 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $17.8\pm0.1$ & $18.3\pm0.1$ & --\\
ASASSN-14mf & GALEXASC J000454.54-322615.3 & $19.1\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $18.0\pm0.1$ & $18.7\pm0.1$ & --\\
ASASSN-14mg & GALEXASC J025358.03-213854.7 & $20.0\pm0.1$ & -- & -- & -- & -- & -- & $17.6\pm0.1$ & $17.0\pm0.1$ & $16.8\pm0.1$ & $16.6\pm0.1$ & $16.5\pm0.1$ & $17.3\pm0.1$ & $17.1\pm0.1$ & $17.1\pm0.2$ & $17.2\pm0.1$ & $17.6\pm0.1$ & PS1\\
ASASSN-14mu & KUG 0923+457 & $18.3\pm0.1$ & $17.4\pm0.1$ & $16.3\pm0.1$ & $15.9\pm0.1$ & $15.7\pm0.1$ & $15.5\pm0.1$ & $17.6\pm0.1$ & -- & -- & $16.4\pm0.1$ & $16.4\pm0.1$ & $17.4\pm0.1$ & $17.0\pm0.1$ & $17.4\pm0.2$ & $17.1\pm0.1$ & $17.5\pm0.1$ & SDSS\\
ASASSN-14mw & AM 0139-655 NED02 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.4\pm0.1$ & $12.2\pm0.1$ & $12.5\pm0.1$ & $13.4\pm0.1$ & $13.9\pm0.1$ & --\\
ASASSN-14my & NGC 3774 & -- & -- & -- & -- & -- & -- & $14.6\pm0.1$ & $13.9\pm0.1$ & $13.8\pm0.1$ & $13.4\pm0.1$ & $13.4\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $13.0\pm0.1$ & $15.2\pm0.1$ & $15.8\pm0.1$ & PS1\\
ASASSN-15ad & PGC 902451 & -- & -- & -- & -- & -- & -- & $17.3\pm0.1$ & $16.6\pm0.1$ & $16.8\pm0.1$ & $16.8\pm0.1$ & $16.4\pm0.1$ & -- & -- & -- & $17.3\pm0.1$ & $18.0\pm0.1$ & PS1\\
ASASSN-15ae & 2MASX J15510599+3425520 & $17.6\pm0.1$ & $17.3\pm0.1$ & $16.0\pm0.1$ & $15.6\pm0.1$ & $15.4\pm0.1$ & $15.3\pm0.1$ & $16.3\pm0.1$ & $15.8\pm0.1$ & $15.7\pm0.1$ & $15.6\pm0.1$ & $15.6\pm0.1$ & $15.9\pm0.1$ & $16.0\pm0.2$ & $16.1\pm0.1$ & $17.0\pm0.1$ & $17.4\pm0.1$ & SDSS\\
ASASSN-15aj & NGC 3449 & $16.2\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $10.6\pm0.1$ & $10.4\pm0.1$ & $10.5\pm0.1$ & $12.3\pm0.1$ & $12.9\pm0.1$ & --\\
ASASSN-15ak & UGC 00110 & $17.0\pm0.1$ & $16.7\pm0.1$ & $15.3\pm0.1$ & $14.9\pm0.1$ & $14.7\pm0.1$ & $14.6\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & $16.7\pm0.1$ & $17.2\pm0.1$ & SDSS\\
ASASSN-15al & GALEXASC J045749.46-213526.3 & $18.9\pm0.1$ & -- & -- & -- & -- & -- & $17.3\pm0.1$ & $16.9\pm0.1$ & $16.6\pm0.1$ & $16.7\pm0.1$ & $17.1\pm0.1$ & -- & -- & -- & $18.0\pm0.1$ & $18.4\pm0.1$ & PS1\\
ASASSN-15ar & CGCG 439-010 & -- & -- & -- & -- & -- & -- & $14.8\pm0.1$ & $14.1\pm0.1$ & $13.8\pm0.1$ & $13.5\pm0.1$ & $13.3\pm0.1$ & $13.2\pm0.1$ & $13.0\pm0.1$ & $13.1\pm0.1$ & $14.8\pm0.1$ & $15.4\pm0.1$ & PS1\\
ASASSN-15as & SDSS J093916.69+062551.1 & $21.7\pm0.1$ & $21.0\pm0.2$ & $19.9\pm0.1$ & $19.6\pm0.1$ & $19.4\pm0.1$ & $19.6\pm0.2$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & SDSS\\
ASASSN-15az & 2MASX J11083863-1014456 & $21.8\pm0.5$ & -- & -- & -- & -- & -- & $16.3\pm0.1$ & $15.6\pm0.1$ & $15.2\pm0.1$ & $15.0\pm0.1$ & $14.8\pm0.1$ & $14.7\pm0.1$ & $14.4\pm0.1$ & $14.5\pm0.1$ & $15.7\pm0.1$ & $16.4\pm0.1$ & PS1\\
ASASSN-15ba & SDSS J140455.12+085514.0 & $19.8\pm0.1$ & $19.2\pm0.1$ & $18.0\pm0.1$ & $17.6\pm0.1$ & $17.4\pm0.1$ & $17.2\pm0.1$ & $18.1\pm0.1$ & $17.7\pm0.1$ & $17.5\pm0.1$ & $17.5\pm0.1$ & $18.1\pm0.1$ & -- & -- & -- & $19.1\pm0.1$ & $19.5\pm0.2$ & SDSS\\
ASASSN-15bc & 2MASX J04061478-0853112 & -- & -- & -- & -- & -- & -- & $15.8\pm0.1$ & $15.1\pm0.1$ & $14.9\pm0.1$ & $14.8\pm0.1$ & $14.9\pm0.1$ & $14.9\pm0.1$ & $14.7\pm0.1$ & $14.9\pm0.1$ & $15.8\pm0.1$ & $16.3\pm0.1$ & PS1\\
ASASSN-15be & GALEXASC J025245.83-341850.6 & $18.6\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $18.3\pm0.1$ & $18.7\pm0.1$ & --\\
ASASSN-15bf & 2MASX J04384102-4137212 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $14.7\pm0.1$ & $14.6\pm0.1$ & $14.8\pm0.1$ & $15.3\pm0.1$ & $15.9\pm0.1$ & --\\
ASASSN-15bk & CGCG 078-056 & $18.2\pm0.1$ & $17.1\pm0.1$ & $15.7\pm0.1$ & $14.9\pm0.1$ & $14.5\pm0.1$ & $14.2\pm0.1$ & $15.8\pm0.1$ & $15.2\pm0.1$ & $14.8\pm0.1$ & $14.7\pm0.1$ & $14.5\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $14.2\pm0.1$ & $15.2\pm0.1$ & $15.7\pm0.1$ & SDSS\\
ASASSN-15bm & GALEXASC J150551.56-053737.2 & $17.9\pm0.1$ & -- & -- & -- & -- & -- & $15.6\pm0.1$ & $14.9\pm0.1$ & $14.6\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $13.8\pm0.1$ & $13.7\pm0.1$ & $13.7\pm0.1$ & $14.9\pm0.1$ & $15.5\pm0.1$ & PS1\\
ASASSN-15bn & GALEXASC J155536.57+664316.5 & $18.8\pm0.1$ & -- & -- & -- & -- & -- & $17.0\pm0.1$ & $16.5\pm0.1$ & $16.3\pm0.1$ & $16.2\pm0.1$ & $16.4\pm0.1$ & -- & -- & -- & $17.9\pm0.1$ & $18.5\pm0.1$ & PS1\\
ASASSN-15bo & SDSS J144455.21+243443.9 & $20.7\pm0.3$ & $19.7\pm0.1$ & $18.7\pm0.1$ & $18.3\pm0.1$ & $18.1\pm0.1$ & $17.9\pm0.1$ & $18.7\pm0.1$ & $18.4\pm0.1$ & $18.1\pm0.1$ & $18.0\pm0.1$ & $18.0\pm0.1$ & -- & -- & -- & $18.5\pm0.1$ & $19.3\pm0.1$ & SDSS\\
ASASSN-15cb & VCC 1810 & $17.6\pm0.1$ & $16.8\pm0.1$ & $15.6\pm0.1$ & $15.1\pm0.1$ & $14.8\pm0.1$ & $14.7\pm0.1$ & $15.7\pm0.1$ & $15.2\pm0.1$ & $15.0\pm0.1$ & $14.8\pm0.1$ & $14.6\pm0.1$ & $14.6\pm0.1$ & $14.3\pm0.1$ & $14.8\pm0.1$ & $15.4\pm0.1$ & $15.9\pm0.1$ & SDSS\\
ASASSN-15cd & CGCG 064-017 & $17.6\pm0.1$ & $16.3\pm0.1$ & $15.3\pm0.1$ & $15.0\pm0.1$ & $15.8\pm0.1$ & $15.3\pm0.1$ & $15.5\pm0.1$ & $15.2\pm0.1$ & $15.0\pm0.1$ & $15.0\pm0.1$ & $14.9\pm0.1$ & $15.0\pm0.1$ & $14.9\pm0.1$ & $15.1\pm0.1$ & $15.6\pm0.1$ & $15.7\pm0.1$ & PS1\\
ASASSN-15cq & CGCG 218-007 & $19.1\pm0.1$ & $16.5\pm0.1$ & $14.9\pm0.1$ & $14.1\pm0.1$ & $13.7\pm0.1$ & $13.4\pm0.1$ & $14.9\pm0.1$ & $14.3\pm0.1$ & $13.9\pm0.1$ & $13.7\pm0.1$ & $13.5\pm0.1$ & $13.3\pm0.1$ & $13.1\pm0.1$ & $13.1\pm0.1$ & $14.0\pm0.1$ & $14.3\pm0.1$ & SDSS\\
ASASSN-15cz & SBS 1132+579 & -- & $16.0\pm0.1$ & $14.6\pm0.1$ & $13.9\pm0.1$ & $13.5\pm0.1$ & $13.3\pm0.1$ & $14.4\pm0.1$ & $13.9\pm0.1$ & $13.5\pm0.1$ & $13.5\pm0.1$ & $13.2\pm0.1$ & $13.0\pm0.1$ & $12.7\pm0.1$ & $12.8\pm0.1$ & $13.7\pm0.1$ & $14.1\pm0.1$ & SDSS\\
ASASSN-15da & 2MASX J05235186-2442081 & -- & -- & -- & -- & -- & -- & $17.5\pm0.1$ & $16.8\pm0.1$ & $16.5\pm0.1$ & $16.2\pm0.1$ & $16.0\pm0.1$ & $15.8\pm0.1$ & $15.4\pm0.1$ & $15.4\pm0.1$ & $16.5\pm0.1$ & $17.0\pm0.1$ & PS1\\
ASASSN-15db & NGC 5996 & $14.4\pm0.1$ & $15.1\pm0.1$ & $14.6\pm0.1$ & $14.4\pm0.1$ & $14.6\pm0.1$ & $14.1\pm0.1$ & $12.9\pm0.1$ & $12.6\pm0.1$ & $12.4\pm0.1$ & $12.3\pm0.1$ & $12.2\pm0.1$ & $12.5\pm0.1$ & $12.4\pm0.1$ & $12.5\pm0.1$ & $14.0\pm0.1$ & $14.3\pm0.1$ & PS1\\
ASASSN-15dc & SDSS J150130.77-003222.8 & $19.4\pm0.1$ & $18.6\pm0.1$ & $17.4\pm0.1$ & $17.0\pm0.1$ & $16.8\pm0.1$ & $16.5\pm0.1$ & $17.5\pm0.1$ & $17.1\pm0.1$ & $16.9\pm0.1$ & $16.8\pm0.1$ & $16.8\pm0.1$ & -- & -- & -- & $17.8\pm0.1$ & $18.3\pm0.1$ & SDSS\\
ASASSN-15dd & CGCG 107-031 & $20.2\pm0.1$ & $16.7\pm0.1$ & $14.9\pm0.1$ & $14.1\pm0.1$ & $13.6\pm0.1$ & $13.3\pm0.1$ & $15.1\pm0.1$ & $14.3\pm0.1$ & $13.9\pm0.1$ & $13.7\pm0.1$ & $13.6\pm0.1$ & $13.3\pm0.1$ & $13.1\pm0.1$ & $13.3\pm0.1$ & $14.5\pm0.1$ & $15.2\pm0.1$ & SDSS\\
ASASSN-15de & SDSS J112849.43+295454.2 & -- & $18.8\pm0.1$ & $17.8\pm0.1$ & $17.7\pm0.1$ & $17.7\pm0.1$ & $17.6\pm0.1$ & $15.8\pm0.1$ & $15.4\pm0.1$ & $15.2\pm0.1$ & $15.1\pm0.1$ & $15.0\pm0.1$ & $14.8\pm0.1$ & $14.7\pm0.1$ & $14.8\pm0.1$ & $16.3\pm0.1$ & $16.6\pm0.1$ & PS1\\
ASASSN-15df & SDSS J103529.47+343420.2 & $19.3\pm0.1$ & $19.1\pm0.1$ & $18.0\pm0.1$ & $17.6\pm0.1$ & $17.4\pm0.1$ & $17.4\pm0.1$ & $18.4\pm0.1$ & $17.9\pm0.1$ & $17.8\pm0.1$ & $17.9\pm0.1$ & $18.9\pm0.1$ & -- & -- & -- & $19.2\pm0.1$ & $20.1\pm0.3$ & SDSS\\
ASASSN-15dz & CGCG 080-055 & $16.9\pm0.1$ & $16.4\pm0.1$ & $15.2\pm0.1$ & $14.7\pm0.1$ & $14.4\pm0.1$ & $14.1\pm0.1$ & $15.1\pm0.1$ & $14.6\pm0.1$ & $14.5\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $14.1\pm0.1$ & $13.9\pm0.1$ & $14.1\pm0.1$ & $15.2\pm0.1$ & $15.8\pm0.1$ & SDSS\\
ASASSN-15eb & ESO 561-G012 & $20.2\pm0.2$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $11.5\pm0.1$ & $11.2\pm0.1$ & $11.4\pm0.1$ & $12.8\pm0.1$ & $13.5\pm0.1$ & --\\
ASASSN-15fa & NGC 6319 & $17.1\pm0.1$ & $15.7\pm0.1$ & $13.9\pm0.1$ & $13.1\pm0.1$ & $12.7\pm0.1$ & $12.4\pm0.1$ & $14.2\pm0.1$ & $13.4\pm0.1$ & $13.1\pm0.1$ & $12.8\pm0.1$ & $12.6\pm0.1$ & $12.4\pm0.1$ & $12.1\pm0.1$ & $12.3\pm0.1$ & $13.6\pm0.1$ & $14.2\pm0.1$ & SDSS\\
ASASSN-15fj & 2MASX J17100856+7443426 & $21.8\pm0.4$ & $18.1\pm0.1$ & $16.3\pm0.1$ & $15.6\pm0.1$ & $15.2\pm0.1$ & $14.9\pm0.1$ & $16.3\pm0.1$ & $15.7\pm0.1$ & $15.3\pm0.1$ & $15.1\pm0.1$ & $15.0\pm0.1$ & $14.7\pm0.1$ & $14.6\pm0.1$ & $14.7\pm0.1$ & $15.7\pm0.1$ & $16.3\pm0.1$ & SDSS\\
ASASSN-15fk & 2MASX J05401415-3848285 & $20.7\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.6\pm0.1$ & $13.4\pm0.1$ & $13.5\pm0.1$ & $14.6\pm0.1$ & $15.3\pm0.1$ & --\\
ASASSN-15fr & 2MASX J09202045-0738229 & -- & -- & -- & -- & -- & -- & $15.9\pm0.1$ & $15.4\pm0.1$ & $15.3\pm0.1$ & $15.1\pm0.1$ & $15.1\pm0.1$ & $15.2\pm0.1$ & $15.0\pm0.1$ & $15.1\pm0.1$ & $16.5\pm0.1$ & $17.1\pm0.1$ & PS1\\
ASASSN-15fs & CGCG 229-010 & $18.6\pm0.1$ & -- & -- & -- & -- & -- & $15.6\pm0.1$ & $15.1\pm0.1$ & $14.7\pm0.1$ & $14.5\pm0.1$ & $14.2\pm0.1$ & $13.9\pm0.1$ & $13.7\pm0.1$ & $13.8\pm0.1$ & $14.8\pm0.1$ & $15.2\pm0.1$ & PS1\\
ASASSN-15fy & Uncatalogued & $22.4\pm0.3$ & -- & -- & -- & -- & -- & $20.7\pm0.1$ & $20.3\pm0.1$ & $21.3\pm0.1$ & $21.4\pm0.1$ & $21.8\pm0.1$ & -- & -- & -- & -- & -- & PS1\\
ASASSN-15ga & NGC 4866 & $16.4\pm0.1$ & $14.3\pm0.1$ & $12.3\pm0.1$ & $11.4\pm0.1$ & $10.9\pm0.1$ & $10.6\pm0.1$ & -- & -- & -- & -- & -- & $ 9.8\pm0.1$ & $ 9.6\pm0.1$ & $ 9.8\pm0.1$ & $12.1\pm0.1$ & $12.8\pm0.1$ & SDSS\\
ASASSN-15go & 2MASX J06113048-1629085 & -- & -- & -- & -- & -- & -- & $15.4\pm0.1$ & $14.7\pm0.1$ & $14.4\pm0.1$ & $14.1\pm0.1$ & $13.9\pm0.1$ & $13.6\pm0.1$ & $13.4\pm0.1$ & $13.5\pm0.1$ & $14.6\pm0.1$ & $15.2\pm0.1$ & PS1\\
ASASSN-15gr & ESO 366-G015 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $17.3\pm0.1$ & $17.9\pm0.1$ & --\\
ASASSN-15gw & NGC 5536 & $16.8\pm0.1$ & $15.4\pm0.1$ & $14.0\pm0.1$ & $13.3\pm0.1$ & $13.0\pm0.1$ & $12.7\pm0.1$ & $14.2\pm0.1$ & $13.5\pm0.1$ & $13.3\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $12.7\pm0.1$ & $12.4\pm0.1$ & $12.6\pm0.1$ & $13.8\pm0.1$ & $14.3\pm0.1$ & SDSS\\
ASASSN-15gz & 2MASX J14423254-1327294 & $21.2\pm0.3$ & -- & -- & -- & -- & -- & $15.9\pm0.1$ & $15.1\pm0.1$ & $14.7\pm0.1$ & $14.5\pm0.1$ & $14.3\pm0.1$ & $14.2\pm0.1$ & $13.9\pm0.1$ & $14.1\pm0.1$ & $14.9\pm0.1$ & $15.6\pm0.1$ & PS1\\
ASASSN-15hc & LCRS B102206.7-024353 & $18.2\pm0.1$ & $17.2\pm0.1$ & $16.1\pm0.1$ & $15.6\pm0.1$ & $15.3\pm0.1$ & $15.1\pm0.1$ & $16.0\pm0.1$ & $15.6\pm0.1$ & $15.4\pm0.1$ & $15.2\pm0.1$ & $15.1\pm0.1$ & $14.9\pm0.1$ & $14.8\pm0.1$ & $14.8\pm0.1$ & $16.1\pm0.1$ & $16.7\pm0.1$ & SDSS\\
ASASSN-15he & ESO 069-G005 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $15.1\pm0.1$ & $14.8\pm0.1$ & $15.2\pm0.1$ & $16.5\pm0.1$ & $17.1\pm0.1$ & --\\
ASASSN-15hf & ESO 375-G041 & $19.2\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.5\pm0.1$ & $12.3\pm0.1$ & $12.5\pm0.1$ & $13.9\pm0.1$ & $14.6\pm0.1$ & --\\
ASASSN-15hg & CGCG 063-098 & $19.4\pm0.1$ & $17.1\pm0.1$ & $15.3\pm0.1$ & $14.5\pm0.1$ & $14.0\pm0.1$ & $13.7\pm0.1$ & $15.4\pm0.1$ & $14.7\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $13.8\pm0.1$ & $13.6\pm0.1$ & $13.4\pm0.1$ & $13.5\pm0.1$ & $14.6\pm0.1$ & $15.3\pm0.1$ & SDSS\\
ASASSN-15hh & NGC 2115A & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.7\pm0.1$ & $12.5\pm0.1$ & $12.6\pm0.1$ & $13.6\pm0.1$ & $14.2\pm0.1$ & --\\
ASASSN-15ho & 2MASXi J0909234-044327 & $17.7\pm0.1$ & -- & -- & -- & -- & -- & $16.5\pm0.1$ & $16.0\pm0.1$ & $15.8\pm0.1$ & $15.8\pm0.1$ & $15.7\pm0.1$ & -- & -- & -- & $16.7\pm0.1$ & $17.2\pm0.1$ & PS1\\
ASASSN-15hx & GALEXASC J134316.80-313318.2 & $19.0\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $17.5\pm0.1$ & $18.0\pm0.1$ & --\\
ASASSN-15hy & Uncatalogued & $22.4\pm0.3$ & -- & -- & -- & -- & -- & $18.5\pm0.1$ & $18.1\pm0.1$ & $17.8\pm0.1$ & $17.8\pm0.1$ & $17.9\pm0.1$ & -- & -- & -- & -- & -- & PS1\\
ASASSN-15hz & APMUKS B222606.49-654315.6 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $17.6\pm0.1$ & $18.1\pm0.1$ & --\\
ASASSN-15ic & 2MASX J06145320-4247357 & $22.3\pm0.6$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $14.9\pm0.1$ & $14.6\pm0.1$ & $14.8\pm0.1$ & $15.5\pm0.1$ & $16.1\pm0.1$ & --\\
ASASSN-15ih & GALEXASC J095959.71-025322.1 & $17.7\pm0.1$ & $18.2\pm0.1$ & $16.1\pm0.1$ & $15.7\pm0.1$ & $15.5\pm0.1$ & $15.3\pm0.1$ & $16.2\pm0.1$ & $15.9\pm0.1$ & $15.7\pm0.1$ & $15.3\pm0.1$ & $15.4\pm0.1$ & -- & -- & -- & $17.0\pm0.1$ & $17.5\pm0.1$ & PS1\\
ASASSN-15il & 2MASX J15570808-1240252 & $20.6\pm0.2$ & -- & -- & -- & -- & -- & $15.9\pm0.1$ & $15.2\pm0.1$ & $14.8\pm0.1$ & $14.6\pm0.1$ & $14.4\pm0.1$ & $14.1\pm0.1$ & $13.8\pm0.1$ & $14.0\pm0.1$ & $15.1\pm0.1$ & $15.7\pm0.1$ & PS1\\
ASASSN-15ja & ESO 113-G018 & $19.3\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.9\pm0.1$ & $12.6\pm0.1$ & $12.8\pm0.1$ & $13.9\pm0.1$ & $14.6\pm0.1$ & --\\
ASASSN-15jb & 2MASX J11200680+3407396 & $21.9\pm0.4$ & $17.9\pm0.1$ & $16.1\pm0.1$ & $15.2\pm0.1$ & $14.8\pm0.1$ & $14.5\pm0.1$ & $16.1\pm0.1$ & $15.3\pm0.1$ & $15.0\pm0.1$ & $14.7\pm0.1$ & $14.4\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $14.3\pm0.1$ & $15.4\pm0.1$ & $16.1\pm0.1$ & SDSS\\
ASASSN-15jf & GALEXASC J222510.84-502347.7 & $21.0\pm0.2$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $20.0\pm0.1$ & $20.1\pm12.5$ & --\\
ASASSN-15jg & SDSS J104655.44-021927.0 & $19.8\pm0.1$ & $18.8\pm0.1$ & $17.8\pm0.1$ & $17.4\pm0.1$ & $17.2\pm0.1$ & $17.1\pm0.1$ & $17.8\pm0.1$ & $17.4\pm0.1$ & $17.2\pm0.1$ & $17.1\pm0.1$ & $17.1\pm0.1$ & -- & -- & -- & $17.8\pm0.1$ & $18.2\pm0.1$ & SDSS\\
ASASSN-15ji & ESO 536-G008 & $18.0\pm0.1$ & -- & -- & -- & -- & -- & $15.6\pm0.1$ & $15.0\pm0.1$ & $14.5\pm0.1$ & $14.4\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $13.7\pm0.1$ & $13.8\pm0.1$ & $14.8\pm0.1$ & $15.4\pm0.1$ & PS1\\
ASASSN-15jl & SDSS J152241.16+505836.0 & -- & $19.2\pm0.1$ & $18.1\pm0.1$ & $17.7\pm0.1$ & $17.4\pm0.1$ & $17.3\pm0.1$ & $18.1\pm0.1$ & $17.7\pm0.1$ & $17.4\pm0.1$ & $17.4\pm0.1$ & $17.4\pm0.1$ & -- & -- & -- & $18.3\pm0.1$ & $18.8\pm0.1$ & SDSS\\
ASASSN-15jm & 2MASX J17210913+2534558 & -- & $17.1\pm0.1$ & $16.0\pm0.1$ & $15.5\pm0.1$ & $15.1\pm0.1$ & $14.9\pm0.1$ & $15.9\pm0.1$ & $15.4\pm0.1$ & $15.2\pm0.1$ & $15.1\pm0.1$ & $15.0\pm0.1$ & $15.0\pm0.1$ & $14.9\pm0.1$ & $14.9\pm0.1$ & $15.8\pm0.1$ & $16.3\pm0.1$ & SDSS\\
ASASSN-15jo & ALLWISE J140643.89-342721.4 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $18.4\pm0.1$ & $19.5\pm0.2$ & --\\
ASASSN-15js & 2MFGC 08437 & $18.8\pm0.1$ & $18.1\pm0.1$ & $16.3\pm0.1$ & $15.8\pm0.1$ & $15.4\pm0.1$ & $15.2\pm0.1$ & $16.4\pm0.1$ & $15.9\pm0.1$ & $15.6\pm0.1$ & $15.5\pm0.1$ & $15.3\pm0.1$ & $15.5\pm0.1$ & $15.4\pm0.1$ & $15.5\pm0.1$ & $16.7\pm0.1$ & $17.3\pm0.1$ & SDSS\\
ASASSN-15jt & 2MASX J13080914+2749354 & $20.7\pm0.1$ & $17.1\pm0.1$ & $15.4\pm0.1$ & $14.7\pm0.1$ & $14.3\pm0.1$ & $14.0\pm0.1$ & $15.7\pm0.1$ & $15.0\pm0.1$ & $14.6\pm0.1$ & $14.4\pm0.1$ & $14.2\pm0.1$ & $14.3\pm0.1$ & $14.4\pm0.1$ & $14.4\pm0.1$ & $15.4\pm0.1$ & $16.1\pm0.1$ & SDSS\\
ASASSN-15ke & 2MASX J15254441+5921091 & $18.0\pm0.1$ & $17.1\pm0.1$ & $15.9\pm0.1$ & $15.3\pm0.1$ & $15.0\pm0.1$ & $14.7\pm0.1$ & $16.0\pm0.1$ & $15.5\pm0.1$ & $15.2\pm0.1$ & $15.1\pm0.1$ & $15.0\pm0.1$ & $14.9\pm0.1$ & $14.6\pm0.1$ & $14.8\pm0.1$ & $15.5\pm0.1$ & $16.1\pm0.1$ & SDSS\\
ASASSN-15kg & 2MASX J08401168-0435369 & $16.0\pm0.1$ & -- & -- & -- & -- & -- & $14.0\pm0.1$ & $13.5\pm0.1$ & $13.2\pm0.1$ & $13.1\pm0.1$ & $12.9\pm0.1$ & $12.8\pm0.1$ & $12.5\pm0.1$ & $12.8\pm0.1$ & $14.5\pm0.1$ & $15.0\pm0.1$ & PS1\\
ASASSN-15kk & UGC 04883 & $17.4\pm0.1$ & -- & -- & -- & -- & -- & $13.4\pm0.1$ & $12.8\pm0.1$ & $12.5\pm0.1$ & $12.3\pm0.1$ & $12.1\pm0.1$ & $11.8\pm0.1$ & $11.6\pm0.1$ & $11.8\pm0.1$ & $12.9\pm0.1$ & $13.4\pm0.1$ & PS1\\
ASASSN-15kn & 2MASX J12415081-0710092 & $19.9\pm0.2$ & $17.0\pm0.1$ & $15.2\pm0.1$ & $14.3\pm0.1$ & $13.8\pm0.1$ & $13.5\pm0.1$ & $18.5\pm0.1$ & $14.4\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $13.6\pm0.1$ & $13.3\pm0.1$ & $13.0\pm0.1$ & $13.0\pm0.1$ & $14.3\pm0.1$ & $14.7\pm0.1$ & SDSS\\
ASASSN-15kp & AM 1255-315 & $19.9\pm0.2$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.6\pm0.1$ & $12.4\pm0.1$ & $12.7\pm0.1$ & $13.8\pm0.1$ & $14.5\pm0.1$ & --\\
ASASSN-15kq & GALEXASC J064843.83-541213.4 & $19.3\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $14.7\pm0.1$ & $14.4\pm0.1$ & $14.4\pm0.1$ & $13.0\pm0.1$ & $13.7\pm0.1$ & --\\
ASASSN-15kx & MCG +06-49-001 & $21.7\pm0.3$ & -- & -- & -- & -- & -- & $15.0\pm0.1$ & $14.2\pm0.1$ & $13.7\pm0.1$ & $13.4\pm0.1$ & $13.3\pm0.1$ & $12.9\pm0.1$ & $12.6\pm0.1$ & $12.7\pm0.1$ & $14.1\pm0.1$ & $14.8\pm0.1$ & PS1\\
ASASSN-15la & NGC 5517 & $17.1\pm0.1$ & $15.7\pm0.1$ & $14.0\pm0.1$ & $13.3\pm0.1$ & $12.9\pm0.1$ & $12.7\pm0.1$ & $14.7\pm0.1$ & $13.7\pm0.1$ & $13.3\pm0.1$ & $13.1\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $12.6\pm0.1$ & $12.8\pm0.1$ & $14.0\pm0.1$ & $14.6\pm0.1$ & SDSS\\
ASASSN-15lg & CGCG 044-042 & $18.3\pm0.1$ & $17.1\pm0.1$ & $15.7\pm0.1$ & $15.0\pm0.1$ & $14.7\pm0.1$ & $14.4\pm0.1$ & $15.6\pm0.1$ & $15.0\pm0.1$ & $14.8\pm0.1$ & $14.6\pm0.1$ & $14.4\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $14.2\pm0.1$ & $15.5\pm0.1$ & $16.0\pm0.1$ & SDSS\\
ASASSN-15li & 2MASX J14250783+6253235 & $19.1\pm0.1$ & $17.8\pm0.1$ & $16.5\pm0.1$ & $15.9\pm0.1$ & $15.6\pm0.1$ & $15.3\pm0.1$ & $16.7\pm0.1$ & $16.2\pm0.1$ & $15.9\pm0.1$ & $15.7\pm0.1$ & $15.4\pm0.1$ & $15.4\pm0.1$ & $15.1\pm0.1$ & $15.3\pm0.1$ & $15.9\pm0.1$ & $16.4\pm0.1$ & SDSS\\
ASASSN-15lo & GALEXASC J225332.83+194232.9 & -- & $18.1\pm0.1$ & $17.0\pm0.1$ & $16.5\pm0.1$ & $16.3\pm0.1$ & $16.1\pm0.1$ & $17.0\pm0.1$ & $16.5\pm0.1$ & $16.3\pm0.1$ & $16.5\pm0.1$ & $16.3\pm0.1$ & $16.1\pm0.1$ & $15.8\pm0.1$ & $16.0\pm0.2$ & $17.2\pm0.1$ & $17.8\pm0.1$ & SDSS\\
ASASSN-15lp & MRK 0576 & $17.1\pm0.1$ & $16.2\pm0.1$ & $15.2\pm0.1$ & $14.7\pm0.1$ & $14.5\pm0.1$ & $14.2\pm0.1$ & $15.1\pm0.1$ & $14.7\pm0.1$ & $14.4\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $14.0\pm0.1$ & $14.7\pm0.1$ & $15.2\pm0.1$ & SDSS\\
ASASSN-15lu & 2MASX J13211289+4015564 & $18.4\pm0.1$ & $17.2\pm0.1$ & $16.1\pm0.1$ & $15.6\pm0.1$ & $15.2\pm0.1$ & $15.0\pm0.1$ & $16.2\pm0.1$ & $15.7\pm0.1$ & $15.5\pm0.1$ & $15.3\pm0.1$ & $15.0\pm0.1$ & $15.0\pm0.1$ & $14.8\pm0.1$ & $14.9\pm0.1$ & $15.5\pm0.1$ & $15.9\pm0.1$ & SDSS\\
ASASSN-15mc & UGC 02295 & -- & $15.5\pm0.1$ & $13.9\pm0.1$ & $13.0\pm0.1$ & $12.6\pm0.1$ & $12.3\pm0.1$ & -- & $13.5\pm0.1$ & $12.8\pm0.1$ & $12.5\pm0.1$ & $12.5\pm0.1$ & $11.9\pm0.1$ & $11.6\pm0.1$ & $11.8\pm0.1$ & $13.4\pm0.1$ & $14.0\pm0.1$ & SDSS\\
ASASSN-15mf & UGC 09108 NED02 & -- & $17.5\pm0.1$ & $15.6\pm0.1$ & $14.8\pm0.1$ & $14.4\pm0.1$ & $14.1\pm0.1$ & $14.9\pm0.1$ & $14.1\pm0.1$ & $13.8\pm0.1$ & $16.5\pm0.1$ & $15.2\pm0.1$ & $12.9\pm0.1$ & $12.6\pm0.1$ & $12.8\pm0.1$ & $15.9\pm0.1$ & $16.5\pm0.1$ & SDSS\\
ASASSN-15mg & 2MASX J15322270+4150586 & $19.2\pm0.1$ & $18.0\pm0.1$ & $16.6\pm0.1$ & $15.9\pm0.1$ & $15.5\pm0.1$ & $15.3\pm0.1$ & $16.8\pm0.1$ & $16.1\pm0.1$ & $15.8\pm0.1$ & $15.6\pm0.1$ & $15.5\pm0.1$ & $15.4\pm0.1$ & $15.2\pm0.1$ & $15.6\pm0.1$ & $16.7\pm0.1$ & $17.2\pm0.1$ & SDSS\\
ASASSN-15mi & MRK 0283a & $17.4\pm0.1$ & $17.0\pm0.1$ & $16.2\pm0.1$ & $15.9\pm0.1$ & $15.7\pm0.1$ & $15.5\pm0.1$ & $16.6\pm0.1$ & $16.3\pm0.1$ & $16.2\pm0.1$ & $16.1\pm0.1$ & $15.9\pm0.1$ & $15.9\pm0.1$ & $15.7\pm0.1$ & $15.9\pm0.1$ & $16.6\pm0.1$ & $17.1\pm0.1$ & SDSS\\
ASASSN-15ml & 2MASX J20030163-2154516 & $18.9\pm0.1$ & -- & -- & -- & -- & -- & $15.7\pm0.1$ & $15.0\pm0.1$ & $14.7\pm0.1$ & $14.4\pm0.1$ & $14.0\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $13.9\pm0.1$ & $15.2\pm0.1$ & $15.9\pm0.1$ & PS1\\
ASASSN-15mp & 2MASX J00584521-1404122 & $21.5\pm0.3$ & -- & -- & -- & -- & -- & $16.6\pm0.1$ & $16.0\pm0.1$ & $15.7\pm0.1$ & $15.4\pm0.1$ & $15.3\pm0.1$ & $15.2\pm0.1$ & $14.9\pm0.1$ & $14.9\pm0.1$ & $16.5\pm0.1$ & $17.1\pm0.1$ & PS1\\
ASASSN-15mq & 2MASX J05014660-1343503 & $21.4\pm0.3$ & -- & -- & -- & -- & -- & $15.9\pm0.1$ & $15.2\pm0.1$ & $14.7\pm0.1$ & $14.5\pm0.1$ & $14.3\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $14.0\pm0.1$ & $15.1\pm0.1$ & $15.8\pm0.1$ & PS1\\
ASASSN-15ms & SDSS J145027.61+063713.3 & $18.5\pm0.1$ & $18.2\pm0.1$ & $17.3\pm0.1$ & $17.0\pm0.1$ & $16.8\pm0.1$ & $16.7\pm0.1$ & $17.1\pm0.1$ & $16.8\pm0.1$ & $16.7\pm0.1$ & $16.7\pm0.1$ & $16.7\pm0.1$ & -- & -- & -- & $17.7\pm0.1$ & $18.1\pm0.1$ & SDSS\\
ASASSN-15mx & SDSS J142443.90+260255.4 & $19.3\pm0.1$ & $19.0\pm0.1$ & $17.5\pm0.1$ & $17.2\pm0.1$ & $17.0\pm0.1$ & $17.1\pm0.1$ & $17.5\pm0.1$ & $17.2\pm0.1$ & $17.1\pm0.1$ & $17.0\pm0.1$ & $17.2\pm0.1$ & -- & -- & -- & $18.2\pm0.1$ & $18.6\pm0.1$ & SDSS\\
ASASSN-15nh & 2MASX J00443129-0301012 & $19.6\pm0.1$ & $16.7\pm0.1$ & $14.9\pm0.1$ & $14.1\pm0.1$ & $13.8\pm0.1$ & $13.5\pm0.1$ & $14.9\pm0.1$ & $14.3\pm0.1$ & $13.9\pm0.1$ & $13.7\pm0.1$ & $13.5\pm0.1$ & $13.3\pm0.1$ & $13.0\pm0.1$ & $13.2\pm0.1$ & $14.2\pm0.1$ & $14.8\pm0.1$ & SDSS\\
ASASSN-15nn & UGC 01332 & -- & -- & -- & -- & -- & -- & $14.2\pm0.1$ & $13.3\pm0.1$ & $12.8\pm0.1$ & $12.4\pm0.1$ & $12.4\pm0.1$ & $11.6\pm0.1$ & $11.3\pm0.1$ & $11.5\pm0.1$ & $13.3\pm0.1$ & $14.0\pm0.1$ & PS1\\
ASASSN-15np & 2MASX J15060265+0733415 & $21.4\pm0.1$ & $18.6\pm0.1$ & $17.0\pm0.1$ & $16.1\pm0.1$ & $15.7\pm0.1$ & $15.3\pm0.1$ & $17.2\pm0.1$ & $16.4\pm0.1$ & $16.0\pm0.1$ & $15.7\pm0.1$ & $15.6\pm0.1$ & $15.4\pm0.1$ & $15.2\pm0.1$ & $15.1\pm0.1$ & $15.7\pm0.1$ & $16.0\pm0.1$ & SDSS\\
ASASSN-15nq & 2MFGC 13779 & -- & $17.9\pm0.1$ & $15.9\pm0.1$ & $15.0\pm0.1$ & $14.4\pm0.1$ & $14.0\pm0.1$ & $16.0\pm0.1$ & $15.3\pm0.1$ & $14.8\pm0.1$ & $14.5\pm0.1$ & $14.2\pm0.1$ & $13.9\pm0.1$ & $13.6\pm0.1$ & $13.7\pm0.1$ & $14.6\pm0.1$ & $15.3\pm0.1$ & SDSS\\
ASASSN-15nr & CGCG 082-031 & $18.5\pm0.1$ & -- & -- & -- & -- & -- & $15.4\pm0.1$ & $14.8\pm0.1$ & $14.4\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $13.5\pm0.1$ & $13.7\pm0.1$ & $14.5\pm0.1$ & $15.0\pm0.1$ & PS1\\
ASASSN-15ns & MRK 0887 & $19.9\pm0.1$ & $16.0\pm0.1$ & $14.1\pm0.1$ & $13.3\pm0.1$ & $12.9\pm0.1$ & $12.6\pm0.1$ & $14.3\pm0.1$ & $13.6\pm0.1$ & $13.2\pm0.1$ & $13.0\pm0.1$ & $13.7\pm0.1$ & $12.5\pm0.1$ & $12.2\pm0.1$ & $12.5\pm0.1$ & $13.2\pm0.1$ & $14.3\pm0.1$ & SDSS\\
ASASSN-15od & MCG -01-07-004 & $16.3\pm0.1$ & $15.7\pm0.1$ & $14.7\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $13.7\pm0.1$ & $14.6\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $14.0\pm0.1$ & $14.1\pm0.1$ & $14.0\pm0.1$ & $13.9\pm0.1$ & $14.2\pm0.1$ & $15.5\pm0.1$ & $16.1\pm0.1$ & SDSS\\
ASASSN-15og & GALEXASC J032107.24-311845.8 & $20.5\pm0.1$ & -- & -- & -- & -- & -- & $18.0\pm0.1$ & $17.5\pm0.1$ & $17.1\pm0.1$ & $17.2\pm0.1$ & $17.1\pm0.1$ & -- & -- & -- & $17.2\pm0.1$ & $17.8\pm0.1$ & PS1\\
ASASSN-15oh & MCG +06-49-027 & -- & $16.4\pm0.1$ & $14.6\pm0.1$ & $13.7\pm0.1$ & $13.2\pm0.1$ & $12.9\pm0.1$ & $15.1\pm0.1$ & $14.1\pm0.1$ & $13.7\pm0.1$ & $13.4\pm0.1$ & $13.2\pm0.1$ & $12.8\pm0.1$ & $12.5\pm0.1$ & $12.7\pm0.1$ & $13.8\pm0.1$ & $14.6\pm0.1$ & SDSS\\
ASASSN-15ol & NGC 0745 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $11.7\pm0.1$ & $11.5\pm0.1$ & $11.7\pm0.1$ & -- & -- & --\\
ASASSN-15om & LCRS B021111.4-453206 & $18.0\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $15.0\pm0.1$ & $14.5\pm0.1$ & $14.6\pm0.1$ & $14.6\pm0.1$ & $15.0\pm0.1$ & --\\
ASASSN-15on & SDSS J163636.15+553311.0 & $21.4\pm0.3$ & $19.8\pm0.1$ & $18.6\pm0.1$ & $18.1\pm0.1$ & $17.9\pm0.1$ & $17.7\pm0.1$ & $18.6\pm0.1$ & $18.1\pm0.1$ & $17.9\pm0.1$ & $17.8\pm0.1$ & $17.6\pm0.1$ & -- & -- & -- & $18.6\pm0.1$ & $19.1\pm0.1$ & SDSS\\
ASASSN-15os & GALEXASC J205408.07-551628.8 & $19.8\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $18.7\pm0.1$ & $19.1\pm0.1$ & --\\
ASASSN-15ou & None & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $19.7\pm0.1$ & $20.3\pm0.1$ & --\\
ASASSN-15ox & LSBG F418-058 & $17.9\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $16.8\pm0.1$ & $17.2\pm0.1$ & --\\
ASASSN-15pe & CGCG 226-005 & $19.4\pm0.1$ & $15.9\pm0.1$ & $13.9\pm0.1$ & $13.0\pm0.1$ & $12.6\pm0.1$ & $12.3\pm0.1$ & $14.1\pm0.1$ & $13.4\pm0.1$ & $12.9\pm0.1$ & $12.7\pm0.1$ & $12.4\pm0.1$ & $12.1\pm0.1$ & $11.8\pm0.1$ & $12.0\pm0.1$ & $13.4\pm0.1$ & $14.0\pm0.1$ & SDSS\\
ASASSN-15pf & ESO 241-G016 & $20.5\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.8\pm0.1$ & $13.6\pm0.1$ & $13.7\pm0.1$ & $14.7\pm0.1$ & $15.4\pm0.1$ & --\\
ASASSN-15ph & 2MASX J22090684+0144384 & $19.4\pm0.1$ & $17.9\pm0.1$ & $16.1\pm0.1$ & $15.2\pm0.1$ & $14.8\pm0.1$ & $14.5\pm0.1$ & $15.9\pm0.1$ & $15.3\pm0.1$ & $14.9\pm0.1$ & $14.7\pm0.1$ & $14.6\pm0.1$ & $14.5\pm0.1$ & $14.3\pm0.1$ & $14.4\pm0.1$ & $15.6\pm0.1$ & $16.2\pm0.1$ & SDSS\\
ASASSN-15pl & ESO 545-G025 & $17.6\pm0.1$ & -- & -- & -- & -- & -- & $15.9\pm0.1$ & $15.4\pm0.1$ & $15.3\pm0.1$ & $15.4\pm0.1$ & $15.3\pm0.1$ & $15.7\pm0.1$ & $15.6\pm0.1$ & $15.6\pm0.2$ & $17.0\pm0.1$ & $17.5\pm0.1$ & PS1\\
ASASSN-15pm & 2MASX J01383676-0440581 & $18.2\pm0.1$ & $16.9\pm0.1$ & $15.5\pm0.1$ & $14.8\pm0.1$ & $14.4\pm0.1$ & $14.0\pm0.1$ & $15.8\pm0.1$ & $15.1\pm0.1$ & $14.8\pm0.1$ & $14.6\pm0.1$ & $14.6\pm0.1$ & $14.3\pm0.1$ & $14.2\pm0.1$ & $14.2\pm0.1$ & $15.3\pm0.1$ & $15.7\pm0.1$ & SDSS\\
ASASSN-15pn & SDSS J040326.23-052930.6 & $19.7\pm0.1$ & $18.9\pm0.1$ & $17.7\pm0.1$ & $17.2\pm0.1$ & $16.9\pm0.1$ & $16.7\pm0.1$ & $17.7\pm0.1$ & $17.2\pm0.1$ & $16.9\pm0.1$ & $16.8\pm0.1$ & $16.7\pm0.1$ & -- & -- & -- & $17.0\pm0.1$ & $17.5\pm0.1$ & SDSS\\
ASASSN-15pp & ESO 159-G023 & $16.8\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.2\pm0.1$ & $12.0\pm0.1$ & $12.1\pm0.1$ & $14.0\pm0.1$ & $14.6\pm0.1$ & --\\
ASASSN-15pr & 2MASX J23063962-1234238 & $18.2\pm0.1$ & -- & -- & -- & -- & -- & $17.6\pm0.1$ & $16.4\pm0.1$ & $16.2\pm0.1$ & $16.1\pm0.1$ & $16.0\pm0.1$ & $16.0\pm0.1$ & $15.7\pm0.1$ & $16.1\pm0.2$ & $16.6\pm0.1$ & $17.2\pm0.1$ & PS1\\
ASASSN-15ps & 2MASS J06144589-6613031 & $22.4\pm0.3$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $17.2\pm0.1$ & $16.9\pm0.1$ & $17.2\pm0.2$ & $17.2\pm0.1$ & $17.8\pm0.1$ & --\\
ASASSN-15py & SDSS J080519.59+225751.1 & $20.7\pm0.1$ & $19.4\pm0.1$ & $18.0\pm0.1$ & $17.4\pm0.1$ & $17.0\pm0.1$ & $16.6\pm0.1$ & $18.0\pm0.1$ & $17.3\pm0.1$ & $17.0\pm0.1$ & $16.9\pm0.1$ & $16.7\pm0.1$ & -- & -- & -- & $17.0\pm0.1$ & $17.5\pm0.1$ & SDSS\\
ASASSN-15pz & ESO 357-G005 & $16.8\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $17.9\pm0.1$ & $18.3\pm0.1$ & --\\
ASASSN-15qc & UGC 00402 & $18.1\pm0.1$ & $15.8\pm0.1$ & $14.2\pm0.1$ & $13.5\pm0.1$ & $13.1\pm0.1$ & $12.8\pm0.1$ & $14.4\pm0.1$ & $13.9\pm0.1$ & $13.6\pm0.1$ & $13.4\pm0.1$ & $13.3\pm0.1$ & $13.2\pm0.1$ & $12.9\pm0.1$ & $13.1\pm0.1$ & $14.1\pm0.1$ & $14.6\pm0.1$ & SDSS\\
ASASSN-15qy & 2MASX J00011837-3321048 & $18.1\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $16.7\pm0.1$ & $16.6\pm0.2$ & $16.6\pm0.2$ & $17.2\pm0.1$ & $17.8\pm0.1$ & --\\
ASASSN-15re & CGCG 448-007 & $18.7\pm0.1$ & $17.0\pm0.1$ & $15.3\pm0.1$ & $14.5\pm0.1$ & $14.0\pm0.1$ & $13.7\pm0.1$ & $15.5\pm0.1$ & $14.7\pm0.1$ & $14.4\pm0.1$ & $14.1\pm0.1$ & $13.9\pm0.1$ & $13.6\pm0.1$ & $13.4\pm0.1$ & $13.5\pm0.1$ & $14.5\pm0.1$ & $15.0\pm0.1$ & SDSS\\
ASASSN-15rm & 2MFGC 05056 & -- & -- & -- & -- & -- & -- & $16.5\pm0.1$ & $15.6\pm0.1$ & $15.1\pm0.1$ & $14.8\pm0.1$ & $14.4\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $14.0\pm0.1$ & $15.1\pm0.1$ & $15.6\pm0.1$ & PS1\\
ASASSN-15rq & GALEXASC J000802.78-363348.1 & $19.7\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $18.2\pm0.1$ & $18.8\pm0.1$ & --\\
ASASSN-15rv & 2MASX J04225455-5230097 & $18.9\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $15.6\pm0.1$ & $15.4\pm0.1$ & $15.4\pm0.1$ & $16.8\pm0.1$ & $17.3\pm0.1$ & --\\
ASASSN-15rw & GALEXASC J021558.44+121415.2 & $20.6\pm0.1$ & $19.3\pm0.1$ & $18.4\pm0.1$ & $17.9\pm0.1$ & $17.8\pm0.1$ & $17.6\pm0.1$ & $18.3\pm0.1$ & $17.8\pm0.1$ & $17.8\pm0.1$ & $17.7\pm0.1$ & $17.6\pm0.1$ & -- & -- & -- & $17.9\pm0.1$ & $18.4\pm0.1$ & SDSS\\
ASASSN-15sb & 2MFGC 04848 & $21.2\pm0.5$ & -- & -- & -- & -- & -- & $15.3\pm0.1$ & $14.4\pm0.1$ & $13.9\pm0.1$ & $13.5\pm0.1$ & $13.2\pm0.1$ & $12.8\pm0.1$ & $12.6\pm0.1$ & $12.7\pm0.1$ & $13.8\pm0.1$ & $14.4\pm0.1$ & PS1\\
ASASSN-15sf & GALEXASC J001127.51-062549.8 & $19.3\pm0.1$ & $18.6\pm0.1$ & $17.3\pm0.1$ & $16.8\pm0.1$ & $16.6\pm0.1$ & $16.5\pm0.1$ & $17.8\pm0.1$ & $17.0\pm0.1$ & $16.7\pm0.1$ & $16.7\pm0.1$ & $17.8\pm0.1$ & -- & -- & -- & $18.5\pm0.1$ & $18.9\pm0.1$ & SDSS\\
ASASSN-15sh & 2MASX J19320827-6226340 & $17.6\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.9\pm0.1$ & $13.7\pm0.1$ & $14.0\pm0.1$ & $15.2\pm0.1$ & $15.8\pm0.1$ & --\\
ASASSN-15so & NGC 3583 & -- & $14.2\pm0.1$ & $12.5\pm0.1$ & $11.7\pm0.1$ & $11.2\pm0.1$ & $10.8\pm0.1$ & -- & -- & -- & -- & -- & $10.4\pm0.1$ & $10.2\pm0.1$ & $10.4\pm0.1$ & $12.4\pm0.1$ & $12.9\pm0.1$ & SDSS\\
ASASSN-15ss & MCG -02-16-004 & -- & -- & -- & -- & -- & -- & $15.7\pm0.1$ & $14.6\pm0.1$ & $14.1\pm0.1$ & $13.8\pm0.1$ & $13.5\pm0.1$ & $13.1\pm0.1$ & $12.8\pm0.1$ & $13.0\pm0.1$ & $13.9\pm0.1$ & $14.4\pm0.1$ & PS1\\
ASASSN-15sx & ESO 472-G018 & $18.4\pm0.1$ & -- & -- & -- & -- & -- & $14.7\pm0.1$ & $14.0\pm0.1$ & $13.6\pm0.1$ & $13.9\pm0.1$ & $13.3\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $13.0\pm0.1$ & $14.3\pm0.1$ & $15.0\pm0.1$ & PS1\\
ASASSN-15tb & LCRS B123822.1-062502 & $17.4\pm0.1$ & $16.2\pm0.1$ & $15.0\pm0.1$ & $14.3\pm0.1$ & $14.0\pm0.1$ & $13.7\pm0.1$ & $15.3\pm0.1$ & $14.7\pm0.1$ & $14.4\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $14.0\pm0.1$ & $13.9\pm0.1$ & $14.0\pm0.1$ & $15.1\pm0.1$ & $15.6\pm0.1$ & SDSS\\
ASASSN-15tf & 2MASX J21291986-2305268 & $17.8\pm0.1$ & -- & -- & -- & -- & -- & $15.8\pm0.1$ & $15.3\pm0.1$ & $15.0\pm0.1$ & $14.9\pm0.1$ & $15.0\pm0.1$ & $15.0\pm0.1$ & $14.7\pm0.1$ & $14.8\pm0.1$ & $16.0\pm0.1$ & $16.6\pm0.1$ & PS1\\
ASASSN-15tg & GALEXASC J002041.66+251341.1 & $18.6\pm0.1$ & -- & -- & -- & -- & -- & $16.8\pm0.1$ & $16.5\pm0.1$ & $16.2\pm0.1$ & $16.0\pm0.1$ & $16.0\pm0.1$ & $15.2\pm0.1$ & $15.0\pm0.1$ & $15.4\pm0.1$ & $16.0\pm0.1$ & $16.6\pm0.1$ & PS1\\
ASASSN-15ti & 2MASX J03051061+3754003 & $20.1\pm0.2$ & $18.2\pm0.1$ & $17.1\pm0.1$ & $16.6\pm0.1$ & $16.4\pm0.1$ & $16.2\pm0.1$ & $17.4\pm0.1$ & $16.9\pm0.1$ & $16.7\pm0.1$ & $16.5\pm0.1$ & $16.5\pm0.1$ & $16.4\pm0.1$ & $15.9\pm0.2$ & $16.2\pm0.2$ & $17.1\pm0.1$ & $17.7\pm0.1$ & SDSS\\
ASASSN-15tj & SDSS J075527.63+520911.1 & -- & $18.1\pm0.1$ & $17.2\pm0.1$ & $16.7\pm0.1$ & $16.6\pm0.1$ & $16.4\pm0.1$ & $17.1\pm0.1$ & $16.6\pm0.1$ & $16.4\pm0.1$ & $16.3\pm0.1$ & $16.1\pm0.1$ & -- & -- & -- & $18.5\pm0.1$ & $19.0\pm0.1$ & SDSS\\
ASASSN-15tn & CGCG 496-051 & $17.8\pm0.1$ & $17.0\pm0.1$ & $15.8\pm0.1$ & $15.3\pm0.1$ & $15.0\pm0.1$ & $14.8\pm0.1$ & $17.2\pm0.1$ & $15.4\pm0.1$ & $15.1\pm0.1$ & $14.9\pm0.1$ & $14.8\pm0.1$ & $14.7\pm0.1$ & $14.6\pm0.1$ & $14.6\pm0.1$ & $15.7\pm0.1$ & $16.3\pm0.1$ & SDSS\\
ASASSN-15ts & 2MASX J03344211-2050502 & -- & -- & -- & -- & -- & -- & $15.7\pm0.1$ & $14.9\pm0.1$ & $14.5\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $13.6\pm0.1$ & $13.8\pm0.1$ & $14.9\pm0.1$ & $15.6\pm0.1$ & PS1\\
ASASSN-15tt & 2MASXi J0638012-373927 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $16.5\pm0.1$ & $16.3\pm0.1$ & $16.4\pm0.1$ & $16.5\pm0.1$ & $17.0\pm0.1$ & --\\
ASASSN-15tz & UGC 02164 & -- & $17.1\pm0.1$ & $15.4\pm0.1$ & $14.4\pm0.1$ & $13.9\pm0.1$ & $13.5\pm0.1$ & $15.7\pm0.1$ & $14.5\pm0.1$ & $14.1\pm0.1$ & $13.8\pm0.1$ & $13.6\pm0.1$ & $13.3\pm0.1$ & $12.9\pm0.1$ & $13.1\pm0.1$ & $14.4\pm0.1$ & $14.9\pm0.1$ & SDSS\\
ASASSN-15ub & CGCG 314-006 & $17.9\pm0.1$ & $16.5\pm0.1$ & $15.6\pm0.1$ & $14.3\pm0.1$ & $13.8\pm0.1$ & $14.2\pm0.1$ & $15.1\pm0.1$ & $14.4\pm0.1$ & $14.1\pm0.1$ & $13.8\pm0.1$ & $13.6\pm0.1$ & $13.8\pm0.1$ & $13.1\pm0.1$ & $12.8\pm0.1$ & $14.5\pm0.1$ & $15.0\pm0.1$ & SDSS\\
ASASSN-15uh & KUG 0925+693 & $18.8\pm0.1$ & -- & -- & -- & -- & -- & $16.5\pm0.1$ & $16.0\pm0.1$ & $15.8\pm0.1$ & $15.7\pm0.1$ & $15.6\pm0.1$ & $15.9\pm0.1$ & $15.7\pm0.1$ & $16.0\pm0.1$ & $16.5\pm0.1$ & $17.0\pm0.1$ & PS1\\
ASASSN-15uk & SDSS J144816.71+171235.6 & -- & $21.3\pm0.2$ & $20.7\pm0.1$ & $20.4\pm0.1$ & $20.4\pm0.1$ & $20.3\pm0.3$ & $20.7\pm0.1$ & $20.6\pm0.1$ & $20.5\pm0.1$ & $20.5\pm0.1$ & -- & -- & -- & -- & -- & -- & SDSS\\
ASASSN-15ul & KUG 1457+066 & $17.3\pm0.1$ & $15.8\pm0.1$ & $14.6\pm0.1$ & $14.0\pm0.1$ & $13.7\pm0.1$ & $13.4\pm0.1$ & $15.4\pm0.1$ & $14.9\pm0.1$ & $14.3\pm0.1$ & $14.3\pm0.1$ & $14.2\pm0.1$ & $14.4\pm0.1$ & $14.1\pm0.1$ & $14.3\pm0.1$ & $15.5\pm0.1$ & $16.1\pm0.1$ & SDSS\\
ASASSN-15up & GALEXASC J042539.92-494621.0 & $19.2\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $16.8\pm0.1$ & $17.2\pm0.1$ & --\\
ASASSN-15uq & ALLWISE J070957.84-650756.9 & $22.4\pm0.3$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $18.7\pm0.1$ & $19.1\pm0.1$ & --\\
ASASSN-15us & NGC 7213 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $ 8.9\pm0.1$ & $ 8.8\pm0.1$ & $ 9.0\pm0.1$ & $10.9\pm0.1$ & $11.2\pm0.1$ & --\\
ASASSN-15uu & VV 790a & $16.5\pm0.1$ & $15.6\pm0.1$ & $14.6\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $14.0\pm0.1$ & $14.8\pm0.1$ & $14.8\pm0.1$ & $14.6\pm0.1$ & $14.3\pm0.1$ & $14.4\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $14.3\pm0.1$ & $15.1\pm0.1$ & $15.5\pm0.1$ & SDSS\\
ASASSN-15uv & 2MASX J08270817+2748382 & -- & $17.5\pm0.1$ & $16.1\pm0.1$ & $15.5\pm0.1$ & $15.1\pm0.1$ & $14.9\pm0.1$ & $16.6\pm0.1$ & $15.4\pm0.1$ & $15.1\pm0.1$ & $15.0\pm0.1$ & $14.8\pm0.1$ & $14.7\pm0.1$ & $14.6\pm0.1$ & $14.8\pm0.1$ & $15.6\pm0.1$ & $16.2\pm0.1$ & SDSS\\
ASASSN-15uw & 2MASX J02353437-0603496 & $20.3\pm0.1$ & $17.4\pm0.1$ & $15.5\pm0.1$ & $14.7\pm0.1$ & $14.2\pm0.1$ & $13.9\pm0.1$ & $15.5\pm0.1$ & $14.8\pm0.1$ & $14.4\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $13.5\pm0.1$ & $13.8\pm0.1$ & $14.7\pm0.1$ & $15.5\pm0.1$ & SDSS\\
ASASSN-16aa & UGC 04251 & -- & $15.6\pm0.1$ & $14.0\pm0.1$ & $13.2\pm0.1$ & $12.9\pm0.1$ & $12.6\pm0.1$ & $14.4\pm0.1$ & $13.8\pm0.1$ & $13.3\pm0.1$ & $13.1\pm0.1$ & $12.9\pm0.1$ & $12.5\pm0.1$ & $12.2\pm0.1$ & $12.4\pm0.1$ & $13.5\pm0.1$ & $14.1\pm0.1$ & SDSS\\
ASASSN-16ad & KUG 0136+335 & $17.8\pm0.1$ & $16.9\pm0.1$ & $15.8\pm0.1$ & $15.4\pm0.1$ & $15.1\pm0.1$ & $15.0\pm0.1$ & $15.8\pm0.1$ & $15.4\pm0.1$ & $15.2\pm0.1$ & $15.1\pm0.1$ & $15.0\pm0.1$ & $16.1\pm0.1$ & $15.9\pm0.1$ & $16.4\pm0.2$ & $16.9\pm0.1$ & $17.4\pm0.1$ & SDSS\\
ASASSN-16ah & Uncatalogued & $20.3\pm0.2$ & -- & -- & -- & -- & -- & $17.1\pm0.1$ & $16.4\pm0.1$ & $16.2\pm0.1$ & $15.8\pm0.1$ & $15.5\pm0.1$ & -- & -- & -- & $17.3\pm0.1$ & $17.7\pm0.1$ & PS1\\
ASASSN-16aj & NGC 1562 & $20.0\pm0.2$ & -- & -- & -- & -- & -- & $15.2\pm0.1$ & $14.1\pm0.1$ & $13.7\pm0.1$ & $13.5\pm0.1$ & $13.5\pm0.1$ & $13.0\pm0.1$ & $12.7\pm0.1$ & $12.9\pm0.1$ & $14.1\pm0.1$ & $14.8\pm0.1$ & PS1\\
ASASSN-16ar & 2MASX J04283087-1739233 & -- & -- & -- & -- & -- & -- & $15.3\pm0.1$ & $14.6\pm0.1$ & $14.1\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $13.5\pm0.1$ & $13.3\pm0.1$ & $13.5\pm0.1$ & $14.6\pm0.1$ & $15.3\pm0.1$ & PS1\\
ASASSN-16av & NGC 3926 NED02 & $19.1\pm0.1$ & $15.9\pm0.1$ & $14.1\pm0.1$ & $13.2\pm0.1$ & $12.8\pm0.1$ & $12.5\pm0.1$ & $14.5\pm0.1$ & $13.7\pm0.1$ & $13.4\pm0.1$ & $13.0\pm0.1$ & $13.2\pm0.1$ & $12.6\pm0.1$ & $12.3\pm0.1$ & $12.5\pm0.1$ & $13.8\pm0.1$ & $14.6\pm0.1$ & SDSS\\
ASASSN-16aw & ESO 306-G 016 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.7\pm0.1$ & $12.4\pm0.1$ & $12.6\pm0.1$ & $14.0\pm0.1$ & $14.7\pm0.1$ & --\\
ASASSN-16ax & 2MASX J01312331+6019128 & -- & -- & -- & -- & -- & -- & $16.2\pm0.1$ & $15.3\pm0.1$ & $14.8\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $13.4\pm0.1$ & $13.0\pm0.1$ & $13.2\pm0.1$ & $14.1\pm0.1$ & $14.8\pm0.1$ & PS1\\
ASASSN-16ay & UGC 03738 & -- & -- & -- & -- & -- & -- & $15.1\pm0.1$ & $14.5\pm0.1$ & $14.2\pm0.1$ & $13.9\pm0.1$ & $13.6\pm0.1$ & $13.4\pm0.1$ & $13.2\pm0.1$ & $13.4\pm0.1$ & $14.6\pm0.1$ & $15.3\pm0.1$ & PS1\\
ASASSN-16az & 2MASX J11303364-4233359 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $14.5\pm0.1$ & $14.2\pm0.1$ & $14.4\pm0.1$ & $15.2\pm0.1$ & $15.8\pm0.1$ & --\\
ASASSN-16bb & SDSS J140557.36+435257.2 & $18.9\pm0.1$ & $18.3\pm0.1$ & $17.2\pm0.1$ & $16.9\pm0.1$ & $16.7\pm0.1$ & $16.7\pm0.1$ & $17.6\pm0.1$ & $17.3\pm0.1$ & $16.9\pm0.1$ & $17.0\pm0.1$ & $17.0\pm0.1$ & -- & -- & -- & $18.3\pm0.1$ & $18.7\pm0.1$ & SDSS\\
ASASSN-16bc & 2MASX J12052488-2123572 & $18.3\pm0.1$ & -- & -- & -- & -- & -- & $15.2\pm0.1$ & $14.5\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $13.7\pm0.1$ & $13.5\pm0.1$ & $13.6\pm0.1$ & $14.7\pm0.1$ & $14.9\pm0.1$ & PS1\\
ASASSN-16bg & 2MASX J12592491+2744198 & $20.9\pm0.3$ & $17.6\pm0.1$ & $15.9\pm0.1$ & $15.0\pm0.1$ & $14.6\pm0.1$ & $14.3\pm0.1$ & $15.8\pm0.1$ & $15.2\pm0.1$ & $14.8\pm0.1$ & $14.6\pm0.1$ & $14.3\pm0.1$ & $14.2\pm0.1$ & $13.9\pm0.1$ & $14.2\pm0.1$ & $15.0\pm0.1$ & $15.8\pm0.1$ & SDSS\\
ASASSN-16bl & 2MASX J11422674-3654256 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.6\pm0.1$ & $13.3\pm0.1$ & $13.5\pm0.1$ & $14.5\pm0.1$ & $15.2\pm0.1$ & --\\
ASASSN-16bn & 2MASX J03103162+0416184 & $21.8\pm0.4$ & $17.2\pm0.1$ & $15.3\pm0.1$ & $14.4\pm0.1$ & $13.9\pm0.1$ & $13.5\pm0.1$ & $15.3\pm0.1$ & $14.5\pm0.1$ & $14.1\pm0.1$ & $13.9\pm0.1$ & $13.7\pm0.1$ & $13.5\pm0.1$ & $13.2\pm0.1$ & $13.4\pm0.1$ & $14.5\pm0.1$ & $15.2\pm0.1$ & SDSS\\
ASASSN-16bp & CGCG 336-041 & $17.7\pm0.1$ & -- & -- & -- & -- & -- & $14.9\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $13.7\pm0.1$ & $13.5\pm0.1$ & $13.2\pm0.1$ & $13.0\pm0.1$ & $13.1\pm0.1$ & $13.7\pm0.1$ & $13.9\pm0.1$ & PS1\\
ASASSN-16bq & IC 0986 & $19.4\pm0.1$ & $16.2\pm0.1$ & $14.2\pm0.1$ & $13.4\pm0.1$ & $13.0\pm0.1$ & $12.6\pm0.1$ & $14.3\pm0.1$ & $13.6\pm0.1$ & $13.2\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $12.5\pm0.1$ & $12.2\pm0.1$ & $12.5\pm0.1$ & $13.5\pm0.1$ & $14.2\pm0.1$ & SDSS\\
ASASSN-16br & 2MASX J15453055-1309057 & $19.2\pm0.1$ & -- & -- & -- & -- & -- & $16.2\pm0.1$ & $15.6\pm0.1$ & $15.3\pm0.1$ & $15.1\pm0.1$ & $14.8\pm0.1$ & $14.6\pm0.1$ & $14.4\pm0.1$ & $14.4\pm0.1$ & $14.7\pm0.1$ & $15.1\pm0.1$ & PS1\\
ASASSN-16bv & LCRS B014209.4-420839 & $18.8\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $18.1\pm0.1$ & $18.5\pm0.1$ & --\\
ASASSN-16bx & CGCG 280-023 & $17.8\pm0.1$ & -- & -- & -- & -- & -- & $14.9\pm0.1$ & $14.2\pm0.1$ & $13.8\pm0.1$ & $13.5\pm0.1$ & $13.5\pm0.1$ & $12.9\pm0.1$ & $12.8\pm0.1$ & $12.9\pm0.1$ & $14.5\pm0.1$ & $15.2\pm0.1$ & PS1\\
ASASSN-16ch & MSPM 00984 & $19.0\pm0.1$ & $17.5\pm0.1$ & $16.2\pm0.1$ & $15.5\pm0.1$ & $15.2\pm0.1$ & $14.9\pm0.1$ & $16.2\pm0.1$ & $15.6\pm0.1$ & $15.2\pm0.1$ & $15.2\pm0.1$ & $14.8\pm0.1$ & $14.5\pm0.1$ & $14.2\pm0.1$ & $14.4\pm0.1$ & $15.9\pm0.1$ & $16.4\pm0.1$ & SDSS\\
ASASSN-16ci & NGC 1272 & $18.7\pm0.1$ & $17.0\pm0.1$ & $14.9\pm0.1$ & $14.1\pm0.1$ & $13.3\pm0.1$ & $13.1\pm0.1$ & -- & -- & -- & -- & -- & $10.8\pm0.1$ & $10.5\pm0.1$ & $10.7\pm0.1$ & $12.8\pm0.1$ & $13.5\pm0.1$ & SDSS\\
ASASSN-16cm & 2MASX J15192684-0055256 & $18.9\pm0.1$ & $17.6\pm0.1$ & $16.2\pm0.1$ & $15.6\pm0.1$ & $15.2\pm0.1$ & $15.0\pm0.1$ & $16.1\pm0.1$ & $15.6\pm0.1$ & $15.2\pm0.1$ & $15.0\pm0.1$ & $14.8\pm0.1$ & $14.7\pm0.1$ & $14.4\pm0.1$ & $14.7\pm0.1$ & $15.3\pm0.1$ & $15.8\pm0.1$ & SDSS\\
ASASSN-16cn & ESO 579-G018 & $18.0\pm0.1$ & $16.3\pm0.1$ & $14.5\pm0.1$ & $13.6\pm0.1$ & $13.1\pm0.1$ & $12.7\pm0.1$ & $14.7\pm0.1$ & $14.0\pm0.1$ & $13.5\pm0.1$ & $13.3\pm0.1$ & $13.1\pm0.1$ & $12.7\pm0.1$ & $12.4\pm0.1$ & $12.5\pm0.1$ & $13.5\pm0.1$ & $13.9\pm0.1$ & SDSS\\
ASASSN-16cs & KUG 0647+311 & $18.7\pm0.1$ & -- & -- & -- & -- & -- & $16.2\pm0.1$ & $15.6\pm0.1$ & $15.4\pm0.1$ & $15.2\pm0.1$ & $15.1\pm0.1$ & $15.3\pm0.1$ & $15.0\pm0.1$ & $15.4\pm0.1$ & $15.7\pm0.1$ & $16.1\pm0.1$ & PS1\\
ASASSN-16ct & SDSS J151354.30+044525.7 & -- & $19.9\pm0.1$ & $18.4\pm0.1$ & $17.8\pm0.1$ & $17.5\pm0.1$ & $17.3\pm0.1$ & $18.5\pm0.1$ & $18.0\pm0.1$ & $17.7\pm0.1$ & $17.6\pm0.1$ & $17.5\pm0.1$ & -- & -- & -- & $18.2\pm0.1$ & $19.0\pm0.1$ & SDSS\\
ASASSN-16cu & IC 4723 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.0\pm0.1$ & $12.7\pm0.1$ & $13.0\pm0.1$ & $14.4\pm0.1$ & $14.8\pm0.1$ & --\\
ASASSN-16cy & CGCG 295-010 & $17.3\pm0.1$ & $17.0\pm0.1$ & $14.5\pm0.1$ & $13.7\pm0.1$ & $13.3\pm0.1$ & $13.0\pm0.1$ & $14.6\pm0.1$ & $14.0\pm0.1$ & $13.6\pm0.1$ & $13.4\pm0.1$ & $13.2\pm0.1$ & $13.1\pm0.1$ & $12.9\pm0.1$ & $13.0\pm0.1$ & $14.3\pm0.1$ & $14.9\pm0.1$ & SDSS\\
ASASSN-16dn & GALEXASC J104848.62-201544.1 & $18.3\pm0.1$ & -- & -- & -- & -- & -- & $17.7\pm0.1$ & $17.4\pm0.1$ & $17.2\pm0.1$ & $17.1\pm0.1$ & $16.8\pm0.1$ & -- & -- & -- & $18.7\pm0.1$ & $19.0\pm0.1$ & PS1\\
ASASSN-16dp & SDSS J145942.12+040518.1 & $20.0\pm0.1$ & $19.3\pm0.1$ & $18.0\pm0.1$ & $17.5\pm0.1$ & $17.3\pm0.1$ & $17.2\pm0.1$ & $18.2\pm0.1$ & $17.8\pm0.1$ & $17.5\pm0.1$ & $17.6\pm0.1$ & $17.6\pm0.1$ & -- & -- & -- & $18.6\pm0.1$ & $19.3\pm0.2$ & SDSS\\
ASASSN-16dw & 2MASX J13300119-2758297 & -- & -- & -- & -- & -- & -- & $16.0\pm0.1$ & $15.3\pm0.1$ & $14.9\pm0.1$ & $14.7\pm0.1$ & $14.4\pm0.1$ & $14.4\pm0.1$ & $14.2\pm0.1$ & $14.3\pm0.1$ & $15.6\pm0.1$ & $16.3\pm0.1$ & PS1\\
ASASSN-16dx & APMUKS B032028.93-441621.0 & $17.9\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $17.3\pm0.1$ & $17.1\pm0.2$ & $17.2\pm0.2$ & $17.4\pm0.1$ & $17.8\pm0.1$ & --\\
ASASSN-16ec & 2MASX J13031054-2159149 & $18.4\pm0.1$ & -- & -- & -- & -- & -- & $15.8\pm0.1$ & $15.1\pm0.1$ & $14.8\pm0.1$ & $14.6\pm0.1$ & $14.4\pm0.1$ & $14.1\pm0.1$ & $13.9\pm0.1$ & $14.0\pm0.1$ & $15.1\pm0.1$ & $15.8\pm0.1$ & PS1\\
ASASSN-16ej & UGC 11409 & -- & $17.2\pm0.1$ & $15.3\pm0.1$ & $14.3\pm0.1$ & $13.8\pm0.1$ & $13.4\pm0.1$ & $15.6\pm0.1$ & $14.7\pm0.1$ & $14.2\pm0.1$ & $13.8\pm0.1$ & $13.7\pm0.1$ & $13.3\pm0.1$ & $13.0\pm0.1$ & $13.1\pm0.1$ & $14.3\pm0.1$ & $14.9\pm0.1$ & SDSS\\
ASASSN-16em & GALEXASC J133213.24+844042.7 & $20.8\pm0.2$ & -- & -- & -- & -- & -- & $17.9\pm0.1$ & $17.4\pm0.1$ & $17.1\pm0.1$ & $17.0\pm0.1$ & $16.9\pm0.1$ & $17.1\pm0.1$ & $17.0\pm0.2$ & $17.1\pm0.2$ & $17.5\pm0.1$ & $18.0\pm0.1$ & PS1\\
ASASSN-16eo & ALLWISE J054312.80+413115.5 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $18.3\pm0.1$ & $18.9\pm0.1$ & --\\
ASASSN-16eq & UGC 11898 & -- & $16.7\pm0.1$ & $14.9\pm0.1$ & $13.8\pm0.1$ & $13.2\pm0.1$ & $12.8\pm0.1$ & $14.8\pm0.1$ & $13.9\pm0.1$ & $13.4\pm0.1$ & $13.1\pm0.1$ & $12.9\pm0.1$ & $12.3\pm0.1$ & $11.9\pm0.1$ & $12.0\pm0.1$ & $13.2\pm0.1$ & $13.5\pm0.1$ & SDSS\\
ASASSN-16es & SDSS J115054.45+021828.1 & $20.4\pm0.1$ & $19.4\pm0.1$ & $18.4\pm0.1$ & $18.0\pm0.1$ & $17.7\pm0.1$ & $17.7\pm0.1$ & $18.9\pm0.1$ & $18.4\pm0.1$ & $18.2\pm0.1$ & $18.1\pm0.1$ & -- & -- & -- & -- & $19.0\pm0.1$ & $19.5\pm0.2$ & SDSS\\
ASASSN-16et & 2MASX J10200192+5627397 & $18.9\pm0.1$ & $17.8\pm0.1$ & $16.7\pm0.1$ & $16.3\pm0.1$ & $16.1\pm0.1$ & $15.9\pm0.1$ & $16.7\pm0.1$ & $16.3\pm0.1$ & $16.1\pm0.1$ & $16.0\pm0.1$ & $16.0\pm0.1$ & $15.9\pm0.1$ & $16.0\pm0.2$ & $16.1\pm0.2$ & $16.9\pm0.1$ & $17.5\pm0.1$ & SDSS\\
ASASSN-16ex & SDSS J171023.63+262350.3 & $19.6\pm0.1$ & $19.4\pm0.1$ & $18.1\pm0.1$ & $17.8\pm0.1$ & $17.5\pm0.1$ & $17.3\pm0.1$ & $18.3\pm0.1$ & $17.8\pm0.1$ & $17.9\pm0.1$ & $18.4\pm0.1$ & $18.6\pm0.1$ & -- & -- & -- & $19.1\pm0.1$ & $19.8\pm0.2$ & SDSS\\
ASASSN-16fa & UGC 06434 & $18.3\pm0.1$ & $16.8\pm0.1$ & $15.2\pm0.1$ & $14.4\pm0.1$ & $13.9\pm0.1$ & $13.6\pm0.1$ & $15.9\pm0.1$ & $14.5\pm0.1$ & -- & -- & -- & $13.2\pm0.1$ & $13.0\pm0.1$ & $13.1\pm0.1$ & $14.2\pm0.1$ & $14.9\pm0.1$ & SDSS\\
ASASSN-16fc & SDSS J153151.40+372445.8 & $18.9\pm0.1$ & $24.5\pm3.1$ & $20.5\pm0.1$ & $19.4\pm0.1$ & $18.8\pm0.1$ & $18.4\pm0.1$ & $17.4\pm0.1$ & $17.2\pm0.1$ & $16.9\pm0.1$ & $17.0\pm0.1$ & $16.4\pm0.1$ & -- & -- & -- & $18.1\pm0.1$ & $18.5\pm0.1$ & PS1\\
ASASSN-16fd & 2MASX J22212881-2215454 & $19.6\pm0.1$ & -- & -- & -- & -- & -- & $14.9\pm0.1$ & $14.2\pm0.1$ & $13.9\pm0.1$ & $13.7\pm0.1$ & $13.4\pm0.1$ & $13.4\pm0.1$ & $13.1\pm0.1$ & $13.3\pm0.1$ & $14.6\pm0.1$ & $15.3\pm0.1$ & PS1\\
ASASSN-16fe & APMUKS B225823.09-373218.0 & $18.7\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $17.3\pm0.1$ & $17.7\pm0.1$ & --\\
ASASSN-16fg & 2MASX J00051603-1629348 & $17.4\pm0.1$ & -- & -- & -- & -- & -- & $15.6\pm0.1$ & $15.2\pm0.1$ & $15.0\pm0.1$ & $14.9\pm0.1$ & $14.8\pm0.1$ & $14.6\pm0.1$ & $14.5\pm0.1$ & $14.7\pm0.1$ & $15.5\pm0.1$ & $16.0\pm0.1$ & PS1\\
ASASSN-16fh & 2MASXi J0002057-265846 & $18.7\pm0.1$ & -- & -- & -- & -- & -- & $16.8\pm0.1$ & $16.5\pm0.1$ & $16.3\pm0.1$ & $16.2\pm0.1$ & $16.1\pm0.1$ & $17.1\pm0.2$ & $16.6\pm0.1$ & $16.9\pm0.2$ & $16.8\pm0.1$ & $17.3\pm0.1$ & PS1\\
ASASSN-16fj & IC 1289 & $17.2\pm0.1$ & -- & -- & -- & -- & -- & $15.1\pm0.1$ & $14.6\pm0.1$ & $14.3\pm0.1$ & -- & -- & $13.8\pm0.1$ & $13.5\pm0.1$ & $13.7\pm0.1$ & $14.6\pm0.1$ & $15.2\pm0.1$ & PS1\\
ASASSN-16fl & 2MASX J10065350-1543022 & $20.5\pm0.1$ & -- & -- & -- & -- & -- & $15.0\pm0.1$ & $14.3\pm0.1$ & $13.9\pm0.1$ & $13.7\pm0.1$ & $13.4\pm0.1$ & $13.3\pm0.1$ & $13.1\pm0.1$ & $13.2\pm0.1$ & $14.2\pm0.1$ & $14.9\pm0.1$ & PS1\\
ASASSN-16fn & Uncatalogued & -- & -- & -- & -- & -- & -- & $17.4\pm0.1$ & $17.2\pm0.1$ & $17.0\pm0.1$ & $17.0\pm0.1$ & $17.0\pm0.1$ & -- & -- & -- & $18.0\pm0.1$ & $18.7\pm0.1$ & PS1\\
ASASSN-16fo & 2MASX J13323577-0516218 & $21.3\pm0.2$ & -- & -- & -- & -- & -- & $16.3\pm0.1$ & $15.6\pm0.1$ & $15.1\pm0.1$ & $14.9\pm0.1$ & $14.8\pm0.1$ & $14.6\pm0.1$ & $14.3\pm0.1$ & $14.6\pm0.1$ & $15.4\pm0.1$ & $16.1\pm0.1$ & PS1\\
ASASSN-16fs & UGC 09523 & $19.1\pm0.1$ & $16.0\pm0.1$ & $14.0\pm0.1$ & $13.2\pm0.1$ & $12.8\pm0.1$ & $12.5\pm0.1$ & $14.2\pm0.1$ & $13.5\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $12.6\pm0.1$ & $12.2\pm0.1$ & $12.0\pm0.1$ & $12.2\pm0.1$ & $13.4\pm0.1$ & $14.1\pm0.1$ & SDSS\\
ASASSN-16fv & IC 4705 & $17.9\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $11.9\pm0.1$ & $11.5\pm0.1$ & $11.8\pm0.1$ & $13.5\pm0.1$ & $14.1\pm0.1$ & --\\
ASASSN-16fx & GALEXASC J020044.56-461644.0 & $19.0\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $18.7\pm0.1$ & $19.1\pm0.1$ & --\\
ASASSN-16gf & CGCG 104-069 & $20.5\pm0.3$ & $16.9\pm0.1$ & $15.0\pm0.1$ & $14.2\pm0.1$ & $13.8\pm0.1$ & $13.5\pm0.1$ & $15.1\pm0.1$ & $14.5\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $13.6\pm0.1$ & $13.4\pm0.1$ & $13.2\pm0.1$ & $13.4\pm0.1$ & $14.3\pm0.1$ & $15.0\pm0.1$ & SDSS\\
ASASSN-16gm & GALEXASC J200348.67-601528.7 & $18.6\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $17.2\pm0.1$ & $17.8\pm0.1$ & --\\
ASASSN-16gp & WKK 2066 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $17.2\pm0.1$ & $17.8\pm0.1$ & --\\
ASASSN-16gq & ESO 446-G023 & $18.3\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.9\pm0.1$ & $12.6\pm0.1$ & $12.7\pm0.1$ & $14.1\pm0.1$ & $14.7\pm0.1$ & --\\
ASASSN-16gv & CGCG 503-021 & $17.4\pm0.1$ & $16.8\pm0.1$ & $15.3\pm0.1$ & $14.7\pm0.1$ & $14.4\pm0.1$ & $14.2\pm0.1$ & $15.2\pm0.1$ & $14.8\pm0.1$ & $14.5\pm0.1$ & $14.4\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $14.0\pm0.1$ & $14.2\pm0.1$ & $15.4\pm0.1$ & $16.0\pm0.1$ & SDSS\\
ASASSN-16gz & APMUKS B043218.28-211910.3 & -- & -- & -- & -- & -- & -- & $17.4\pm0.1$ & $17.0\pm0.1$ & $16.8\pm0.1$ & $16.8\pm0.1$ & $16.5\pm0.1$ & -- & -- & -- & $17.8\pm0.1$ & $18.5\pm0.1$ & PS1\\
ASASSN-16ha & FAIRALL 0673 & $18.8\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.3\pm0.1$ & $13.1\pm0.1$ & $13.3\pm0.1$ & $14.6\pm0.1$ & $15.3\pm0.1$ & --\\
ASASSN-16hc & 2MASX J13590394+3308172 & $21.3\pm0.3$ & $17.4\pm0.1$ & $15.6\pm0.1$ & $14.7\pm0.1$ & $14.2\pm0.1$ & $13.9\pm0.1$ & $16.1\pm0.1$ & $15.1\pm0.1$ & $14.7\pm0.1$ & $14.6\pm0.1$ & $14.3\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $13.9\pm0.1$ & $14.8\pm0.1$ & $15.5\pm0.1$ & SDSS\\
ASASSN-16hd & GALEXASC J015051.89+223348.8 & $19.8\pm0.1$ & $19.0\pm0.1$ & $18.0\pm0.1$ & $17.6\pm0.1$ & $17.4\pm0.1$ & $17.4\pm0.1$ & -- & $17.9\pm0.1$ & -- & -- & $18.4\pm0.1$ & -- & -- & -- & $18.5\pm0.1$ & $19.2\pm0.1$ & SDSS\\
ASASSN-16hh & MCG +03-06-031 & $18.4\pm0.1$ & $17.3\pm0.1$ & $16.1\pm0.1$ & $15.5\pm0.1$ & $15.1\pm0.1$ & $14.9\pm0.1$ & $16.5\pm0.1$ & $15.7\pm0.1$ & $15.5\pm0.1$ & $15.3\pm0.1$ & $15.1\pm0.1$ & $15.5\pm0.1$ & $15.3\pm0.1$ & $15.3\pm0.1$ & $17.1\pm0.1$ & $17.5\pm0.1$ & SDSS\\
ASASSN-16hp & ESO 509-IG064 & $16.6\pm0.1$ & -- & -- & -- & -- & -- & $14.5\pm0.1$ & $14.1\pm0.1$ & $13.9\pm0.1$ & $13.7\pm0.1$ & $13.5\pm0.1$ & $14.8\pm0.1$ & $14.7\pm0.1$ & $15.0\pm0.1$ & $15.4\pm0.1$ & $15.8\pm0.1$ & PS1\\
ASASSN-16hr & 2MASX J22253147+3859010 & $19.0\pm0.1$ & $17.6\pm0.1$ & $16.4\pm0.1$ & $15.9\pm0.1$ & $15.6\pm0.1$ & $15.3\pm0.1$ & $16.4\pm0.1$ & $15.9\pm0.1$ & $15.6\pm0.1$ & $15.4\pm0.1$ & $15.3\pm0.1$ & $16.1\pm0.1$ & $15.9\pm0.1$ & $16.0\pm0.1$ & $16.1\pm0.1$ & $16.6\pm0.1$ & SDSS\\
ASASSN-16hw & GALEXASC J215327.92-342420.8 & $18.8\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $17.0\pm0.1$ & $17.0\pm0.1$ & $16.8\pm0.1$ & $17.0\pm0.1$ & $17.5\pm0.1$ & --\\
ASASSN-16hz & 2MASX J23154564-0120135 & $18.9\pm0.1$ & $17.1\pm0.1$ & $15.7\pm0.1$ & $14.9\pm0.1$ & $14.6\pm0.1$ & $14.2\pm0.1$ & $15.6\pm0.1$ & $15.0\pm0.1$ & $14.6\pm0.1$ & $14.4\pm0.1$ & $14.2\pm0.1$ & $14.1\pm0.1$ & $13.8\pm0.1$ & $14.0\pm0.1$ & $14.9\pm0.1$ & $15.4\pm0.1$ & SDSS\\
ASASSN-16ic & GALEXASC J011415.49-162456.4 & $20.3\pm0.1$ & -- & -- & -- & -- & -- & $19.3\pm0.1$ & $18.8\pm0.1$ & $18.8\pm0.1$ & $18.5\pm0.1$ & $18.3\pm0.1$ & -- & -- & -- & $19.9\pm0.1$ & $20.4\pm0.5$ & PS1\\
ASASSN-16ie & 2MASXi J1604144+164124 & -- & $18.7\pm0.1$ & $17.2\pm0.1$ & $16.4\pm0.1$ & $16.1\pm0.1$ & $15.8\pm0.1$ & $17.7\pm0.1$ & $16.9\pm0.1$ & $16.4\pm0.1$ & $16.3\pm0.1$ & $16.5\pm0.1$ & -- & -- & -- & $17.3\pm0.1$ & $17.8\pm0.1$ & SDSS\\
ASASSN-16if & AM 0557-522 NED03 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.3\pm0.1$ & $12.0\pm0.1$ & $12.2\pm0.1$ & $13.4\pm0.1$ & $14.0\pm0.1$ & --\\
ASASSN-16io & 2MASX J18400114+5413042 & $19.9\pm0.1$ & -- & -- & -- & -- & -- & $17.4\pm0.1$ & $16.8\pm0.1$ & $17.2\pm0.1$ & $16.6\pm0.1$ & $16.4\pm0.1$ & $15.9\pm0.1$ & $15.6\pm0.1$ & $15.7\pm0.1$ & $16.8\pm0.1$ & $17.3\pm0.1$ & PS1\\
ASASSN-16ip & ESO 479-G007 & $20.2\pm0.1$ & -- & -- & -- & -- & -- & $15.1\pm0.1$ & $14.5\pm0.1$ & $14.1\pm0.1$ & $13.9\pm0.1$ & $13.7\pm0.1$ & $13.5\pm0.1$ & $13.3\pm0.1$ & $13.6\pm0.1$ & $14.8\pm0.1$ & $15.5\pm0.1$ & PS1\\
ASASSN-16iq & ESO 471-G041 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.7\pm0.1$ & $13.5\pm0.1$ & $13.7\pm0.1$ & $15.1\pm0.1$ & $15.7\pm0.1$ & --\\
ASASSN-16jc & NGC 6942 & $17.9\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $10.7\pm0.1$ & $10.5\pm0.1$ & $10.7\pm0.1$ & $12.9\pm0.1$ & $13.5\pm0.1$ & --\\
ASASSN-16je & 2MASX J17055033+6950555 & $18.3\pm0.1$ & -- & -- & -- & -- & -- & $16.3\pm0.1$ & $15.7\pm0.1$ & $15.5\pm0.1$ & $15.3\pm0.1$ & $15.2\pm0.1$ & $15.2\pm0.1$ & $14.9\pm0.1$ & $15.1\pm0.1$ & $16.5\pm0.1$ & $17.0\pm0.1$ & PS1\\
ASASSN-16jf & UGCA 430 & $15.6\pm0.1$ & -- & -- & -- & -- & -- & $15.0\pm0.1$ & $14.6\pm0.1$ & $14.5\pm0.1$ & $14.5\pm0.1$ & $14.0\pm0.1$ & $16.3\pm0.1$ & $16.2\pm0.2$ & $15.9\pm0.2$ & $17.3\pm0.1$ & $17.9\pm0.1$ & --\\
ASASSN-16jh & 2dFGRS S501Z101 & $18.3\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $18.0\pm0.1$ & $18.5\pm0.1$ & --\\
ASASSN-16jj & GALEXASC J234711.93+100501.3 & $19.1\pm0.1$ & $18.3\pm0.1$ & $17.1\pm0.1$ & $16.6\pm0.1$ & $16.3\pm0.1$ & $16.2\pm0.1$ & $17.1\pm0.1$ & $16.8\pm0.1$ & $16.4\pm0.1$ & $16.4\pm0.1$ & $16.5\pm0.1$ & -- & -- & -- & $17.6\pm0.1$ & $18.1\pm0.1$ & SDSS\\
ASASSN-16jq & CGMW 2-2125 & -- & -- & -- & -- & -- & -- & $17.8\pm0.1$ & $17.2\pm0.1$ & $16.9\pm0.1$ & $16.8\pm0.1$ & $16.7\pm0.1$ & -- & -- & -- & -- & -- & PS1\\
ASASSN-16jw & IC 1780 & $18.0\pm0.1$ & $16.9\pm0.1$ & $15.5\pm0.1$ & $14.7\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $15.3\pm0.1$ & $14.8\pm0.1$ & $14.4\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $13.6\pm0.1$ & $13.7\pm0.1$ & $14.9\pm0.1$ & $15.5\pm0.1$ & SDSS\\
ASASSN-16ke & AGC 331536 & $21.3\pm0.2$ & $20.1\pm0.1$ & $18.8\pm0.1$ & $18.3\pm0.1$ & $18.1\pm0.1$ & $17.9\pm0.1$ & $18.9\pm0.1$ & $18.4\pm0.1$ & $18.2\pm0.1$ & $18.1\pm0.1$ & $18.3\pm0.1$ & -- & -- & -- & $18.7\pm0.1$ & $20.0\pm0.3$ & SDSS\\
ASASSN-16kk & LSBG F156-039 & $20.5\pm0.2$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.3\pm0.1$ & $13.1\pm0.1$ & $13.2\pm0.1$ & $14.1\pm0.1$ & $14.8\pm0.1$ & --\\
ASASSN-16km & ESO 197-G010 & $18.5\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $11.0\pm0.1$ & $10.6\pm0.1$ & $10.8\pm0.1$ & $12.7\pm0.1$ & $13.4\pm0.1$ & --\\
ASASSN-16kv & 2MASX J05073951-1932539 & $20.4\pm0.2$ & -- & -- & -- & -- & -- & $15.8\pm0.1$ & $15.0\pm0.1$ & $14.7\pm0.1$ & $14.5\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $13.9\pm0.1$ & $14.1\pm0.1$ & $14.9\pm0.1$ & $15.5\pm0.1$ & PS1\\
ASASSN-16kw & 2MASX J05080487-4141151 & $17.9\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $14.9\pm0.1$ & $15.1\pm0.1$ & $15.0\pm0.1$ & $16.2\pm0.1$ & $16.8\pm0.1$ & --\\
ASASSN-16kz & ESO 555-G029 & $17.6\pm0.1$ & -- & -- & -- & -- & -- & $14.9\pm0.1$ & $14.3\pm0.1$ & $13.9\pm0.1$ & $13.7\pm0.1$ & $13.4\pm0.1$ & $13.4\pm0.1$ & $13.1\pm0.1$ & $13.3\pm0.1$ & $15.1\pm0.1$ & $15.8\pm0.1$ & PS1\\
ASASSN-16la & 2MASXi J0229172+180515 & -- & -- & -- & -- & -- & -- & $16.9\pm0.1$ & $16.3\pm0.1$ & $16.1\pm0.1$ & $15.8\pm0.1$ & $15.7\pm0.1$ & -- & -- & -- & $17.0\pm0.1$ & $17.5\pm0.1$ & PS1\\
ASASSN-16lc & GALEXASC J192901.47-515813.5 & $20.9\pm0.2$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $19.3\pm0.1$ & $20.1\pm0.3$ & --\\
ASASSN-16lg & ARK 530 & -- & -- & -- & -- & -- & -- & $14.1\pm0.1$ & $13.4\pm0.1$ & $13.1\pm0.1$ & $12.8\pm0.1$ & $12.6\pm0.1$ & $12.3\pm0.1$ & $12.1\pm0.1$ & $12.2\pm0.1$ & $13.4\pm0.1$ & $14.1\pm0.1$ & PS1\\
ASASSN-16lm & 2MASX J09033461+4142367 & $18.2\pm0.1$ & $17.3\pm0.1$ & $15.5\pm0.1$ & $14.9\pm0.1$ & $14.6\pm0.1$ & $14.3\pm0.1$ & $16.0\pm0.1$ & $15.6\pm0.1$ & $15.2\pm0.1$ & $15.1\pm0.1$ & $15.0\pm0.1$ & $15.2\pm0.1$ & $15.0\pm0.1$ & $15.3\pm0.1$ & $16.1\pm0.1$ & $16.7\pm0.1$ & SDSS\\
ASASSN-16lx & IC 0607 & $16.7\pm0.1$ & $15.6\pm0.1$ & $14.2\pm0.1$ & $13.4\pm0.1$ & $13.0\pm0.1$ & $12.6\pm0.1$ & $14.1\pm0.1$ & $13.5\pm0.1$ & $13.3\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $13.5\pm0.1$ & $13.3\pm0.1$ & $13.5\pm0.1$ & $15.0\pm0.1$ & $15.7\pm0.1$ & SDSS\\
ASASSN-16lz & ALLWISE J060551.48-504652.2 & $21.1\pm0.3$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $19.6\pm0.1$ & $20.4\pm0.2$ & --\\
ASASSN-16mc & ESO 233-IG014 & $17.0\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.4\pm0.1$ & $13.2\pm0.1$ & $13.3\pm0.1$ & $14.0\pm0.1$ & $14.4\pm0.1$ & --\\
ASASSN-16mj & SDSS J092119.07+170159.5 & $20.7\pm0.2$ & $19.7\pm0.1$ & $18.8\pm0.1$ & $18.5\pm0.1$ & $18.3\pm0.1$ & $18.1\pm0.1$ & $19.1\pm0.1$ & $18.7\pm0.1$ & $18.5\pm0.1$ & $18.4\pm0.1$ & $18.5\pm0.1$ & -- & -- & -- & $18.9\pm0.1$ & $19.3\pm0.2$ & SDSS\\
ASASSN-16mt & 2MASX J01004149-0026406 & $21.3\pm0.2$ & $18.3\pm0.1$ & $16.5\pm0.1$ & $15.8\pm0.1$ & $15.4\pm0.1$ & $15.1\pm0.1$ & $16.4\pm0.1$ & $15.9\pm0.1$ & $15.5\pm0.1$ & $15.3\pm0.1$ & $15.1\pm0.1$ & $14.9\pm0.1$ & $14.8\pm0.1$ & $14.8\pm0.1$ & $15.8\pm0.1$ & $16.4\pm0.1$ & SDSS\\
ASASSN-16mv & ESO 563-G035 & $19.0\pm0.1$ & -- & -- & -- & -- & -- & $14.7\pm0.1$ & $13.7\pm0.1$ & $13.1\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $12.2\pm0.1$ & $11.8\pm0.1$ & $12.0\pm0.1$ & $13.4\pm0.1$ & $13.9\pm0.1$ & PS1\\
ASASSN-16na & 2MASX J04091030+2126244 & -- & -- & -- & -- & -- & -- & $15.6\pm0.1$ & $14.6\pm0.1$ & $13.9\pm0.1$ & $13.6\pm0.1$ & $13.4\pm0.1$ & $12.8\pm0.1$ & $12.5\pm0.1$ & $12.6\pm0.1$ & $13.7\pm0.1$ & $14.3\pm0.1$ & PS1\\
ASASSN-16nm & 2MASX J21255058-3724071 & $18.2\pm0.2$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $14.2\pm0.1$ & $14.1\pm0.1$ & $14.2\pm0.1$ & $15.5\pm0.1$ & $16.0\pm0.1$ & --\\
ASASSN-16nn & APMUKS B214820.71-555825.5 & $19.3\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $18.1\pm0.1$ & $18.5\pm0.1$ & --\\
ASASSN-16no & IC 0493 & $16.9\pm0.1$ & -- & -- & $13.0\pm0.1$ & -- & -- & $14.5\pm0.1$ & $13.8\pm0.1$ & $13.5\pm0.1$ & $13.4\pm0.1$ & $13.2\pm0.1$ & $13.0\pm0.1$ & $12.7\pm0.1$ & $12.9\pm0.1$ & $14.1\pm0.1$ & $14.6\pm0.1$ & PS1\\
ASASSN-16np & SDSS J123643.42+260647.1 & $19.5\pm0.1$ & $18.6\pm0.1$ & $17.6\pm0.1$ & $17.1\pm0.1$ & $16.9\pm0.1$ & $16.6\pm0.1$ & $17.6\pm0.1$ & $17.1\pm0.1$ & $16.9\pm0.1$ & $16.7\pm0.1$ & $16.6\pm0.1$ & $16.8\pm0.1$ & $16.7\pm0.1$ & $17.0\pm0.1$ & $17.0\pm0.1$ & $17.4\pm0.1$ & SDSS\\
ASASSN-16nt & CGCG 068-029 & $20.4\pm0.2$ & $17.2\pm0.1$ & $15.4\pm0.1$ & $14.6\pm0.1$ & $14.2\pm0.1$ & $13.9\pm0.1$ & $15.5\pm0.1$ & $14.8\pm0.1$ & $14.5\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $13.9\pm0.1$ & $13.7\pm0.1$ & $13.9\pm0.1$ & $14.8\pm0.1$ & $15.5\pm0.1$ & SDSS\\
ASASSN-16nv & 2MASX J05482726-2319189 & -- & -- & -- & -- & -- & -- & $16.3\pm0.1$ & $16.2\pm0.1$ & $16.0\pm0.1$ & $15.9\pm0.1$ & $15.7\pm0.1$ & $15.6\pm0.1$ & $15.6\pm0.1$ & $15.6\pm0.1$ & $16.4\pm0.1$ & $16.8\pm0.1$ & PS1\\
ASASSN-16of & ESO 087-IG 041 & $18.5\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $14.8\pm0.1$ & $15.1\pm0.1$ & --\\
ASASSN-16oj & SDSS J053208.29-020407.9 & -- & $19.5\pm0.3$ & $17.3\pm0.1$ & $16.4\pm0.1$ & $15.9\pm0.1$ & $15.6\pm0.1$ & $18.2\pm0.1$ & $17.0\pm0.1$ & $16.0\pm0.1$ & $16.5\pm0.1$ & $15.9\pm0.1$ & -- & -- & -- & -- & -- & SDSS\\
ASASSN-16ok & GALEXASC J005328.92-362154.1 & $20.6\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $20.1\pm0.1$ & -- & --\\
ASASSN-16ol & GALEXASC J011003.70-702046.4 & $18.9\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $18.1\pm0.1$ & $18.5\pm0.1$ & --\\
ASASSN-16om & AM 2329-410 & $20.6\pm0.2$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.7\pm0.1$ & $13.5\pm0.1$ & $13.7\pm0.1$ & $14.7\pm0.1$ & $15.3\pm0.1$ & --\\
ASASSN-16oo & 2MASX J01411858-0012382 & $18.1\pm0.1$ & $17.3\pm0.1$ & $16.3\pm0.1$ & $15.9\pm0.1$ & $15.6\pm0.1$ & $15.4\pm0.1$ & $16.3\pm0.1$ & $15.9\pm0.1$ & $15.6\pm0.1$ & $15.6\pm0.1$ & $15.5\pm0.1$ & $15.5\pm0.1$ & $15.3\pm0.1$ & $15.2\pm0.1$ & $16.6\pm0.1$ & $17.0\pm0.1$ & SDSS\\
ASASSN-16oq & AM 1228-353 NED02 & $17.6\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.8\pm0.1$ & $13.5\pm0.1$ & $13.6\pm0.1$ & $14.1\pm0.1$ & $14.5\pm0.1$ & --\\
ASASSN-16ov & NPM1G +01.0158 & -- & -- & -- & -- & -- & -- & $16.4\pm0.1$ & $15.6\pm0.1$ & $15.2\pm0.1$ & $15.0\pm0.1$ & $14.8\pm0.1$ & -- & -- & -- & $16.0\pm0.1$ & $16.7\pm0.1$ & PS1\\
ASASSN-16oz & GALEXASC J090013.19-133803.5 & $20.7\pm0.2$ & -- & -- & -- & -- & -- & $18.9\pm0.1$ & $18.6\pm0.1$ & $18.6\pm0.1$ & $19.3\pm0.1$ & $18.4\pm0.1$ & -- & -- & -- & $19.5\pm0.1$ & $19.7\pm0.2$ & PS1\\
ASASSN-16pa & ALLWISE J003315.83-842917.8 & $21.3\pm0.2$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $17.8\pm0.1$ & $18.3\pm0.1$ & --\\
ASASSN-16pb & CGCG 058-057 & $17.9\pm0.1$ & $17.2\pm0.1$ & $15.9\pm0.1$ & $15.4\pm0.1$ & $15.1\pm0.1$ & $14.8\pm0.1$ & $16.2\pm0.1$ & $15.6\pm0.1$ & $15.3\pm0.1$ & $15.1\pm0.1$ & $15.1\pm0.1$ & -- & -- & -- & $16.8\pm0.1$ & $17.5\pm0.1$ & SDSS\\
ASASSN-16pd & PGC 241921 & $20.0\pm0.2$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $17.7\pm0.1$ & $18.3\pm0.1$ & --\\
ASASSN-16pj & GALEXASC J232303.16-361420.6 & $19.3\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $17.8\pm0.1$ & $18.4\pm0.1$ & --\\
ASASSN-16pk & SDSS J122739.65+403648.9 & $18.9\pm0.1$ & $18.4\pm0.1$ & $17.4\pm0.1$ & $17.1\pm0.1$ & $16.9\pm0.1$ & $16.8\pm0.1$ & $17.2\pm0.1$ & $16.8\pm0.1$ & $16.7\pm0.1$ & $16.5\pm0.1$ & $16.4\pm0.1$ & -- & -- & -- & $17.6\pm0.1$ & $18.1\pm0.1$ & SDSS\\
ASASSN-16pl & IC 0988 & $18.4\pm0.1$ & $16.0\pm0.1$ & $14.3\pm0.1$ & $13.6\pm0.1$ & $13.2\pm0.1$ & $13.0\pm0.1$ & -- & -- & -- & -- & -- & $12.8\pm0.1$ & $12.5\pm0.1$ & $12.8\pm0.1$ & $13.9\pm0.1$ & $14.5\pm0.1$ & SDSS\\
2014bz & 2MASX J13560316-4334319 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $14.3\pm0.1$ & $14.0\pm0.1$ & $14.6\pm0.1$ & $15.5\pm0.1$ & $16.2\pm0.1$ & --\\
2014ba & NGC 7410 & $15.5\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $ 9.0\pm0.1$ & $ 8.8\pm0.1$ & $ 9.1\pm0.1$ & $12.1\pm0.1$ & $12.7\pm0.1$ & --\\
2014bb & NGC 5214 & $15.7\pm0.1$ & $15.2\pm0.1$ & $13.9\pm0.1$ & $13.3\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $14.2\pm0.1$ & $13.6\pm0.1$ & $13.3\pm0.1$ & $13.1\pm0.1$ & $13.1\pm0.1$ & $12.7\pm0.1$ & $12.5\pm0.1$ & $12.6\pm0.1$ & $14.2\pm0.1$ & $14.7\pm0.1$ & SDSS\\
PSN J15024996+4847062 & 2MASX J15024995+4847010 & -- & $18.1\pm0.1$ & $16.6\pm0.1$ & $16.1\pm0.1$ & $15.7\pm0.1$ & $15.6\pm0.1$ & $16.6\pm0.1$ & $16.1\pm0.1$ & $15.8\pm0.1$ & $15.7\pm0.1$ & $15.6\pm0.1$ & $15.2\pm0.1$ & $14.9\pm0.2$ & $15.0\pm0.2$ & $16.7\pm0.1$ & $17.2\pm0.1$ & SDSS\\
2014bg & UGC 09396 & $17.1\pm0.1$ & $15.7\pm0.1$ & $14.1\pm0.1$ & $13.4\pm0.1$ & $12.9\pm0.1$ & $12.6\pm0.1$ & $14.2\pm0.1$ & $13.6\pm0.1$ & $13.2\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $12.5\pm0.1$ & $12.2\pm0.1$ & $12.3\pm0.1$ & $13.8\pm0.1$ & $14.3\pm0.1$ & SDSS\\
iPTF14bdn & UGC 08503 & $17.2\pm0.1$ & $17.8\pm0.1$ & $16.3\pm0.1$ & $15.9\pm0.1$ & $15.5\pm0.1$ & $15.3\pm0.1$ & $16.0\pm0.1$ & $15.6\pm0.1$ & $15.6\pm0.1$ & $15.6\pm0.1$ & -- & -- & -- & -- & $17.7\pm0.1$ & $18.3\pm0.1$ & SDSS\\
2014ch & SDSS J155830.96+125157.5 & -- & $20.9\pm0.2$ & $19.6\pm0.1$ & $19.4\pm0.1$ & $19.2\pm0.1$ & $19.3\pm0.2$ & $19.8\pm0.1$ & $19.2\pm0.1$ & $19.1\pm0.1$ & $19.0\pm0.1$ & $21.3\pm0.1$ & -- & -- & -- & -- & -- & SDSS\\
2014bs & NGC 5270 & $16.0\pm0.1$ & $15.7\pm0.1$ & $14.2\pm0.1$ & $13.5\pm0.1$ & $13.2\pm0.1$ & $12.9\pm0.1$ & $15.0\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $13.8\pm0.1$ & $13.2\pm0.1$ & $12.8\pm0.1$ & $12.7\pm0.1$ & $12.8\pm0.1$ & $14.3\pm0.1$ & $15.0\pm0.1$ & SDSS\\
LSQ14cnm & 2MASX J16052452+0113000 & $18.7\pm0.1$ & $17.7\pm0.1$ & $16.6\pm0.1$ & $16.2\pm0.1$ & $16.0\pm0.1$ & $15.8\pm0.1$ & $16.6\pm0.1$ & $16.2\pm0.1$ & $16.0\pm0.1$ & $15.9\pm0.1$ & $15.8\pm0.1$ & $15.5\pm0.1$ & $15.4\pm0.1$ & $15.7\pm0.2$ & $16.3\pm0.1$ & $16.8\pm0.1$ & SDSS\\
2014bv & NGC 4386 & -- & -- & -- & -- & -- & -- & $12.5\pm0.1$ & $11.8\pm0.1$ & $11.4\pm0.1$ & $11.1\pm0.1$ & $10.8\pm0.1$ & $10.3\pm0.1$ & $10.1\pm0.1$ & $10.3\pm0.1$ & $12.2\pm0.1$ & $12.9\pm0.1$ & PS1\\
CSS140628:164427+285658 & SDSS J164427.41+285656.8 & $21.0\pm0.1$ & $20.4\pm0.1$ & $19.5\pm0.1$ & $19.4\pm0.1$ & $19.2\pm0.1$ & $19.2\pm0.1$ & $19.6\pm0.1$ & $19.4\pm0.1$ & $19.2\pm0.1$ & $19.3\pm0.1$ & $19.4\pm0.1$ & -- & -- & -- & $20.1\pm0.1$ & $20.5\pm0.4$ & SDSS\\
2014ck & UGC 12182 & $18.8\pm0.1$ & -- & -- & -- & -- & -- & $15.4\pm0.1$ & $14.7\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $13.8\pm0.1$ & $13.2\pm0.1$ & $12.8\pm0.1$ & $13.3\pm0.1$ & $15.3\pm0.1$ & $16.0\pm0.1$ & PS1\\
2014by & UGC 09267 & $17.1\pm0.1$ & $15.9\pm0.1$ & $14.4\pm0.1$ & $13.7\pm0.1$ & $13.3\pm0.1$ & $13.0\pm0.1$ & $15.0\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $13.6\pm0.1$ & $13.6\pm0.1$ & $13.2\pm0.1$ & $13.0\pm0.1$ & $13.4\pm0.1$ & $14.6\pm0.1$ & $15.1\pm0.1$ & SDSS\\
2014bx & NGC 6808 & $16.1\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $11.0\pm0.1$ & $10.8\pm0.1$ & $10.9\pm0.1$ & $12.6\pm0.1$ & $13.0\pm0.1$ & --\\
PSN J01340299-0104458 & UGC 01120 & $17.2\pm0.1$ & $16.1\pm0.1$ & $14.5\pm0.1$ & $13.7\pm0.1$ & $13.2\pm0.1$ & $12.9\pm0.1$ & $14.7\pm0.1$ & $14.0\pm0.1$ & $13.6\pm0.1$ & $13.3\pm0.1$ & $13.1\pm0.1$ & $12.7\pm0.1$ & $12.4\pm0.1$ & $12.6\pm0.1$ & $13.8\pm0.1$ & $14.4\pm0.1$ & SDSS\\
2014da & NGC 0128 & $17.6\pm0.1$ & $14.2\pm0.1$ & $12.3\pm0.1$ & $11.4\pm0.1$ & $11.0\pm0.1$ & $10.6\pm0.1$ & -- & -- & -- & -- & -- & $10.4\pm0.1$ & $10.2\pm0.1$ & $10.4\pm0.1$ & $12.2\pm0.1$ & $12.9\pm0.1$ & SDSS\\
PSN J02451711+4213503 & GALEXASC J024517.55+421344.1 & $19.0\pm0.1$ & -- & -- & -- & -- & -- & $17.2\pm0.1$ & $16.7\pm0.1$ & $16.5\pm0.1$ & $16.3\pm0.1$ & $16.1\pm0.1$ & -- & -- & -- & $17.8\pm0.1$ & $18.4\pm0.1$ & PS1\\
2014cc & NGC 2255 & $16.0\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.6\pm0.1$ & $12.5\pm0.1$ & $12.6\pm0.1$ & $14.0\pm0.1$ & $14.6\pm0.1$ & --\\
2014cd & NGC 1578 & $16.3\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $11.7\pm0.1$ & $11.5\pm0.1$ & $11.7\pm0.1$ & $13.3\pm0.1$ & $13.9\pm0.1$ & --\\
2014cj & ESO 087-G031 & $18.7\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.7\pm0.1$ & $12.5\pm0.1$ & $12.5\pm0.1$ & $13.7\pm0.1$ & $14.3\pm0.1$ & --\\
MASTER OT J162412.26+091303.0 & CGCG 080-023 & $17.8\pm0.1$ & $16.7\pm0.1$ & $15.5\pm0.1$ & $14.8\pm0.1$ & $14.5\pm0.1$ & $14.2\pm0.1$ & $15.6\pm0.1$ & $15.0\pm0.1$ & $14.7\pm0.1$ & $14.8\pm0.1$ & $14.8\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $14.2\pm0.2$ & $16.1\pm0.1$ & $16.7\pm0.1$ & SDSS\\
2014cb & VV 322b & $17.9\pm0.1$ & -- & -- & -- & -- & -- & $15.9\pm0.1$ & $14.7\pm0.1$ & $14.4\pm0.1$ & $14.1\pm0.1$ & $13.8\pm0.1$ & $13.3\pm0.1$ & $12.9\pm0.1$ & $13.0\pm0.1$ & $14.2\pm0.1$ & $14.7\pm0.1$ & PS1\\
2014dd & UGC 02504 & -- & -- & -- & -- & -- & -- & $14.7\pm0.1$ & $13.8\pm0.1$ & $13.3\pm0.1$ & $12.9\pm0.1$ & $12.6\pm0.1$ & $12.1\pm0.1$ & $11.8\pm0.1$ & $11.9\pm0.1$ & $13.2\pm0.1$ & $14.5\pm0.1$ & PS1\\
2014dg & UGC 02855 & $16.2\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & $11.3\pm0.1$ & -- & -- & $ 9.3\pm0.1$ & $ 9.0\pm0.1$ & $ 9.1\pm0.1$ & $12.3\pm0.1$ & $12.4\pm0.1$ & --\\
2014dk & DDG2014 J002812.09+070940.1 & -- & $22.0\pm0.6$ & $20.7\pm0.1$ & $20.3\pm0.1$ & $20.2\pm0.1$ & $19.9\pm0.4$ & $21.4\pm0.1$ & $20.1\pm0.1$ & $20.3\pm0.1$ & $19.6\pm0.1$ & $19.0\pm0.1$ & -- & -- & -- & -- & -- & SDSS\\
2014dm & NGC 1516A & -- & -- & -- & -- & -- & -- & $15.1\pm0.1$ & $14.0\pm0.1$ & $13.7\pm0.1$ & $13.5\pm0.1$ & $13.2\pm0.1$ & $12.5\pm0.1$ & $12.2\pm0.1$ & $12.4\pm0.1$ & $14.0\pm0.1$ & $14.4\pm0.1$ & PS1\\
PSN J09084248+4448132 & UGC 04798 & $16.7\pm0.1$ & $16.6\pm0.1$ & $15.0\pm0.1$ & $14.3\pm0.1$ & $14.0\pm0.1$ & $13.7\pm0.1$ & $15.5\pm0.1$ & $14.9\pm0.1$ & $14.4\pm0.1$ & $14.0\pm0.1$ & $13.9\pm0.1$ & $13.5\pm0.1$ & $13.4\pm0.1$ & $13.6\pm0.1$ & $15.5\pm0.1$ & $16.1\pm0.1$ & SDSS\\
2014dt & M61 & $12.4\pm0.1$ & $13.9\pm0.1$ & $12.5\pm0.1$ & $11.9\pm0.1$ & $11.5\pm0.1$ & $11.1\pm0.1$ & -- & $ 7.6\pm0.1$ & $ 9.7\pm0.1$ & $10.2\pm0.1$ & $10.2\pm0.1$ & $ 7.8\pm0.1$ & $ 7.1\pm0.1$ & $ 6.9\pm0.1$ & $11.7\pm0.1$ & $12.3\pm0.1$ & --\\
2014du & UGC 01899 & $18.7\pm0.1$ & -- & -- & -- & -- & -- & $14.4\pm0.1$ & $13.6\pm0.1$ & $13.2\pm0.1$ & $12.9\pm0.1$ & $12.6\pm0.1$ & $12.2\pm0.1$ & $11.8\pm0.1$ & $12.2\pm0.1$ & $13.7\pm0.1$ & $14.3\pm0.1$ & PS1\\
MASTER OT J011330.63+493634.9 & UGC 00766 & $18.4\pm0.1$ & -- & -- & -- & -- & -- & $16.4\pm0.1$ & $15.4\pm0.1$ & $15.1\pm0.1$ & $15.0\pm0.1$ & $15.3\pm0.1$ & $14.7\pm0.1$ & $14.7\pm0.1$ & $15.1\pm0.2$ & $16.5\pm0.1$ & $17.0\pm0.1$ & PS1\\
PSN J04561965-1548027 & IC 2104 & $18.2\pm0.1$ & -- & -- & -- & -- & -- & $ 9.6\pm0.1$ & $12.3\pm0.1$ & $10.0\pm0.1$ & $11.0\pm0.1$ & $ 8.8\pm0.1$ & $11.8\pm0.1$ & $11.6\pm0.1$ & $11.9\pm0.1$ & $13.2\pm0.1$ & $13.7\pm0.1$ & --\\
2014eg & ESO 154-G010 & $16.7\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $11.0\pm0.1$ & $10.6\pm0.1$ & $10.9\pm0.1$ & $12.6\pm0.1$ & $13.0\pm0.1$ & --\\
2014dv & NGC 2501 & $16.8\pm0.1$ & -- & -- & -- & -- & -- & $13.1\pm0.1$ & $12.4\pm0.1$ & $12.0\pm0.1$ & $11.7\pm0.1$ & $11.5\pm0.1$ & $11.1\pm0.1$ & $10.8\pm0.1$ & $11.0\pm0.1$ & $12.8\pm0.1$ & $13.4\pm0.1$ & PS1\\
PSN J10292799+2200468 & UGC 05691 & $17.5\pm0.1$ & $16.9\pm0.1$ & $15.2\pm0.1$ & $14.4\pm0.1$ & $14.0\pm0.1$ & $13.7\pm0.1$ & $16.2\pm0.1$ & $15.1\pm0.1$ & $14.3\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $13.5\pm0.1$ & $13.2\pm0.1$ & $13.5\pm0.1$ & $15.0\pm0.1$ & $15.7\pm0.1$ & SDSS\\
PSN J04173792+3617317 & UGC 03000 & $19.8\pm0.1$ & -- & -- & -- & -- & -- & $15.1\pm0.1$ & $14.2\pm0.1$ & $13.5\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $12.0\pm0.1$ & $11.6\pm0.1$ & $11.7\pm0.1$ & $13.2\pm0.1$ & $13.8\pm0.1$ & PS1\\
2014ea & UGC 05912 & $15.8\pm0.1$ & $15.2\pm0.1$ & $13.9\pm0.1$ & $13.3\pm0.1$ & $13.0\pm0.1$ & $12.9\pm0.1$ & -- & -- & -- & -- & -- & $12.7\pm0.1$ & $12.6\pm0.1$ & $12.6\pm0.1$ & $15.1\pm0.1$ & $15.7\pm0.1$ & SDSS\\
MASTER OT J062509.46+283255.1 & UGC 03462 & -- & -- & -- & -- & -- & -- & $15.9\pm0.1$ & $15.0\pm0.1$ & $14.6\pm0.1$ & $14.4\pm0.1$ & $14.1\pm0.1$ & $13.3\pm0.1$ & $12.9\pm0.1$ & $13.2\pm0.1$ & $15.3\pm0.1$ & $15.9\pm0.1$ & PS1\\
2014dy & 2MASX J02485792-0045389 & $19.9\pm0.2$ & $19.1\pm0.1$ & $17.2\pm0.1$ & $16.3\pm0.1$ & $15.9\pm0.1$ & $15.6\pm0.1$ & $17.2\pm0.1$ & $16.4\pm0.1$ & $16.1\pm0.1$ & $15.8\pm0.1$ & $15.7\pm0.1$ & $15.3\pm0.1$ & $15.0\pm0.1$ & $15.1\pm0.1$ & $16.0\pm0.1$ & $16.5\pm0.1$ & SDSS\\
2014dz & 2MASX J03281358+3800587 & -- & $17.8\pm0.1$ & $15.8\pm0.1$ & $14.9\pm0.1$ & $14.3\pm0.1$ & $14.0\pm0.1$ & $15.9\pm0.1$ & $15.0\pm0.1$ & $14.6\pm0.1$ & $14.2\pm0.1$ & $13.9\pm0.1$ & $13.5\pm0.1$ & $13.4\pm0.1$ & $13.6\pm0.1$ & $14.7\pm0.1$ & $15.4\pm0.1$ & SDSS\\
2014dx & MCG -03-22-002 & $18.6\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.1\pm0.1$ & $11.8\pm0.1$ & $12.0\pm0.1$ & $13.2\pm0.1$ & $13.8\pm0.1$ & --\\
2015B & NGC 4782 & $16.6\pm0.1$ & -- & -- & -- & -- & -- & $12.4\pm0.1$ & $11.7\pm0.1$ & $11.1\pm0.1$ & $10.8\pm0.1$ & $10.6\pm0.1$ & $ 9.7\pm0.1$ & $ 9.5\pm0.1$ & $ 9.7\pm0.1$ & $12.2\pm0.1$ & $12.9\pm0.1$ & PS1\\
LSQ15z & 2MASX J13082255-0844002 & $19.6\pm0.1$ & -- & -- & -- & -- & -- & $17.4\pm0.1$ & $16.8\pm0.1$ & $16.5\pm0.1$ & $16.3\pm0.1$ & $16.1\pm0.1$ & $16.0\pm0.1$ & $15.7\pm0.1$ & $15.8\pm0.1$ & $16.2\pm0.1$ & $16.5\pm0.1$ & PS1\\
2015A & NGC 2955 & $15.7\pm0.1$ & $14.7\pm0.1$ & $13.2\pm0.1$ & $12.6\pm0.1$ & $12.2\pm0.1$ & $11.9\pm0.1$ & $14.2\pm0.1$ & $13.4\pm0.1$ & $12.7\pm0.1$ & $13.1\pm0.1$ & $12.3\pm0.1$ & $12.1\pm0.1$ & $11.8\pm0.1$ & $12.0\pm0.1$ & $13.4\pm0.1$ & $13.9\pm0.1$ & SDSS\\
2015E & KUG 0311+000 & $19.3\pm0.1$ & $18.1\pm0.1$ & $16.8\pm0.1$ & $16.1\pm0.1$ & $15.7\pm0.1$ & $15.5\pm0.1$ & $16.7\pm0.1$ & $16.1\pm0.1$ & $15.8\pm0.1$ & $15.6\pm0.1$ & $15.4\pm0.1$ & $15.2\pm0.1$ & $15.0\pm0.1$ & $15.2\pm0.1$ & $15.8\pm0.1$ & $16.3\pm0.1$ & SDSS\\
2015H & NGC 3464 & $15.0\pm0.1$ & $15.2\pm0.1$ & $13.5\pm0.1$ & $12.6\pm0.1$ & $12.2\pm0.1$ & $11.9\pm0.1$ & $13.1\pm0.1$ & $12.5\pm0.1$ & $12.2\pm0.1$ & $12.0\pm0.1$ & $11.8\pm0.1$ & $11.5\pm0.1$ & $11.3\pm0.1$ & $11.5\pm0.1$ & $14.0\pm0.1$ & $14.6\pm0.1$ & SDSS\\
PSN J13471211-2422171 & ESO 509-G108 & $19.2\pm0.1$ & -- & -- & -- & -- & -- & $14.0\pm0.1$ & $13.2\pm0.1$ & $12.8\pm0.1$ & $12.5\pm0.1$ & $12.2\pm0.1$ & $11.9\pm0.1$ & $11.7\pm0.1$ & $11.9\pm0.1$ & $13.1\pm0.1$ & $13.9\pm0.1$ & PS1\\
iPTF15ku & KUG 1232+315 & $18.4\pm0.1$ & $18.1\pm0.1$ & $17.0\pm0.1$ & $16.5\pm0.1$ & $16.3\pm0.1$ & $16.1\pm0.1$ & $16.8\pm0.1$ & $16.6\pm0.1$ & $16.4\pm0.1$ & $16.3\pm0.1$ & $16.4\pm0.1$ & -- & -- & -- & $17.7\pm0.1$ & $18.1\pm0.1$ & SDSS\\
CSS150214:140955+173155 & NGC 5490 & $17.9\pm0.1$ & $14.8\pm0.1$ & $12.7\pm0.1$ & $11.9\pm0.1$ & $11.5\pm0.1$ & $11.2\pm0.1$ & -- & -- & -- & -- & -- & $10.9\pm0.1$ & $10.7\pm0.1$ & $10.9\pm0.1$ & $12.4\pm0.1$ & $13.1\pm0.1$ & SDSS\\
PSN J19235601-5955321 & NGC 6782 & $15.5\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $10.8\pm0.1$ & $10.6\pm0.1$ & $10.8\pm0.1$ & $12.3\pm0.1$ & $12.9\pm0.1$ & --\\
2015F & NGC 2442 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $ 9.0\pm0.1$ & $ 8.8\pm0.1$ & $ 8.9\pm0.1$ & $11.8\pm0.1$ & $12.4\pm0.1$ & --\\
PS15mb & SDSS J085940.13+151113.5 & -- & $19.8\pm0.1$ & $18.2\pm0.1$ & $17.7\pm0.1$ & $17.4\pm0.1$ & $17.3\pm0.1$ & $18.4\pm0.1$ & $17.6\pm0.1$ & $17.4\pm0.1$ & $17.3\pm0.1$ & $17.2\pm0.1$ & -- & -- & -- & $18.0\pm0.1$ & $18.5\pm0.1$ & SDSS\\
PSN J08593491+4555343 & UGC 04709 & -- & $16.3\pm0.1$ & $14.9\pm0.1$ & $14.3\pm0.1$ & $14.0\pm0.1$ & $13.7\pm0.1$ & $14.6\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $13.6\pm0.1$ & $13.5\pm0.1$ & $13.3\pm0.1$ & $13.5\pm0.1$ & $14.7\pm0.1$ & $15.2\pm0.1$ & SDSS\\
SMTJ10310056-3658262 & ESO 375-G052 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.8\pm0.1$ & $12.7\pm0.1$ & $12.8\pm0.1$ & $14.0\pm0.1$ & $14.7\pm0.1$ & --\\
2015bp & NGC 5839 & $18.0\pm0.1$ & $16.3\pm0.1$ & $13.1\pm0.1$ & $12.2\pm0.1$ & $11.8\pm0.1$ & $11.5\pm0.1$ & -- & -- & -- & -- & -- & $11.2\pm0.1$ & $10.9\pm0.1$ & $11.2\pm0.1$ & $12.7\pm0.1$ & $13.4\pm0.1$ & SDSS\\
PSN J13332289+5843315 & 2MASX J13332590+5843195 & $18.4\pm0.1$ & $17.8\pm0.1$ & $16.6\pm0.1$ & $16.2\pm0.1$ & $15.9\pm0.1$ & $15.7\pm0.1$ & $16.7\pm0.1$ & $16.2\pm0.1$ & $16.0\pm0.1$ & $15.8\pm0.1$ & $15.7\pm0.1$ & $15.8\pm0.1$ & $15.3\pm0.1$ & $15.4\pm0.1$ & $16.5\pm0.1$ & $17.1\pm0.1$ & SDSS\\
LSQ15adm & AM 2010-581 & $19.6\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $15.9\pm0.1$ & $15.6\pm0.1$ & $15.7\pm0.1$ & $17.0\pm0.1$ & $17.4\pm0.1$ & --\\
MASTER OT J074610.09-712224.9 & 2MFGC 06148 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $14.8\pm0.1$ & $14.6\pm0.1$ & $14.8\pm0.1$ & $15.4\pm0.1$ & $16.0\pm0.1$ & --\\
2015I & NGC 2357 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $11.9\pm0.1$ & $11.8\pm0.1$ & $11.5\pm0.1$ & $11.6\pm0.1$ & $13.7\pm0.1$ & $14.2\pm0.1$ & --\\
PS15ahs & MCG +07-37-011 & -- & $17.0\pm0.1$ & $15.7\pm0.1$ & $15.2\pm0.1$ & $14.9\pm0.1$ & $14.6\pm0.1$ & $15.9\pm0.1$ & $15.2\pm0.1$ & $15.0\pm0.1$ & $14.9\pm0.1$ & $14.8\pm0.1$ & $14.8\pm0.1$ & $14.6\pm0.1$ & $14.7\pm0.1$ & $16.3\pm0.1$ & $16.8\pm0.1$ & SDSS\\
2015M & COMAi J130032.301+275841.02 & $22.6\pm0.3$ & $25.1\pm0.7$ & $23.8\pm0.3$ & $22.7\pm0.2$ & $23.1\pm0.4$ & $22.7\pm0.7$ & $19.5\pm0.1$ & -- & $19.2\pm0.1$ & $18.9\pm0.1$ & $19.4\pm0.1$ & -- & -- & -- & -- & -- & PS1\\
PSN J16283836+3932552 & NGC 6166 & -- & $15.8\pm0.1$ & $13.7\pm0.1$ & $12.9\pm0.1$ & $12.4\pm0.1$ & $12.2\pm0.1$ & -- & -- & -- & -- & -- & $11.2\pm0.1$ & $11.0\pm0.1$ & $11.2\pm0.1$ & $13.6\pm0.1$ & $14.2\pm0.1$ & SDSS\\
PSN J16025128+4713292 & UGC 10156 NED01 & -- & $16.5\pm0.1$ & $25.1\pm25.4$ & $24.8\pm29.3$ & $24.4\pm28.4$ & $14.4\pm0.1$ & $14.6\pm0.1$ & -- & $13.2\pm0.1$ & $12.8\pm0.1$ & -- & -- & -- & -- & $12.6\pm0.1$ & $13.0\pm0.1$ & PS1\\
Gaia15agm & ESO 241-G005 & $18.4\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $18.4\pm0.1$ & $19.1\pm0.1$ & --\\
MASTER OT J114925.48-050713.8 & NGC 3915 & -- & -- & -- & -- & -- & -- & $14.2\pm0.1$ & $13.6\pm0.1$ & $13.3\pm0.1$ & $13.2\pm0.1$ & $13.1\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $13.1\pm0.1$ & $14.8\pm0.1$ & $15.4\pm0.1$ & PS1\\
2015ai & UGC 08734 & $18.9\pm0.1$ & $16.3\pm0.1$ & $14.5\pm0.1$ & $13.6\pm0.1$ & $13.2\pm0.1$ & $12.8\pm0.1$ & $14.6\pm0.1$ & $13.9\pm0.1$ & $13.5\pm0.1$ & $13.2\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $12.5\pm0.1$ & $12.7\pm0.1$ & $14.0\pm0.1$ & $14.7\pm0.1$ & SDSS\\
2015N & UGC 11797 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $11.8\pm0.1$ & $11.4\pm0.1$ & $11.5\pm0.1$ & $12.7\pm0.1$ & $13.3\pm0.1$ & --\\
Supernova in Mrk 477 & Mrk 477 & -- & $15.9\pm0.1$ & $14.8\pm0.1$ & $14.7\pm0.1$ & $14.4\pm0.1$ & $14.3\pm0.1$ & $14.9\pm0.1$ & $14.7\pm0.1$ & $14.6\pm0.1$ & $14.5\pm0.1$ & $14.2\pm0.1$ & $14.1\pm0.1$ & $14.0\pm0.1$ & $13.9\pm0.1$ & $14.0\pm0.1$ & $13.4\pm0.1$ & SDSS\\
2015ab & NGC 938 & $19.1\pm0.1$ & $15.2\pm0.1$ & $13.3\pm0.1$ & $12.4\pm0.1$ & $11.9\pm0.1$ & $11.6\pm0.1$ & $13.5\pm0.1$ & $12.7\pm0.1$ & $12.4\pm0.1$ & $12.1\pm0.1$ & $11.9\pm0.1$ & $11.5\pm0.1$ & $11.3\pm0.1$ & $11.5\pm0.1$ & $12.9\pm0.1$ & $13.6\pm0.1$ & SDSS\\
PSN J20435314+1230304 & NGC 6956 & -- & -- & -- & -- & -- & -- & $13.9\pm0.1$ & -- & -- & -- & -- & $11.2\pm0.1$ & $11.0\pm0.1$ & $11.2\pm0.1$ & $13.3\pm0.1$ & $13.9\pm0.1$ & --\\
2015aw & ESO 197-G024 & $17.9\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.7\pm0.1$ & $13.4\pm0.1$ & $13.7\pm0.1$ & $15.5\pm0.1$ & $16.1\pm0.1$ & --\\
2015ac & UGC 12474 & $18.4\pm0.1$ & -- & -- & $15.6\pm0.1$ & $15.0\pm0.1$ & -- & $13.8\pm0.1$ & $13.0\pm0.1$ & $12.6\pm0.1$ & $12.4\pm0.1$ & $12.1\pm0.1$ & $11.8\pm0.1$ & $11.4\pm0.1$ & $11.6\pm0.1$ & $12.9\pm0.1$ & $13.4\pm0.1$ & PS1\\
2015ad & UGC 02282 & -- & -- & -- & -- & -- & -- & $14.3\pm0.1$ & $13.7\pm0.1$ & $13.4\pm0.1$ & $13.2\pm0.1$ & $13.1\pm0.1$ & $13.4\pm0.1$ & $13.1\pm0.1$ & $13.2\pm0.1$ & $15.4\pm0.1$ & $16.0\pm0.1$ & PS1\\
MASTER OT J233743.22-473039.3 & ESO 240-G010 & $17.1\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $10.7\pm0.1$ & $10.4\pm0.1$ & $10.7\pm0.1$ & $12.5\pm0.1$ & $13.1\pm0.1$ & --\\
2015ak & ESO 108-IG021 & $15.3\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.2\pm0.1$ & $12.0\pm0.1$ & $12.2\pm0.1$ & $13.6\pm0.1$ & $13.9\pm0.1$ & --\\
PSN J22412689+3917220 & UGC 12156 & -- & -- & -- & -- & -- & -- & $14.6\pm0.1$ & $14.0\pm0.1$ & $13.7\pm0.1$ & $13.5\pm0.1$ & $13.4\pm0.1$ & $13.9\pm0.1$ & $13.6\pm0.1$ & $13.9\pm0.1$ & $15.8\pm0.1$ & $16.4\pm0.1$ & PS1\\
PSN J00275992+3045595 & UGC 00276 & -- & $17.8\pm0.1$ & $15.4\pm0.1$ & $14.5\pm0.1$ & $14.0\pm0.1$ & $13.5\pm0.1$ & -- & $14.6\pm0.1$ & $14.2\pm0.1$ & $13.9\pm0.1$ & $13.6\pm0.1$ & $13.2\pm0.1$ & $12.8\pm0.1$ & $12.9\pm0.1$ & $14.1\pm0.1$ & $14.5\pm0.1$ & SDSS\\
PSN J23523718+1433092 & UGC 12822 & $19.6\pm0.1$ & $15.9\pm0.1$ & $14.0\pm0.1$ & $13.2\pm0.1$ & $12.8\pm0.1$ & $12.4\pm0.1$ & $14.2\pm0.1$ & $13.5\pm0.1$ & $13.1\pm0.1$ & $12.9\pm0.1$ & $12.8\pm0.1$ & $12.5\pm0.1$ & $12.2\pm0.1$ & $12.4\pm0.1$ & $13.5\pm0.1$ & $14.2\pm0.1$ & SDSS\\
PSN J02524671+4656470 & UGC 02351 & -- & $16.4\pm0.1$ & $14.5\pm0.1$ & $13.5\pm0.1$ & $12.9\pm0.1$ & $12.6\pm0.1$ & $15.9\pm0.1$ & $15.8\pm0.1$ & $13.2\pm0.1$ & $15.1\pm0.1$ & $13.5\pm0.1$ & $12.1\pm0.1$ & $11.9\pm0.1$ & $12.0\pm0.1$ & $13.9\pm0.1$ & $14.6\pm0.1$ & SDSS\\
LSQ15bci & MCG -05-04-023 & $18.8\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.0\pm0.1$ & $12.8\pm0.1$ & $13.0\pm0.1$ & $14.3\pm0.1$ & $14.9\pm0.1$ & --\\
2015ao & ESO 354-G003 & $19.0\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.3\pm0.1$ & $12.1\pm0.1$ & $12.3\pm0.1$ & $13.7\pm0.1$ & $14.4\pm0.1$ & --\\
PS15cku & 2MASX J01242239+0335168 & $17.9\pm0.1$ & $17.8\pm0.1$ & $16.1\pm0.1$ & $15.7\pm0.1$ & $15.4\pm0.1$ & $15.2\pm0.1$ & $16.1\pm0.1$ & $15.8\pm0.1$ & $15.5\pm0.1$ & $15.4\pm0.1$ & $15.3\pm0.1$ & $15.3\pm0.1$ & $15.3\pm0.1$ & $15.4\pm0.1$ & $16.7\pm0.1$ & $17.2\pm0.1$ & SDSS\\
MASTER OT J103747.94-270507.2 & IC 2597 & $17.7\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $10.5\pm0.1$ & $10.3\pm0.1$ & $10.5\pm0.1$ & $12.3\pm0.1$ & $13.0\pm0.1$ & --\\
PSN J02004778+1641365 & 2MASX J02004757+1641401 & $22.1\pm0.4$ & $19.0\pm0.1$ & $17.2\pm0.1$ & $16.2\pm0.1$ & $15.7\pm0.1$ & $15.4\pm0.1$ & $17.3\pm0.1$ & $16.6\pm0.1$ & $15.9\pm0.1$ & $15.7\pm0.1$ & $15.4\pm0.1$ & $15.3\pm0.1$ & $15.1\pm0.1$ & $15.2\pm0.1$ & -- & -- & SDSS\\
PSN J21312375+4336312 & 2MASX J21312321+4336182 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.5\pm0.1$ & $13.0\pm0.1$ & $13.1\pm0.1$ & $13.8\pm0.1$ & $14.1\pm0.1$ & --\\
PSN J09100885+5003396 & UGC 04812 & -- & -- & -- & -- & -- & -- & $14.5\pm0.1$ & $14.1\pm0.1$ & $13.9\pm0.1$ & $13.8\pm0.1$ & $13.8\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $13.9\pm0.1$ & $15.3\pm0.1$ & $15.8\pm0.1$ & PS1\\
CSS151109:101502+074830 & SDSS J101502.54+074826.6 & $20.1\pm0.1$ & $19.1\pm0.1$ & $18.1\pm0.1$ & $17.7\pm0.1$ & $17.5\pm0.1$ & $17.3\pm0.1$ & $18.1\pm0.1$ & $17.8\pm0.1$ & $17.7\pm0.1$ & $17.5\pm0.1$ & $17.6\pm0.1$ & -- & -- & -- & $18.3\pm0.1$ & $18.9\pm0.1$ & SDSS\\
2015ar & NGC 383 & -- & $14.2\pm0.1$ & $12.3\pm0.1$ & $11.4\pm0.1$ & $10.9\pm0.1$ & $10.5\pm0.1$ & $12.9\pm0.1$ & $12.1\pm0.1$ & $11.8\pm0.1$ & $11.4\pm0.1$ & $11.2\pm0.1$ & $10.5\pm0.1$ & $10.3\pm0.1$ & $10.4\pm0.1$ & $12.3\pm0.1$ & $12.9\pm0.1$ & SDSS\\
PSN J07051005+2102327 & 2MASX J07051014+2102233 & -- & -- & -- & -- & -- & -- & $16.6\pm0.1$ & $16.1\pm0.1$ & $15.7\pm0.1$ & $15.5\pm0.1$ & $15.3\pm0.1$ & $15.9\pm0.1$ & $15.9\pm0.1$ & $15.8\pm0.1$ & $16.1\pm0.1$ & $16.3\pm0.1$ & PS1\\
PS15cwx & 2MFGC 04279 & -- & -- & -- & -- & -- & -- & $16.6\pm0.1$ & $15.8\pm0.1$ & $15.3\pm0.1$ & $14.9\pm0.1$ & $14.7\pm0.1$ & $14.4\pm0.1$ & $14.1\pm0.1$ & $14.2\pm0.1$ & $15.8\pm0.1$ & $16.4\pm0.1$ & PS1\\
MASTER OT J215050.94-702028.9 & NGC 7123 & $18.6\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $10.6\pm0.1$ & $10.2\pm0.1$ & $10.4\pm0.1$ & $12.0\pm0.1$ & $12.6\pm0.1$ & --\\
2015az & IC 0290 & -- & $16.7\pm0.1$ & $14.9\pm0.1$ & $14.1\pm0.1$ & $13.6\pm0.1$ & $13.3\pm0.1$ & $14.8\pm0.1$ & $14.1\pm0.1$ & $13.7\pm0.1$ & $13.4\pm0.1$ & $13.2\pm0.1$ & $13.0\pm0.1$ & $12.7\pm0.1$ & $13.0\pm0.1$ & $14.2\pm0.1$ & $15.0\pm0.1$ & SDSS\\
2015bd & NGC 3662 & -- & $16.6\pm0.1$ & $14.5\pm0.1$ & $13.4\pm0.1$ & $12.7\pm0.1$ & $12.2\pm0.1$ & $13.6\pm0.1$ & $12.9\pm0.1$ & $12.6\pm0.1$ & $12.3\pm0.1$ & $12.1\pm0.1$ & $11.7\pm0.1$ & $11.5\pm0.1$ & $11.7\pm0.1$ & $14.0\pm0.1$ & $14.6\pm0.1$ & SDSS\\
CSS151209:232318+164003 & GALEXMSC J232317.78+164003.8 & $22.0\pm0.1$ & $20.2\pm0.1$ & $19.0\pm0.1$ & $18.4\pm0.1$ & $18.1\pm0.1$ & $17.9\pm0.1$ & $18.9\pm0.1$ & $18.4\pm0.1$ & $18.2\pm0.1$ & $18.0\pm0.1$ & $18.2\pm0.1$ & -- & -- & -- & $18.8\pm0.1$ & $19.5\pm0.2$ & SDSS\\
PSN J01534240+2956107 & UGC 01359 & -- & $15.6\pm0.1$ & $14.2\pm0.1$ & $13.5\pm0.1$ & $13.1\pm0.1$ & $12.8\pm0.1$ & -- & $15.2\pm0.1$ & $13.3\pm0.1$ & $13.2\pm0.1$ & $13.2\pm0.1$ & $12.8\pm0.1$ & $12.5\pm0.1$ & $12.6\pm0.1$ & $13.9\pm0.1$ & $14.4\pm0.1$ & SDSS\\
CSS151230:044008+123051 & UGC 03123 & -- & -- & -- & -- & -- & -- & $16.2\pm0.1$ & $15.2\pm0.1$ & $14.7\pm0.1$ & $14.3\pm0.1$ & $13.9\pm0.1$ & $13.5\pm0.1$ & $13.1\pm0.1$ & $13.2\pm0.1$ & $14.4\pm0.1$ & $14.9\pm0.1$ & PS1\\
2016D & 2MASX J04012613-5445295 & $20.0\pm0.2$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.2\pm0.1$ & $13.0\pm0.1$ & $13.1\pm0.1$ & $14.2\pm0.1$ & $14.9\pm0.1$ & --\\
2016W & NGC 946 & $18.8\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $11.7\pm0.1$ & $11.5\pm0.1$ & $11.7\pm0.1$ & $12.9\pm0.1$ & $13.6\pm0.1$ & --\\
ATLAS16aaf & 2MASX J02030578-0350240 & $20.1\pm0.1$ & $17.6\pm0.1$ & $15.9\pm0.1$ & $15.3\pm0.1$ & $14.9\pm0.1$ & $14.7\pm0.1$ & $16.0\pm0.1$ & $15.4\pm0.1$ & $15.1\pm0.1$ & $15.0\pm0.1$ & $14.7\pm0.1$ & $14.7\pm0.1$ & $14.4\pm0.1$ & $14.6\pm0.1$ & $15.5\pm0.1$ & $16.2\pm0.1$ & SDSS\\
ATLAS16aab & 2MASX J03214217+4205549 & -- & $18.2\pm0.1$ & $16.3\pm0.1$ & $15.3\pm0.1$ & $14.9\pm0.1$ & $14.7\pm0.1$ & $16.5\pm0.1$ & $15.7\pm0.1$ & $15.2\pm0.1$ & $15.0\pm0.1$ & $14.7\pm0.1$ & $14.5\pm0.1$ & $14.2\pm0.1$ & $14.4\pm0.1$ & $15.9\pm0.1$ & $16.5\pm0.1$ & SDSS\\
MASTER OT J105908.57+103834.8 & SDSS J105908.63+103829.7 & $21.3\pm0.2$ & $21.1\pm0.2$ & $20.0\pm0.1$ & $19.6\pm0.1$ & $19.5\pm0.1$ & $19.8\pm0.3$ & $20.3\pm0.1$ & $19.8\pm0.1$ & $20.0\pm0.1$ & $20.0\pm0.1$ & $19.9\pm0.1$ & -- & -- & -- & $20.3\pm0.2$ & $19.8\pm0.3$ & SDSS\\
2016adi & NGC 5292 & $15.8\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $10.7\pm0.1$ & $10.5\pm0.1$ & $10.7\pm0.1$ & $12.8\pm0.1$ & $13.5\pm0.1$ & --\\
2016ajf & NGC 1278 & $19.1\pm0.1$ & $15.3\pm0.1$ & $13.2\pm0.1$ & $12.2\pm0.1$ & $11.7\pm0.1$ & $11.3\pm0.1$ & $13.7\pm0.1$ & $12.9\pm0.1$ & $12.3\pm0.1$ & $12.0\pm0.1$ & $11.9\pm0.1$ & $11.2\pm0.1$ & $10.9\pm0.1$ & $11.1\pm0.1$ & $12.8\pm0.1$ & $13.5\pm0.1$ & SDSS\\
Gaia16aeu & 2dFGRS S394Z183 & $20.4\pm0.1$ & -- & -- & -- & -- & -- & $19.0\pm0.1$ & $18.2\pm0.1$ & $17.8\pm0.1$ & $17.9\pm0.1$ & $17.8\pm0.1$ & -- & -- & -- & $18.1\pm0.1$ & $19.1\pm0.1$ & PS1\\
Gaia16agf & Uncatalogued & -- & -- & -- & -- & -- & -- & $16.5\pm0.1$ & $16.2\pm0.1$ & $16.1\pm0.1$ & $15.9\pm0.1$ & $15.9\pm0.1$ & -- & -- & -- & -- & -- & PS1\\
2016aqt & SDSS J134550.90+264747.4 & $19.1\pm0.1$ & $18.8\pm0.1$ & $17.8\pm0.1$ & $17.4\pm0.1$ & $17.2\pm0.1$ & $17.1\pm0.1$ & $18.2\pm0.1$ & $17.8\pm0.1$ & $17.5\pm0.1$ & $17.6\pm0.1$ & $18.5\pm0.1$ & -- & -- & -- & $18.8\pm0.1$ & $19.4\pm0.1$ & SDSS\\
2016bfu & IC 2150 & $15.7\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.0\pm0.1$ & $11.9\pm0.1$ & $12.0\pm0.1$ & $14.6\pm0.1$ & $15.1\pm0.1$ & --\\
MASTER OT J152333.04+092125.6 & CGCG 077-110 & $20.1\pm0.2$ & $16.3\pm0.1$ & $14.4\pm0.1$ & $13.5\pm0.1$ & $13.1\pm0.1$ & $12.8\pm0.1$ & $14.5\pm0.1$ & $13.8\pm0.1$ & $13.5\pm0.1$ & $13.2\pm0.1$ & $12.9\pm0.1$ & $12.8\pm0.1$ & $12.5\pm0.1$ & $12.7\pm0.1$ & $13.8\pm0.1$ & $14.5\pm0.1$ & SDSS\\
iPTF16abc & NGC 5221 & $17.6\pm0.1$ & $15.9\pm0.1$ & $13.9\pm0.1$ & $13.0\pm0.1$ & $12.5\pm0.1$ & $12.1\pm0.1$ & $13.9\pm0.1$ & $13.1\pm0.1$ & $12.7\pm0.1$ & $12.5\pm0.1$ & $12.2\pm0.1$ & $12.1\pm0.1$ & $11.8\pm0.1$ & $12.0\pm0.1$ & $13.5\pm0.1$ & $14.0\pm0.1$ & SDSS\\
2016brx & NGC 7391 & $18.5\pm0.1$ & $14.9\pm0.1$ & $12.8\pm0.1$ & $11.9\pm0.1$ & $11.4\pm0.1$ & $11.1\pm0.1$ & -- & -- & -- & -- & -- & $10.6\pm0.1$ & $10.4\pm0.1$ & $10.6\pm0.1$ & $12.2\pm0.1$ & $12.9\pm0.1$ & SDSS\\
2016bry & UGC 11635 & $16.6\pm0.1$ & -- & -- & -- & -- & -- & $13.5\pm0.1$ & $12.7\pm0.1$ & $12.2\pm0.1$ & $12.0\pm0.1$ & $11.7\pm0.1$ & $11.4\pm0.1$ & $11.2\pm0.1$ & $11.3\pm0.1$ & $13.2\pm0.1$ & $13.7\pm0.1$ & PS1\\
Gaia16alq & Uncatalogued & -- & -- & -- & -- & -- & -- & $19.6\pm0.1$ & $19.2\pm0.1$ & $19.1\pm0.1$ & $19.0\pm0.1$ & $19.1\pm0.1$ & -- & -- & -- & -- & -- & PS1\\
CSS160427:134449+210448 & SDSS J134448.50+210447.1 & $21.8\pm0.4$ & $21.2\pm0.1$ & $20.0\pm0.1$ & $19.6\pm0.1$ & $19.4\pm0.1$ & $19.3\pm0.1$ & $20.0\pm0.1$ & $19.6\pm0.1$ & $19.5\pm0.1$ & $19.3\pm0.1$ & $19.4\pm0.1$ & -- & -- & -- & $20.1\pm0.1$ & $20.2\pm0.3$ & SDSS\\
iPTF16auf & Mrk 0685 & -- & $15.3\pm0.1$ & $14.6\pm0.1$ & $14.5\pm0.1$ & $14.3\pm0.1$ & $14.2\pm0.1$ & -- & -- & -- & -- & -- & $14.6\pm0.1$ & $14.5\pm0.1$ & $14.8\pm0.1$ & $15.5\pm0.1$ & $15.8\pm0.1$ & SDSS\\
MASTER OT J202606.27-200732.6 & GALEXASC J202606.38-200732.4 & $20.5\pm0.1$ & -- & -- & -- & -- & -- & $17.1\pm0.1$ & $16.9\pm0.1$ & $16.8\pm0.1$ & $16.9\pm0.1$ & $16.9\pm0.1$ & $16.7\pm0.1$ & $17.2\pm0.1$ & $17.4\pm0.2$ & $18.3\pm0.1$ & $19.0\pm0.1$ & PS1\\
KAIT-16X & NGC 4125 & $15.9\pm0.1$ & $13.0\pm0.1$ & $11.0\pm0.1$ & $10.1\pm0.1$ & $ 9.6\pm0.1$ & $ 9.3\pm0.1$ & -- & -- & -- & -- & -- & $ 8.8\pm0.1$ & $ 8.6\pm0.1$ & $ 8.8\pm0.1$ & $11.2\pm0.1$ & $11.8\pm0.1$ & SDSS\\
ATLAS16bdg & NGC 4708 & $16.3\pm0.1$ & -- & -- & -- & -- & -- & $13.6\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $12.6\pm0.1$ & $12.4\pm0.1$ & $12.1\pm0.1$ & $12.0\pm0.1$ & $12.2\pm0.1$ & $14.0\pm0.1$ & $14.4\pm0.1$ & PS1\\
PTSS-16ijc & CGCG 280-024 & -- & -- & -- & -- & -- & -- & $15.3\pm0.1$ & $14.4\pm0.1$ & $14.1\pm0.1$ & $13.8\pm0.1$ & $13.6\pm0.1$ & $13.3\pm0.1$ & $13.0\pm0.1$ & $13.2\pm0.1$ & $14.4\pm0.1$ & $15.1\pm0.1$ & PS1\\
MASTER OT J211223.35+144645.1 & GALEXASC J211223.05+144644.9 & $19.9\pm0.1$ & -- & -- & -- & -- & -- & $17.7\pm0.1$ & $17.1\pm0.1$ & $16.9\pm0.1$ & $16.8\pm0.1$ & $16.4\pm0.1$ & $16.6\pm0.1$ & $16.4\pm0.1$ & $16.6\pm0.1$ & $17.4\pm0.1$ & $18.0\pm0.1$ & PS1\\
CSS160708:151956+052419 & SDSS J151955.92+052418.9 & -- & $25.2\pm1.2$ & $22.5\pm0.2$ & $22.5\pm0.2$ & $22.0\pm0.2$ & $23.3\pm1.1$ & $23.5\pm0.1$ & $22.5\pm0.1$ & $22.1\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & PS1\\
2016dag & ESO 018-G002 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $11.4\pm0.1$ & $11.1\pm0.1$ & $11.3\pm0.1$ & $13.2\pm0.1$ & $13.9\pm0.1$ & --\\
2016ekg & ESO 466-G032 & $17.4\pm0.1$ & -- & -- & -- & -- & -- & $15.9\pm0.1$ & $15.7\pm0.1$ & $15.2\pm0.1$ & $15.5\pm0.1$ & $15.5\pm0.1$ & $15.9\pm0.1$ & $15.9\pm0.1$ & $16.2\pm0.2$ & $17.1\pm0.1$ & $17.5\pm0.1$ & PS1\\
Gaia16axi & 2MASX J05595753-1805253 & $18.5\pm0.1$ & -- & -- & -- & -- & -- & $15.0\pm0.1$ & $14.2\pm0.1$ & $13.9\pm0.1$ & $13.6\pm0.1$ & $13.4\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $12.8\pm0.1$ & $13.8\pm0.1$ & $14.3\pm0.1$ & PS1\\
2016eoa & NGC 83 & $18.8\pm0.1$ & $15.4\pm0.1$ & $13.4\pm0.1$ & $12.4\pm0.1$ & $11.9\pm0.1$ & $11.5\pm0.1$ & -- & -- & -- & -- & -- & $11.3\pm0.1$ & $11.1\pm0.1$ & $11.2\pm0.1$ & $12.7\pm0.1$ & $13.3\pm0.1$ & SDSS\\
ATLAS16cjv & IC 0272 & $16.9\pm0.1$ & -- & -- & -- & -- & -- & $14.4\pm0.1$ & $13.8\pm0.1$ & $13.5\pm0.1$ & $13.3\pm0.1$ & $13.0\pm0.1$ & $12.9\pm0.1$ & $12.6\pm0.1$ & $12.8\pm0.1$ & $14.6\pm0.1$ & $15.2\pm0.1$ & PS1\\
Gaia16bba & GALEXASC J010135.75+170604.9 & $20.9\pm0.2$ & $19.9\pm0.1$ & $19.0\pm0.1$ & $18.6\pm0.1$ & $18.4\pm0.1$ & $18.2\pm0.1$ & $19.1\pm0.1$ & $18.6\pm0.1$ & $18.5\pm0.1$ & $18.5\pm0.1$ & $18.8\pm0.1$ & -- & -- & -- & $19.5\pm0.1$ & $20.0\pm0.3$ & SDSS\\
Gaia16bbi & GALEXASC J235916.23+220302.4 & $19.5\pm0.1$ & $18.8\pm0.1$ & $18.1\pm0.1$ & $17.9\pm0.1$ & $17.7\pm0.1$ & $17.6\pm0.1$ & $18.1\pm0.1$ & $17.8\pm0.1$ & $17.7\pm0.1$ & $17.6\pm0.1$ & $17.6\pm0.1$ & -- & -- & -- & $18.2\pm0.1$ & $18.8\pm0.1$ & SDSS\\
ATLAS16cpu & CGCG 249-11 & $18.6\pm0.1$ & $16.4\pm0.1$ & $14.9\pm0.1$ & $14.1\pm0.1$ & $13.7\pm0.1$ & $13.4\pm0.1$ & $15.0\pm0.1$ & $14.3\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $13.6\pm0.1$ & $13.5\pm0.1$ & $13.2\pm0.1$ & $13.4\pm0.1$ & $14.4\pm0.1$ & $15.0\pm0.1$ & SDSS\\
MASTER OT J021729.29-595123.9 & NGC 888 & $19.2\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $12.1\pm0.1$ & $11.8\pm0.1$ & $12.0\pm0.1$ & $13.3\pm0.1$ & $14.0\pm0.1$ & --\\
2016fnr & UGC 10502 & $15.3\pm0.1$ & -- & -- & -- & -- & -- & $13.5\pm0.1$ & $12.9\pm0.1$ & $12.6\pm0.1$ & $12.4\pm0.1$ & $12.3\pm0.1$ & $12.3\pm0.1$ & $12.2\pm0.1$ & $12.4\pm0.1$ & $15.1\pm0.1$ & $15.8\pm0.1$ & PS1\\
Gaia16bew & GALEXASC J140251.91-303700.7 & $17.8\pm0.2$ & -- & -- & -- & -- & -- & $17.7\pm0.1$ & $17.4\pm0.1$ & $17.0\pm0.1$ & $16.9\pm0.1$ & $16.7\pm0.1$ & -- & -- & -- & $16.5\pm0.1$ & $17.2\pm0.1$ & PS1\\
CSS160904:230721+025428 & Uncatalogued & -- & $22.4\pm0.2$ & $21.1\pm0.1$ & $20.6\pm0.1$ & $20.5\pm0.1$ & $20.4\pm0.1$ & $21.1\pm0.1$ & $20.9\pm0.1$ & $20.6\pm0.1$ & $20.4\pm0.1$ & $20.8\pm0.2$ & -- & -- & -- & -- & -- & SDSS\\
2016gfk & IC 1657 & $15.4\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $11.5\pm0.1$ & $11.2\pm0.1$ & $11.4\pm0.1$ & $13.1\pm0.1$ & $13.5\pm0.1$ & --\\
2016gfr & 2MASX J18193566+2347137 & $20.9\pm0.2$ & $17.4\pm0.1$ & $15.6\pm0.1$ & $14.7\pm0.1$ & $14.3\pm0.1$ & $14.1\pm0.1$ & $15.8\pm0.1$ & $15.1\pm0.1$ & $14.7\pm0.1$ & $14.4\pm0.1$ & $14.3\pm0.1$ & $14.0\pm0.1$ & $13.8\pm0.1$ & $14.0\pm0.1$ & $15.1\pm0.1$ & $15.7\pm0.1$ & SDSS\\
Gaia16bhj & MCG -01-12-008 & $17.1\pm0.1$ & -- & -- & -- & -- & -- & $14.5\pm0.1$ & $13.9\pm0.1$ & $13.6\pm0.1$ & $13.4\pm0.1$ & $13.3\pm0.1$ & $13.1\pm0.1$ & $12.8\pm0.1$ & $13.0\pm0.1$ & $14.4\pm0.1$ & $15.0\pm0.1$ & PS1\\
2016ghq & UGC 11199 & $17.8\pm0.1$ & -- & -- & -- & -- & -- & $14.5\pm0.1$ & $13.6\pm0.1$ & $13.1\pm0.1$ & $13.0\pm0.1$ & $12.8\pm0.1$ & $12.8\pm0.1$ & $12.6\pm0.1$ & $12.8\pm0.1$ & $13.8\pm0.1$ & $14.5\pm0.1$ & PS1\\
OGLE16dha & GALEXASC J063224.91-713403.9 & $17.3\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $16.5\pm0.1$ & $17.0\pm0.1$ & --\\
SNhunt325 & CGCG 500-022 & $17.7\pm0.1$ & $16.7\pm0.1$ & $15.6\pm0.1$ & $15.1\pm0.1$ & $14.7\pm0.1$ & $14.5\pm0.1$ & $15.5\pm0.1$ & $15.1\pm0.1$ & $14.8\pm0.1$ & $14.7\pm0.1$ & $14.5\pm0.1$ & $14.4\pm0.1$ & $14.2\pm0.1$ & $14.4\pm0.1$ & $15.1\pm0.1$ & $15.6\pm0.1$ & SDSS\\
Gaia16bkz & NGC 2865 & $16.9\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $10.4\pm0.1$ & $10.2\pm0.1$ & $10.4\pm0.1$ & $12.2\pm0.1$ & $12.8\pm0.1$ & --\\
2016gxp & NGC 51 & $18.5\pm0.1$ & -- & -- & -- & -- & -- & $13.6\pm0.1$ & -- & $12.6\pm0.1$ & $12.2\pm0.1$ & $12.1\pm0.1$ & $11.5\pm0.1$ & $11.3\pm0.1$ & $11.4\pm0.1$ & $12.8\pm0.1$ & $13.4\pm0.1$ & PS1\\
ATLAS16dmf & UGC 05356 & -- & $17.3\pm0.1$ & $15.4\pm0.1$ & $14.6\pm0.1$ & $14.3\pm0.1$ & $13.9\pm0.1$ & $17.1\pm0.1$ & $16.8\pm0.1$ & $14.3\pm0.1$ & $14.5\pm0.1$ & $14.3\pm0.1$ & $13.5\pm0.1$ & $13.3\pm0.1$ & $13.5\pm0.1$ & $15.4\pm0.1$ & $15.9\pm0.1$ & SDSS\\
ATLAS16dou & 2MASX J06045961-3324449 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.2\pm0.1$ & $12.9\pm0.1$ & $13.0\pm0.1$ & $14.1\pm0.1$ & $14.7\pm0.1$ & --\\
MASTER OT J033333.26-623314.7 & 2MASX J03333430-6233033 & $20.3\pm0.2$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.8\pm0.1$ & $13.4\pm0.1$ & $13.5\pm0.1$ & $14.6\pm0.1$ & $15.2\pm0.1$ & --\\
MASTER OT J110533.80+194118.7 & SDSS J110534.12+194118.9 & $17.3\pm0.1$ & $22.3\pm0.2$ & $21.5\pm0.1$ & $21.4\pm0.1$ & $21.4\pm0.1$ & $21.1\pm0.3$ & $15.8\pm0.1$ & $15.4\pm0.1$ & $15.3\pm0.1$ & $15.3\pm0.1$ & $15.0\pm0.1$ & -- & -- & -- & -- & -- & PS1\\
ATLAS16dtf & UGC 03524 & -- & -- & -- & -- & -- & -- & $15.3\pm0.1$ & $14.1\pm0.1$ & $13.6\pm0.1$ & $13.1\pm0.1$ & $12.9\pm0.1$ & $12.1\pm0.1$ & $11.7\pm0.1$ & $11.8\pm0.1$ & $13.2\pm0.1$ & $13.8\pm0.1$ & PS1\\
Gaia16byh & ESO 374-G025 & $17.1\pm0.1$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & $13.3\pm0.1$ & $13.1\pm0.1$ & $13.2\pm0.1$ & $14.3\pm0.1$ & $14.7\pm0.1$ & --\\
Gaia16caa & UGC 09165 & $17.9\pm0.1$ & $16.4\pm0.1$ & $14.8\pm0.1$ & $13.8\pm0.1$ & $13.3\pm0.1$ & $12.9\pm0.1$ & $15.6\pm0.1$ & $14.9\pm0.1$ & $14.5\pm0.1$ & $13.2\pm0.1$ & $13.0\pm0.1$ & $12.5\pm0.1$ & $12.2\pm0.1$ & $12.2\pm0.1$ & $13.3\pm0.1$ & $13.7\pm0.1$ & SDSS\\
Gaia16cay & NGC 5032 & -- & $15.2\pm0.1$ & $13.3\pm0.1$ & $12.5\pm0.1$ & $12.0\pm0.1$ & $11.7\pm0.1$ & $15.2\pm0.1$ & $12.7\pm0.1$ & $12.4\pm0.1$ & $12.3\pm0.1$ & $12.1\pm0.1$ & $11.8\pm0.1$ & $11.6\pm0.1$ & $11.7\pm0.1$ & $13.8\pm0.1$ & $14.5\pm0.1$ & SDSS\\
MASTER OT J133905.0-201718.3 & 2MASX J13390624-2017235 & $18.5\pm0.1$ & -- & -- & -- & -- & -- & $15.7\pm0.1$ & $15.1\pm0.1$ & $14.8\pm0.1$ & $14.6\pm0.1$ & $14.4\pm0.1$ & $14.2\pm0.1$ & $13.9\pm0.1$ & $14.1\pm0.1$ & $14.9\pm0.1$ & $15.1\pm0.1$ & PS1\\
Gaia16cbd & UGC 07367 & $18.5\pm0.1$ & $15.0\pm0.1$ & $13.2\pm0.1$ & $12.4\pm0.1$ & $12.0\pm0.1$ & $11.7\pm0.1$ & $13.3\pm0.1$ & $12.6\pm0.1$ & $12.3\pm0.1$ & $12.0\pm0.1$ & $11.8\pm0.1$ & $11.5\pm0.1$ & $11.3\pm0.1$ & $11.5\pm0.1$ & $12.9\pm0.1$ & $13.6\pm0.1$ & SDSS\\
ATLAS16dzg & CGCG 068-006 & $17.3\pm0.1$ & $16.3\pm0.1$ & $15.2\pm0.1$ & $14.6\pm0.1$ & $14.4\pm0.1$ & $14.1\pm0.1$ & $15.1\pm0.1$ & $14.6\pm0.1$ & $14.4\pm0.1$ & $14.2\pm0.1$ & $14.0\pm0.1$ & $13.9\pm0.1$ & $13.6\pm0.1$ & $13.8\pm0.1$ & $14.5\pm0.1$ & $15.0\pm0.1$ & SDSS\\
ATLAS16dzp & SDSS J084324.74+373246.0 & $21.4\pm0.2$ & $20.9\pm0.1$ & $19.8\pm0.1$ & $19.5\pm0.1$ & $19.2\pm0.1$ & $19.1\pm0.1$ & $19.8\pm0.1$ & $19.5\pm0.1$ & $19.3\pm0.1$ & $19.2\pm0.1$ & $19.3\pm0.1$ & -- & -- & -- & $19.4\pm0.1$ & -- & SDSS\\
\hline
\end{tabular}
\medskip
\raggedright
\noindent This table is available in its entirety in a machine readable form. A portion is shown here for guidance regarding its form and content.\\
$^{a}$ The full table contains additional columns for PS1, 2MASS, and WISE magnitudes.\\
$^{b}$ This column denotes which survey produced the optical magnitudes used in the modeling (if any).\\
\label{tab:phot_table}
\end{minipage}
\end{table}

